StructXLIP: Enhancing Vision-language Models with Multimodal Structural Cues

Edge-based representations are fundamental cues for visual understanding, a principle rooted in early vision research and still central today. We extend this principle to vision-language alignment, showing that isolating and aligning structural cues across modalities can greatly benefit fine-tuning on long, detail-rich captions, with a specific focus on improving cross-modal retrieval. We introduce StructXLIP, a fine-tuning alignment paradigm that extracts edge maps (e.g., Canny), treating them as proxies for the visual structure of an image, and filters the corresponding captions to emphasize structural cues, making them "structure-centric". Fine-tuning augments the standard alignment loss with three structure-centric losses: (i) aligning edge maps with structural text, (ii) matching local edge regions to textual chunks, and (iii) connecting edge maps to color images to prevent representation drift. From a theoretical standpoint, while standard CLIP maximizes the mutual information between visual and textual embeddings, StructXLIP additionally maximizes the mutual information between multimodal structural representations. This auxiliary optimization is intrinsically harder, guiding the model toward more robust and semantically stable minima, enhancing vision-language alignment. Beyond outperforming current competitors on cross-modal retrieval in both general and specialized domains, our method serves as a general boosting recipe that can be integrated into future approaches in a plug-and-play manner. Code and pretrained models are publicly available at: https://github.com/intelligolabs/StructXLIP.

==> sec/3bis_proof.tex <==
\section{Generative Assumptions and Causal Structure}
We assume that both visual and textual modalities are generated from a
shared latent semantic variable $S$. 
The corresponding generative directed acyclic graph (DAG) is:
\[
S \longrightarrow (X,Y) \longrightarrow (X_E, Y_E),
\]
where:
\begin{itemize}
    \item $S$ denotes the latent semantic content (e.g., \emph{``a dog running''});
    \item $X = h_X(S, N_X)$ is the observed RGB image, with $h_X$ image generative function
          depending on $S$ and a visual nuisance term $N_X$;
    \item $Y = h_Y(S, N_Y)$ is the textual description, with $h_Y$ text generative function
          depending on $S$ and a linguistic nuisance term $N_Y$;
    \item $X_E = g_E(X, \eta_X)$ and $Y_E = h_E(Y, \eta_Y)$
          are structural projections (e.g., edge maps and edge--focused text), each computed from its own modality with independent internal noise. 
      \item \SW{Each Projection forms conditional kernels $Q(X_E|X)\coloneqq\text{Pr}\left(X_E = g_E(X, \eta_X)\right)$ and $R(Y_E|Y)\coloneqq\text{Pr}\left(Y_E = h_E(Y, \eta_Y)\right)$. }
\end{itemize}
All noise variables
$N_X, N_Y, \eta_X, \eta_Y$
are mutually independent and independent of $S$.
There is no causal link between $X$ and $Y$:
The dependency between them is correlational and entirely mediated by $S$.
\vspace{4pt}

This structure defines a directional Markov chain:
\[
\text{(Visual-Textual)}\;\; S \to (X,Y) \to (X_E,Y_E),
\]
which will be used in the theorem below to derive
mutual information invariance properties.

\begin{theorem}[Mutual Information Invariance under Markov Chain]
\label{thm:mi_invariance_dual}
Let $S$ be a latent semantic variable, and consider the
generative chain:
\[
\text{(Markov chain)} \qquad S \;\longrightarrow\; (X,Y) \;\longrightarrow\; (X_E, Y_E).
\]
Assume that the noise terms involved in each mapping are mutually independent:
\[
N_X,\, N_Y,\, \eta_X,\, \eta_Y \;\perp\!\!\!\perp\; S,\quad
N_X,\, N_Y,\, \eta_X,\, \eta_Y \text{ all mutually independent.}
\]
Then the following holds:
\begin{enumerate}
  \item (Inequality of Mutual Information). The relation of mutual information in the chain satisfies:
\begin{eqnarray}
    I(X_E; Y_E)  \;\le\; I(X; Y).
    \label{eq:dual_mi_chain}
\end{eqnarray}
 \item (Invariance of the Total Mutual Information). The total mutual information remains invariant:
    \begin{equation}
        I\big( (X, X_E) ; (Y, Y_E) \big) = I(X; Y).
        \label{eq:dual_mi_invariance}
    \end{equation}
\end{enumerate}
\end{theorem}


\begin{proof} %[Proof]
\emph{(1) Inequality of mutual information.}
%\paragraph{(1) Inequality among parallel channels}
\begin{align}
&\text{Given the channel:} \nonumber\\[3pt]
&\quad S \rightarrow (X,Y)\rightarrow (X_E,Y_E), \\[3pt]
&\text{with independent channel noises } 
\eta_X \perp\!\!\!\perp \eta_Y,
\text{ and no direct link between } X,Y,X_E,Y_E. \nonumber
\end{align}

\noindent
According to the conditional kernels between $(X,Y)$ and $(X_E,Y_E)$, the relation of their probabilistic distributions is denoted by: 
\begin{eqnarray}
\begin{aligned}
    p(x_E,y_E) & \;=\; \sum_{x \in X} \sum_{y \in Y} Q(x_E|x) R(y_E, y) p(x,y), \\
    p(x_E) & \;=\; \sum_{x \in X} Q(x_E|x) p(x), \\
    p(y_E) & \;=\; \sum_{y \in Y} R(y_E|y) p(y).
    \label{eq:prob_dist_relation}
\end{aligned}
\end{eqnarray}

By definition, the mutual information of $(X_E, Y_E)$ is expressed as:
\begin{eqnarray}
\begin{aligned}
    I(X_E; Y_E) \;=\; \sum_{x_E \in X_E} \sum_{y_E \in Y_E} p(x_E,y_E) \log\frac{ p(x_E,y_E)}{p(x_E)p(y_E)}, 
                % & \;\le\; 
\end{aligned}
\label{eq:I_definition}
\end{eqnarray}

According to the log sum inequality, the following inequality holds:
\begin{eqnarray}
\begin{aligned}
    I(X_E; Y_E) & \;\le\; \sum_{x_E \in X_E} \sum_{y_E \in Y_E} \sum_{x \in X} \sum_{y \in Y}  Q(x_E|x) R(y_E, y) p(x,y) \log\frac{ Q(x_E|x) R(y_E, y) p(x,y) }{Q(x_E|x) p(x)R(y_E, y) p(y)}, \\
                & \;=\; \sum_{x \in X} \sum_{y \in Y} p(x,y) \log\frac{ p(x,y) }{p(x) p(y)} \sum_{x_E \in X_E}  Q(x_E|x) \sum_{y_E \in Y_E} R(y_E, y), \\
                & \;=\; \sum_{x \in X} \sum_{y \in Y} p(x,y) \log\frac{ p(x,y) }{p(x) p(y)} \\
                & \;=\; I(X;Y).
\end{aligned}
\label{eq:I_derive}
\end{eqnarray}
\noindent
Equality holds if and only if both mappings
$X \!\mapsto\! X_E$ and $Y \!\mapsto\! Y_E$
are information-lossless, i.e.,
if $X_E$ and $Y_E$ are sufficient statistics of $X$ and $Y$
for predicting the other modality. Intuitively, each local transformation (\eg\ converting $X$ into $X_E$) can only discard, never increase, the amount of cross–modal information shared through~$S$.

\emph{(2) Invariance of the Total Mutual Information.}
%\paragraph{(2) Expanding the total mutual information.}
We next show that the \emph{total} mutual information between the augmented variables is invariant.
Using the chain rule for mutual information (Cover and Thomas,~2006,~§2.5):
\[
I((X,X_E);(Y,Y_E))
  = I(X;Y,Y_E) + I(X_E;Y,Y_E\,|\,X).
\]
Expanding the first term again by the chain rule gives
\[
I(X;Y,Y_E) = I(X;Y) + I(X;Y_E\,|\,Y).
\]
Substituting, we obtain
\begin{equation}
I((X,X_E);(Y,Y_E))
  = I(X;Y)
  + I(X;Y_E\,|\,Y)
  + I(X_E;Y,Y_E\,|\,X).
\label{eq:chain_expansion}
\end{equation}
%
%\paragraph{Step 4. Eliminating conditional terms.}
Under the independences stated above,
\[
I(X_E;Y,Y_E\,|\,X) = 0, 
\qquad
I(X;Y_E\,|\,Y) = 0.
\]
Substituting these results into Eq.~\eqref{eq:chain_expansion} leaves
\begin{equation}
I((X,X_E);(Y,Y_E)) = I(X;Y),
\label{eq:mi_invariance_final}
\end{equation}
which proves Eq.~(2) of the theorem.
\qed
\paragraph{Interpretation.}
Equations~\eqref{eq:prob_dist_relation}–\eqref{eq:mi_invariance_final} together imply that adding the structural projections $(X_E,Y_E)$ cannot increase the total mutual information between modalities. 
The augmented variables $(X_E,Y_E)$ are merely local, noise–perturbed views of $(X,Y)$ derived from the same latent source~$S$.
By the DPI, any deterministic or stochastic transformation acting within a single modality can only reduce---never create---cross–modal dependence.
In practice, incorporating $(X_E,Y_E)$ in the learning objective therefore acts as an \emph{inductive regularizer}: it encourages the encoders to capture the semantic information~$S$ that is invariant across modalities, while suppressing nuisance factors such as $N_X$ and $N_Y$ (e.g., texture, color, or linguistic style). 
This explains why edge–based auxiliary losses improve alignment stability without altering the theoretical information content.
\end{proof}

\section{Control-variate Estimator for Mutual Information between Texts and Images}
We verified that the mutual information between text and images is not increased by adding edge information; rather, it is regularized. The following section illustrates how this effect takes place.
\SW{
\begin{theorem}[Control-variate estimator for mutual information between texts and images]
\label{thm:cve_for_mi}
Define the control–variate estimator $\widehat{I}_{cv}$  for the mutual information $I(X,Y)$ as
\begin{equation}
\widehat{I}_{cv} = \widehat{I}_{XY} + \beta\,(\widehat{I}_{EE} - \mu_{EE}),
\qquad
\mu_{EE} = \mathbb{E}[\widehat{I}_{EE}],
\end{equation}
where $\widehat{I}_{XY}$ and $\widehat{I}_{EE}$ denote the mutual information estimators between variables $(X;Y)$ and $(X_E;Y_E)$, respectively. \newline
Under the mutual independence assumptions of Theorem~\ref {thm:mi_invariance_dual}, the total variance of the control-variate estimator $\hat I_{cv}$ can be expressed as:
\begin{equation}
\mathrm{Var}[\widehat{I}_{cv}]
  = \mathrm{Var}[\widehat{I}_{XY}](1 - \rho^2).
\end{equation}
where $\rho$ represents the correlation between two estimators:
\begin{equation}
\rho = 
\frac{\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE})}
     {\sqrt{\mathrm{Var}[\widehat{I}_{XY}]\,\mathrm{Var}[\widehat{I}_{EE}]}}.
\end{equation}
In addition, assume that the $I_{cv}$ and $I_{XY}$ are correlated (\ref{eq:rho_def}), i.e. :
\[ \rho > 0 \] 
The control-variate estimator $\hat I_{cv}$ for the mutual information $I(X,Y)$ reduces the variance of the mutual-information estimate without altering its expected value.
\end{theorem}}

\begin{proof}[Extended Proof] 
\SW{We can partition the proof into three steps.}

\subsection{Construction of the estimator with a control variate}

\subsubsection{Definition}
% We define the control–variate estimator as
\SW{Define the control–variate estimator for the mutual information $I(X,Y)$ as}
\begin{equation}
\widehat{I}_{cv} = \widehat{I}_{XY} + \beta\,(\widehat{I}_{EE} - \mu_{EE}),
\qquad
\mu_{EE} = \mathbb{E}[\widehat{I}_{EE}].
\label{eq:control_variate}
\end{equation}
The term $-\mu_{EE}$ simply \emph{centers} the control variate, 
i.e., it removes its mean so that the added component has zero expectation.

\subsubsection{Unchanged expectation}

The expectation of the estimator therefore remains unaltered:
\begin{equation}
\mathbb{E}[\widehat{I}_{cv}]
  = \mathbb{E}[\widehat{I}_{XY}]
  + \beta\big(\mathbb{E}[\widehat{I}_{EE}] - \mu_{EE}\big)
  = \mathbb{E}[\widehat{I}_{XY}].
\label{eq:expectation_invariance}
\end{equation}

This shows that the modification introduces a quantity that, on average, is null:
the expected value of the estimated bound does not change,
but the stochastic oscillations around it are reduced.

\subsubsection{Intuition}

Intuitively, $\widehat{I}_{EE}$ acts as an auxiliary signal that correlates with 
$\widehat{I}_{XY}$ through shared structural information (edges).
By subtracting its mean and weighting it with $\beta$, 
we introduce a control variate that cancels part of the variance 
of the primary estimator without altering its mean.
The next step is to analyze how this formulation 
reduces the variance of the mutual–information estimate, 
which is the core motivation for the new edge–map / edge–text contrastive loss.

\subsection{Computing the variance of the combined estimator}

We now focus on the variance of the estimator introduced in
Section~\ref{eq:control_variate}, which shows how the additional
edge--text alignment acts as a control variate and reduces the
variance of the mutual information estimate.

\subsubsection{Total variance}

The total variance of the combined estimator is
\begin{equation}
\mathrm{Var}[\widehat{I}_{cv}]
 = \mathrm{Var}[\widehat{I}_{XY}]
   + \beta^2\,\mathrm{Var}[\widehat{I}_{EE}]
   + 2\beta\,\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE}).
\label{eq:var_total}
\end{equation}
This is the standard formula for the variance of a sum of correlated
random variables.

\subsubsection{Optimal coefficient \texorpdfstring{$\beta^\star$}{beta*}}

To find the value of $\beta$ that minimizes the variance, we take the
derivative of~\eqref{eq:var_total} with respect to $\beta$ and set it
to zero:
\begin{equation}
\frac{d}{d\beta}\mathrm{Var}[\widehat{I}_{cv}]
 = 2\beta\,\mathrm{Var}[\widehat{I}_{EE}]
   + 2\,\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE}) = 0,
\end{equation}
which gives
\begin{equation}
\beta^\star
 = -\,\frac{\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE})}
         {\mathrm{Var}[\widehat{I}_{EE}]}.
\label{eq:beta_opt}
\end{equation}

\subsubsection{Verification of the minimum}

The second derivative is
\[
\frac{d^2}{d\beta^2}\mathrm{Var}[\widehat{I}_{cv}]
  = 2\,\mathrm{Var}[\widehat{I}_{EE}] > 0,
\]
confirming that Eq.~\eqref{eq:beta_opt} indeed minimizes the variance.

\subsubsection{Substitution of \texorpdfstring{$\beta^\star$}{beta*}}

Substituting Eq.~\eqref{eq:beta_opt} into
Eq.~\eqref{eq:var_total} yields
\begin{align}
\mathrm{Var}[\widehat{I}_{cv}]
 &= \mathrm{Var}[\widehat{I}_{XY}]
    + \left(-\frac{\mathrm{Cov}_{XY,EE}}{\mathrm{Var}_{EE}}\right)^2
       \mathrm{Var}_{EE}
    + 2\left(-\frac{\mathrm{Cov}_{XY,EE}}{\mathrm{Var}_{EE}}\right)
       \mathrm{Cov}_{XY,EE} \nonumber\\
 &= \mathrm{Var}[\widehat{I}_{XY}]
    - \frac{\mathrm{Cov}_{XY,EE}^2}{\mathrm{Var}_{EE}}.
\label{eq:var_substituted}
\end{align}

\subsubsection{Expression in terms of the correlation coefficient}

By definition of the correlation between the two estimators,
\begin{equation}
\rho = 
\frac{\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE})}
     {\sqrt{\mathrm{Var}[\widehat{I}_{XY}]\,\mathrm{Var}[\widehat{I}_{EE}]}}.
\label{eq:rho_def}
\end{equation}
Squaring Eq.~\eqref{eq:rho_def} gives
\begin{equation}
\mathrm{Cov}_{XY,EE}^2 = 
\rho^2\,\mathrm{Var}[\widehat{I}_{XY}]\,\mathrm{Var}[\widehat{I}_{EE}].
\label{eq:cov_rho}
\end{equation}
Substituting Eq.~\eqref{eq:cov_rho} into Eq.~\eqref{eq:var_substituted}
leads to the compact form
\begin{equation}
\mathrm{Var}[\widehat{I}_{cv}]
  = \mathrm{Var}[\widehat{I}_{XY}](1 - \rho^2).
\label{eq:var_final}
\end{equation}

\subsubsection{Intuitive interpretation}

The correlation $\rho$ measures how strongly the two estimates
$\widehat{I}_{XY}$ and $\widehat{I}_{EE}$ vary together.
\begin{itemize}
    \item If they are perfectly correlated ($\rho = \pm 1$),
          the variance can be completely eliminated (in theory).
    \item If they are independent ($\rho = 0$),
          the control variate has no effect and the variance remains unchanged.
\end{itemize}

Therefore, Eq.~\eqref{eq:var_final} shows that the control variate
always reduces the variance of the mutual information estimator by a
factor proportional to $1-\rho^2$, without changing its expected value.
\subsection{The idea of the control variate}

In statistics, when a quantity of interest is estimated through a noisy estimator 
(such as $\widehat{I}_{XY}$ for the image–text mutual information)
and another correlated but more stable quantity is available 
(such as $\widehat{I}_{EE}$ from edge–edge alignment),
the two can be linearly combined to produce a more precise estimate.
This technique is known as a \emph{control variate}.
It is commonly used in Monte Carlo simulations to reduce the variance of an estimator
without affecting its expectation.

\subsection{Connection with the bound formulation}
Yes, they are the estimates of I(X,Y) and I(X_E,Y_E).
% The lower bound of the InfoNCE loss is given by the paper \cite{math_lower_bound}. So here, the loss function L_clip + beta L_s-t aims to maximize the estimate the lower bound with (logN - L), 
After defining the loss, the paper states that both
$\mathcal{L}_{\text{CLIP}}$ and $\mathcal{L}_{s\text{–}t}$ 
act as (negative) estimators of the InfoNCE lower bound \SW{\cite{math_lower_bound}} on 
the mutual information between $(X, Y)$ and $(X_E, Y_E)$, respectively:
\begin{equation}
\widehat{I}_{XY} = \log N - \mathcal{L}_{\text{CLIP}},
\qquad
\widehat{I}_{EE} = \log N - \mathcal{L}_{s\text{–}t}.
\label{eq:bound_losses}
\end{equation}
Thus, as each loss decreases, the corresponding bound increases.

Substituting these estimators into the control-variate formulation
of Eq.~\eqref{eq:control_variate}, we obtain:
\begin{equation}
\widehat{I}_{cv}
 = (\log N - \mathcal{L}_{\text{CLIP}})
   + \beta\big[(\log N - \mathcal{L}_{s\text{–}t}) - \mu_{EE}\big].
\label{eq:cv_loss_bound}
\end{equation}

Since $\log N$ and $\mu_{EE}$ are constants with respect to optimization,
maximizing $\widehat{I}_{cv}$ (or equivalently minimizing its negative)
leads to the effective training loss:
\begin{equation}
\mathcal{L}_{\text{total}}
 = \mathcal{L}_{\text{CLIP}}
   + \beta\,\mathcal{L}_{s\text{–}t},
\label{eq:final_loss}
\end{equation}
which corresponds to the original formulation of the edge–RGB contrastive loss.
\todo[]{Beta here actually represents a physical meaning of (\ref{eq:beta_opt}). }
\subsection{Interpretation as a regularizer}
\SW{The total loss (\ref{eq:final_loss}) aims at maximizing the control-variate estimator (\ref{eq:control_variate}).} 

From Eq.~\eqref{eq:var_final}, the addition of the edge–text term reduces
the variance of the mutual-information estimate without altering its expected value.
Therefore, the auxiliary edge–RGB loss acts as a \emph{regularizer}:
it stabilizes the optimization of the main contrastive objective,
enforcing consistent structure–aware representations across modalities
while keeping the overall information content unchanged. 
\SW{This completes the proof of Theorem~\ref{thm:cve_for_mi}.}
\end{proof}


%% ===

% =================================================
\Section{(Deprecated) Theorem 2}
\begin{equation}
\begin{aligned}
\mathcal{L}_{ours} = \mathcal{L}_{CLIP} + \beta \mathcal{L}_{s-t} + \gamma \mathcal{L}_{rs} + \sigma \mathcal{L}_{chunk}.
\label{eq:loss}
\end{aligned}
\end{equation}

Since CLIP doesn't perform well due to the lack of structural information, we introduce additional design terms to better align structural information across modalities. 

Specifically, the scribble–text contrastive loss aims to maximize the mutual information I(S,E) between the scribble and edge representations, which captures the structural sub-information of the original image–text mutual information I(I,T). 

Due to the Data Processing Inequality, any additional processing of the source image-text cannot increase the amount of mutual information: 
\begin{equation}
\begin{aligned}
I(S,E) \leq I(I,T).
\end{aligned}
\end{equation}
Although I(S,E) cannot exceed I(I,T), it captures a more stable and noise-insensitive component of the joint dependency between the visual and textual domains—particularly those corresponding to geometry, contours, and layout. In addition, we rigorously demonstrate that our approach achieves a statistically tighter and more stable lower bound on $I(I,T)$ than CLIP: 

Assume that after sufficient optimization, $\hat{I}_{CLIP}$ and $\hat{I}_{s-t}$ act as approximately unbiased estimators of the lower bound of the mutual information $I_{LB}(I,T)$ and $I_{LB}(S,E)$ \cite{math_lower_bound}, respectively:
\begin{equation}
\begin{aligned}
\mathbb{E}[\hat{I}_{{CLIP}}] &= \log N - \mathcal{L}_{CLIP} = I_{\mathrm{LB}}(I,T), \\
\mathbb{E}[\hat{I}_{{s-t}}] &= \log N - \mathcal{L}_{s-t} = I_{\mathrm{LB}}(S,E),     
\end{aligned}
\end{equation}
Assume that the original image-text pair and the scribble-edge pair are not perfectly correlated.

The loss function $\mathcal{L}_{CLIP} + \beta \mathcal{L}_{s-t}$ estimates the mutual information I(I,T) by:
\begin{equation}
\begin{aligned}
\hat{I}_{ours} = \hat{I}_{CLIP} + \beta (\hat{I}_{s-t} - \mathbb{E}[\hat{I}_{{s-t}}]). 
\end{aligned}
\end{equation}
The variations is given by:
\begin{equation}
\begin{aligned}
\text{Var}[\hat I_{ours}] = \text{Var} [\hat{I}_{CLIP}]  + \beta^2 \text{Var} (\hat{I}_{s-t}) + 2 \beta \text{Cov}[\hat{I}_{CLIP},\hat{I}_{s-t}],
\end{aligned}
\end{equation}

with $\beta^*= \textcolor{red}{-} \frac{\text{Cov}[\hat{I}_{CLIP},\hat{I}_{s-t}]}{ \text{Var} (\hat{I}_{s-t})}$: 
\begin{equation}
\begin{aligned}
\text{Var}[\hat I_{ours}] = \text{Var} [\hat{I}_{CLIP}] (1- \rho^2), 
\end{aligned}
\end{equation}
where $\rho = Corr[\hat{I}_{CLIP}, \hat{I}_{s-t}]$. 
Hence, whenever $|\rho| \in [0,1]$, variance of $\hat I_{ours}$ is reduced. 

Finally, because InfoNCE provides an unbiased stochastic lower-bound estimator,
Chebyshev’s inequality gives:
\begin{equation}
\begin{aligned}
\mathbb{P}\!\left( \left| \hat{I}^\star_{ours} - \mathbb{E}\!\left[\hat{I}^\star_{ours}\right] \right| \geq \varepsilon \right)
\leq 
\frac{\mathrm{Var}\!\left[\hat{I}^\star_{ours}\right]}{\varepsilon^2}
= 
\frac{\sigma_c^2 (1 - \rho^2)}{\varepsilon^2}.
\end{aligned}
\end{equation}

Relative to the CLIP, the deviation bound shrinks by the factor of $(1-\rho^2)$. Thus, the empirical mutual information bound becomes statistically tighter. 

Similarly, the introduction of chunk-patch alignments further shrinks the empirical mutual information bound by: 
\begin{equation}
\begin{aligned}
\text{Var}[\hat I_{ours}] = \text{Var} [\hat{I}_{CLIP}] (1- \rho_{s-t}^2)(1-\rho_{chunk}^2), 
\end{aligned}
\end{equation}
To further enhance the structural alignment between the original image and its scribble counterpart, $\mathcal{L}{rs}$
enforces feature-level similarity between the image and its scribble representation. Although $\mathcal{L}_{rs}$ does not explicitly appear in the variance minimization formulation, it implicitly affects the covariance structure between $\hat{I}_{CLIP}$ and $\hat{I}_{s-t}$. By aligning the latent distributions of image and scribble features, $\mathcal{L}_{rs}$ increases their statistical correlation $\rho$, thereby further reducing the joint variance term $\mathrm{Var}[\hat I_{ours}] = \mathrm{Var}[\hat I_{CLIP}](1 - \rho^2)$. Consequently, this auxiliary reconstruction term reinforces the stability and tightness of the mutual information bound.

==> sec/3bis_workshop.tex <==
\section{Theoretical proof 1118 - MARCO}

\paragraph{Theoretical analysis.}
We analyze the effect of the structure-centric objectives
$\mathcal{L}_{I',T'}$ and $\mathcal{L}_{I,I'}$ under an information-theoretic
and optimization lens.

\begin{lemma}[Information ordering for structure-centric views]
Let $I$ and $T$ denote the random variables associated with images and texts,
and let $I' = \mathcal{E}(I)$ and $T' = \mathcal{F}(T)$ be their structure-centric counterparts,
where $\mathcal{E}(\cdot)$ and $\mathcal{F}(\cdot)$ are deterministic maps that remove
appearance-related information and are not invertible.
Then the following inequality holds:
\[
I_{\mathrm{MI}}(I',T') < I_{\mathrm{MI}}(I,T),
\]
where $I_{\mathrm{MI}}(\cdot,\cdot)$ is the mutual information operator.
\end{lemma}

\noindent\textit{Proof sketch.}
The pair $(I',T')$ is obtained from $(I,T)$ through the
deterministic channel $(\mathcal{E},\mathcal{F})$. By the Data Processing Inequality~\cite{tishby99information},
any such transformation cannot increase mutual information, hence
$ I_{\mathrm{MI}}(I',T') \le I_{\mathrm{MI}}(I,T) $.
The inequality is strict whenever either $E$ or $F$ is not injective,
which holds in our setting since edge extraction and lexicon filtering
discard appearance cues.

\medskip

\begin{lemma}[InfoNCE lower bounds for the two objectives]
Let $\imagefeat = \visualencoder(I)$ and $\textfeat = \textencoder(T)$ be the image and
text embeddings, and let $\imagefeat' = \visualencoder(I')$ and
$\textfeat' = \textencoder(T')$ be the structure-centric embeddings.
Assume both $\mathcal{L}_{I,T}$ and $\mathcal{L}_{I',T'}$ are symmetric
InfoNCE losses with batch size $N$. Then
\[
I_{\mathrm{MI}}(\imagefeat,\textfeat) \ge \log N - \mathbb{E}[\mathcal{L}_{I,T}],\quad
I_{\mathrm{MI}}(\imagefeat',\textfeat') \ge \log N - \mathbb{E}[\mathcal{L}_{I',T'}].
\]
\end{lemma}

\noindent\textit{Proof.}
This is the mere application of~\cite{poole2019variational}, stating that the InfoNCE loss is a standard variational lower bound on mutual information.
Applying the result to the pairs $(\imagefeat,\textfeat)$ and $(\imagefeat',\textfeat')$ yields the two
inequalities. The assumptions on symmetry and batch size match the
formulation in Sec. 3.2 of the main paper. In the following, to the sake of clarity, we assume $I_{\mathrm{MI}}(\imagefeat,\textfeat)\approx I_{\mathrm{MI}}(I,T) $ and $I_{\mathrm{MI}}(\imagefeat',\textfeat')\approx I_{\mathrm{MI}}(I',T') $.

\medskip

\begin{lemma}[Directional compatibility of gradients]
Let $\theta$ denote the parameters shared by the vision and text encoders.
Consider the gradients $\nabla_{\theta}\mathcal{L}_{I,T}$ and
$\nabla_{\theta}\mathcal{L}_{I',T'}$.
If the positive pairs in the two losses correspond to the same image–text
instances and the encoders are shared, then the expected cosine similarity
between the two gradients satisfies
\[
\mathbb{E}\big[\cos(\nabla_{\theta}\mathcal{L}_{I,T},
\nabla_{\theta}\mathcal{L}_{I',T'})\big] > 0.
\]
\end{lemma}

\noindent\textit{Proof sketch.}
Both losses use the same positive pairs and differ only in the views
fed to the encoders (full images and captions vs structure-centric
counterparts). The corresponding positive logits are maximized in
both objectives, while negatives are pushed apart.
This induces aligned update directions for parameters that affect
shared features. Under mild regularity assumptions on the encoders,
the expected cosine similarity between the two gradients is strictly
positive. In practice, this is confirmed by the empirical measurements
reported in Fig. 4(c).

\medskip

\begin{theorem}[Effect of the structure-centric auxiliary losses]
Consider the joint objective
\[
\mathcal{L}_{\mathrm{total}} = \mathcal{L}_{I,T}
+ \lambda_{1}\mathcal{L}_{I',T'} + \lambda_{2}\mathcal{L}_{I,I'},
\quad \lambda_{1},\lambda_{2} > 0.
\]
Under the assumptions of the lemmas above, the following properties hold:
\begin{enumerate}
\item The auxiliary alignment task between the pair $(\imagefeat',\textfeat')$ is information-reduced
compared to $(\imagefeat,\textfeat)$, hence $\mathcal{L}_{I',T'}$ optimizes a
harder objective in the sense of Lemma 1 and 2.
\item The gradients of $\mathcal{L}_{I,T}$ and $\mathcal{L}_{I',T'}$
are directionally compatible, so the auxiliary loss does not
conflict with the main alignment.
\item Due to the lower mutual information of $(\imagefeat',\textfeat')$,
the gradient norm of $\nabla_{\theta}\mathcal{L}_{I',T'}$
remains non-negligible even when $\nabla_{\theta}\mathcal{L}_{I,T}$
starts to vanish, which provides persistent optimization signal.
\item The consistency term $\mathcal{L}_{I,I'}$ bounds the drift
between $\imagefeat$ and $\imagefeat'$, so the structure-centric space stays
anchored to the semantic manifold of $\imagefeat$ and training remains stable.
\end{enumerate}
\end{theorem}

\noindent\textit{Proof sketch.}

\textbf{Item 1} follows directly from Lemma 1 and the InfoNCE bounds in Lemma 2,
which place the pair $(\imagefeat',\textfeat')$ at a lower mutual information level than $(\imagefeat,\textfeat)$.
More in the detail, the auxiliary alignment task on $(\imagefeat',\textfeat')$ is strictly information-reduced compared to
$(\imagefeat,\textfeat)$, and therefore $\mathcal{L}_{I',T'}$ optimizes a harder objective.
More precisely, since $I' = \mathcal{E}(I)$ and $T' = \mathcal{F}(T)$ are obtained by applying
non-invertible, deterministic maps that remove appearance-related variability,
the entropy of both variables is reduced:
\[
H(I') < H(I), \qquad H(T') < H(T).
\]
By the Data Processing Inequality, this implies
\[
I_{\mathrm{MI}}(I',T') \le I_{\mathrm{MI}}(I,T).
\]
In addition, the structure-centric views induce a contraction of the positive
pair distribution: the space of valid matches becomes smaller, the intra-class
variability is suppressed, and the negative samples become less separable in
the embedding space. These effects lower the effective signal-to-noise ratio
of the InfoNCE objective, which increases the difficulty of the optimization
landscape associated with $\mathcal{L}_{I',T'}$.
Consequently, the gradients generated by $\mathcal{L}_{I',T'}$ tend to persist
longer during training, since reaching its minimum requires modeling more
subtle, geometry-driven correspondences that remain unresolved after the
full-information objective $\mathcal{L}_{I,T}$ has already saturated.


\textbf{Item 2} follows from Lemma~3 and concerns the directional
compatibility of the gradients.  
Since both $\mathcal{L}_{I,T}$ and $\mathcal{L}_{I',T'}$ operate on the same
positive image–text instances and update the same encoder parameters,
their contrastive objectives induce aligned update rules:  
both maximize the positive logit and suppress the negative logits
associated with the same underlying pairs, even though the views differ.
Let the gradients be:  
\[
g = \nabla_{\theta}\mathcal{L}_{I,T}, \qquad
g' = \nabla_{\theta}\mathcal{L}_{I',T'}.
\]
Lemma~3 ensures that their expected cosine similarity satisfies  
\[
\mathbb{E}\big[\cos(g,g')\big] > 0.
\]
Therefore, the auxiliary gradient does not conflict with the semantic
direction promoted by the main loss.  
Instead, it expands the set of admissible descent directions within a
compatibility cone, enriching the optimization trajectory without
introducing destructive interference.


\textbf{Item 3} relies on the fact that, owing to the information-reduced nature of $(I',T')$,
the loss $\mathcal{L}_{I',T'}$ converges more slowly than
$\mathcal{L}_{I,T}$ and produces non-vanishing gradients
even when the main loss has already flattened.
%
Indeed, $\mathcal{L}_{I,T}$ optimizes an InfoNCE objective
associated with the higher mutual information quantity
$I_{\mathrm{MI}}(I,T)$, whose landscape typically admits a
faster descent: the positive pair $(\imagefeat,\textfeat)$ carries rich
appearance and structural cues, which help discriminate
positives from negatives early in training.
%
In contrast, $\mathcal{L}_{I',T'}$ maximizes the lower
$I_{\mathrm{MI}}(I',T')$, where both $\imagefeat'$ and $\textfeat'$ have reduced
entropy because appearance information has been removed by
$\mathcal{E}(\cdot)$ and $\mathcal{F}(\cdot)$.  This contraction of the feature
space has two effects:
\begin{itemize}
\item the separation between positives and negatives becomes
smaller, making the contrastive objective harder to optimize;

\item the gradients associated with hard positives and hard
negatives decay more slowly, since the model must rely purely
on geometric and structural cues to improve the logits.
\end{itemize}
Formally, since the InfoNCE gradients satisfy
\[
\nabla_{\theta}\mathcal{L}_{I,T}
= \mathbb{E}\big[g(\imagefeat,\textfeat)\big],\qquad
\nabla_{\theta}\mathcal{L}_{I',T'}
= \mathbb{E}\big[g(\imagefeat',\textfeat')\big],
\]
and the score function $g(\cdot)$ for $(\imagefeat',\textfeat')$ has larger
relative variance due to the reduced mutual information,
the expected magnitude of $\nabla_{\theta}\mathcal{L}_{I',T'}$
remains positive for a longer portion of training.
%
Empirically, this manifests in a later convergence time for
$\mathcal{L}_{I',T'}$ compared to $\mathcal{L}_{I,T}$, and in a
sustained gradient norm that continues to provide meaningful
updates even after the main contrastive gradients approach
zero.  This behaviour is consistent with the dynamics shown
in Fig.~4(a,b), where $\mathcal{L}_{I',T'}$ displays a slower
flattening and a more persistent gradient profile.


Finally, \textbf{Item 4} exploits the form of $\mathcal{L}_{I,I'}$, which penalizes large
angular deviations between $\imagefeat$ and $\imagefeat'$ and therefore constrains
the structure-centric representations to remain close to their
full-information counterparts.
Specifically, since $\mathcal{L}_{I,T}$ and $\mathcal{L}_{I',T'}$ correspond to two
correlated but not identical contrastive objectives, their
gradients span a larger subspace than either loss alone.  
Formally, let
\[
g = \nabla_{\theta}\mathcal{L}_{I,T}, \qquad
g' = \nabla_{\theta}\mathcal{L}_{I',T'}.
\]
From Item 2 we know that $\cos(g,g')>0$ in expectation,
which guarantees compatibility.  However, because
$(\imagefeat',\textfeat')$ belongs to an information-reduced space and
responds differently to hard negatives and subtle geometric
patterns, one has
\[
g' \notin \mathrm{span}\{g\},
\]
so the matrix $[g,\;g']$ has rank $2$ almost everywhere.
This implies that the combined update
\[
g_{\mathrm{tot}}
= g + \lambda_{1}g' + \lambda_{2}\nabla_{\theta}\mathcal{L}_{I,I'}
\]
explores descent directions that the main loss alone cannot
access. This additional set of directions reduces the risk of
premature convergence to shallow minima (a common issue
in contrastive objectives), improves escape from flat regions
of the loss surface, and increases the robustness of SGD
trajectories.  In the language of multi-objective optimization,
$\mathcal{L}_{I',T'}$ introduces a complementary gradient
component that expands the effective feasible region of
updates while maintaining alignment with the main semantic
objective. The consistency loss $\mathcal{L}_{I,I'}$ ensures that this
expanded search space remains stable by preventing $\imagefeat'$ from
drifting too far from $\imagefeat$.  As a result, the combined gradient
retains diversity without diverging from the semantic
manifold defined by the original embeddings, yielding a
balanced and stable optimization process.


Taken together, these properties explain why the auxiliary
structure-centric alignment acts as a beneficial regularizer:
it introduces correlated but information-reduced gradients that
improve convergence stability and lead to more robust alignment.



\\
\section{Theoretical proof 1106 - MARCO}
Given the broad applicability and strong empirical performance of StructXLIP, it is natural to investigate its underlying theoretical properties. From an information--theoretic view, the goal is to maximize the mutual information $I(I,T)$. We can assume that $\structextractor(\cdot)$ and $\mathcal{F}(\cdot,\cdot)$ are deterministic functions that extract $I'$ and $T'$, respectively. In terms of representational complexity, $I'$ and $T'$ are simplified versions of $I$ and $T$, as they have a smaller effective vocabulary: 
$I'$ is a binary $\{0,1\}$ edge map, while $T'$ omits any word expressing chromaticity.
Therefore, the Data Processing Inequality (DPI)~\cite{tishby99information} implies that
\[
I(I',T') \le I(I,T).
\] 
Here, the mutual information $I(I,T)$ is estimated through the lower bound 
$\log(N) - \mathcal{L}_{\text{org}}$, while $I(I',T')$ is estimated by 
$\log(N) - \mathcal{L}_{\text{ST}}$, with $N$ denoting the batch size. (experimentally, we observed...).
In addition, we observed that the gradients of the two losses have similar orientation.
Thereofre we may say that the two problems of maximization of mutual information are correlated, and the one with scarcer information is harder to solve, since it has less data to work with. 
DUe to this fact, the $\mathcal{L}_{\text{ST}}$ saturates to $log(N)$ later than $\mathcal{L}_{\text{org}$. Therefore, the effct of the second loss is that of pulling the optimization to better setup in the parameter space. 





the auxiliary term $\mathcal{L}_{\text{ST}}$ acts on surrogated representations 
$X_E=f(X)$ and $Y_E=g(Y)$ that retain structural but not chromatic cues. 
By the Data Processing Inequality (DPI), these views satisfy $I(X_E;Y_E)\le I(X;Y)$, 
and both mutual informations admit InfoNCE lower bounds 
$I(\cdot)\ge \log N - \mathbb{E}[\mathcal{L}(\cdot)]$.


\section{Theoretical proof 1102 - MARCO}
\section{Why it is working - work with our friend}
\paragraph{Theoretical insight.}
From an information--theoretic view, the auxiliary term $\mathcal{L}_{\text{ST}}$ acts on compressed representations 
$X_E=f(X)$ and $Y_E=g(Y)$ that retain structural but not chromatic cues. 
By the Data Processing Inequality (DPI), these views satisfy $I(X_E;Y_E)\le I(X;Y)$, 
and both mutual informations admit InfoNCE lower bounds 
$I(\cdot)\ge \log N - \mathbb{E}[\mathcal{L}(\cdot)]$. 
When the main contrastive bound $I(X;Y)$ saturates, its gradient weakens, 
whereas the auxiliary bound remains active because of its reduced entropy. 
Consequently, the auxiliary gradient $g_a=\nabla_\theta\mathcal{L}_{\text{ST}}$ 
provides a non-vanishing, correlated signal that reinforces the main gradient 
$g_0=\nabla_\theta\mathcal{L}_{\text{org}}$.

From an optimization perspective, the total gradient $g(\lambda)=g_0+\lambda g_a$ 
can be decomposed into mean and stochastic components 
$g=\mu+\varepsilon$. 
Under mild task alignment ($\langle\mu_0,\mu_a\rangle>0$) and 
negative covariance of the noise terms, 
the orthogonal variance of $g(\lambda)$ 
is minimized for a small $\lambda>0$. 
This yields two practical effects: (i)~a reorientation of the descent direction toward 
the true semantic optimum (bias shifting), and 
(ii)~a reduction of orthogonal gradient noise (variance reduction).
Empirically, this explains the smoother loss curves 
and the more stable convergence observed when training with the auxiliary 
edge--text objective.
\paragraph{Theoretical analysis EXPANDED FOR THE ADDITIONAL MATERIAL.}
We analyze our framework under an information--theoretic and optimization lens. 
Let $X$ and $Y$ denote the image and text representations, and let 
$X_E=f(X)$, $Y_E=g(Y)$ be deterministic functions which extract edges and text related to structural properties of the image, respectively. In particular, $f$ and $g$ reduce the size of the vocabulary of the representations, being the edges represented by ${0,1}$ pixel values and the structural text deprived from terms related to chromaticity.  
Since $f,g$ reduce representational entropy, the Data Processing Inequality (DPI) gives
\[
I(X_E;Y_E)\le I(X;Y).
\]
Both mutual informations are estimated through InfoNCE lower bounds:
\[
I(X;Y)\ge \log N - \mathbb{E}[\mathcal{L}_{\text{org}}], \qquad
I(X_E;Y_E)\ge \log N - \mathbb{E}[\mathcal{L}_{\text{ST}}],
\]
where $N$ is the batch size.

\paragraph{Assumptions.}
\begin{itemize}
\item[(A1)] $f,g$ are deterministic and entropy-reducing: $H(X_E)\!<\!H(X)$, $H(Y_E)\!<\!H(Y)$.
\item[(A2)] InfoNCE lower bounds are valid under consistent critics and i.i.d.\ negative sampling~\cite{tschannen2020mutual}.
\item[(A3)] For model parameters $\theta$, denote $g_0=\nabla_\theta \mathcal{L}_{\text{org}}$, 
$g_a=\nabla_\theta \mathcal{L}_{\text{ST}}$, with mean--noise decompositions
$g_0=\mu_0+\varepsilon_0$, $g_a=\mu_a+\varepsilon_a$, where $\mathbb{E}[\varepsilon_\cdot]=0$ 
and all expectations are conditional on $\theta$.
\item[(A4)] Positive task affinity:
\[
\langle \mu_0,\mu_a\rangle > 0, 
\quad 
\text{and}\quad 
\mathrm{tr}\!\big(P_\perp\,\mathrm{Cov}(\varepsilon_0,\varepsilon_a)\,P_\perp\big)<0,
\]
where $P_\perp=I-uu^\top$ projects orthogonally to $u=\mu_0/\|\mu_0\|$.
\item[(A5)] Non-saturation of the auxiliary bound:
there exists $\delta>0$ such that 
$\log N-\mathbb{E}[\mathcal{L}_{\text{ST}}]\le \log N-\delta$ even when 
$I(X;Y)\!\approx\!\log N$. Hence $\|\mu_a\|\!>\!0$ when $\|\mu_0\|\!\to\!0$.
\end{itemize}

\begin{remark}[On (A1)]
The mappings $f,g$ correspond to edge extraction or structural filtering. 
They are deterministic and reduce the representational vocabulary, thus entropy. 
Strict DPI ensures $I(X_E;Y_E)\!<\!I(X;Y)$ unless $f,g$ are invertible.
\end{remark}

\begin{remark}[On (A2)]
The InfoNCE lower bound is unbiased if negative samples are drawn from the marginal and the critic is consistent. 
This assumption aligns with standard analyses in contrastive learning (e.g.~\cite{tschannen2020mutual}).
\end{remark}

\begin{remark}[On (A3)]
The gradient decomposition $g=\mu+\varepsilon$ is standard in stochastic optimization. 
$\mu$ represents the population gradient, $\varepsilon$ the per-batch fluctuation. 
All subsequent variance and covariance terms refer to these batch-induced fluctuations at fixed $\theta$.
\end{remark}

\begin{remark}[On (A4)]
The first condition $\langle \mu_0,\mu_a\rangle>0$ expresses \emph{task alignment}: both gradients point, on average, toward semantically consistent optima.
The second condition assumes negative covariance between orthogonal noise components, i.e.\ $\varepsilon_a$ tends to cancel $\varepsilon_0$ outside the target subspace. 
This can be empirically verified by estimating $\mathrm{tr}(P_\perp\,\widehat{\mathrm{Cov}}(g_0,g_a)\,P_\perp)$ over mini-batches.
\end{remark}

\begin{remark}[On (A5)]
When the main InfoNCE saturates, its gradient vanishes. 
However, since $I(X_E;Y_E)\!<\!I(X;Y)$, the auxiliary bound is less saturated and continues to generate nonzero gradients, providing a regularizing signal.
\end{remark}

\begin{lemma}[Active auxiliary bound]
Under (A1)--(A2)--(A5), when the main InfoNCE bound saturates 
($I(X;Y)\!\approx\!\log N$), the compressed bound remains non-saturated.
Thus, the auxiliary gradient $\mu_a$ provides a non-vanishing signal when 
$\mu_0$ weakens, maintaining informative pressure on the alignment of $(X_E,Y_E)$.
\end{lemma}

\begin{lemma}[Orthogonal noise minimization]
Let $g(\lambda)=g_0+\lambda g_a$ with $\lambda\ge 0$. 
Define the orthogonal variance
\[
\sigma_\perp^2(\lambda)=
\mathrm{tr}\!\big(P_\perp\,\mathrm{Var}[g(\lambda)]\,P_\perp\big)
= a\lambda^2 + 2b\lambda + c,
\]
where
\[
a=\mathrm{tr}(P_\perp\,\mathrm{Var}[g_a]\,P_\perp)\ge 0,\quad
b=\mathrm{tr}(P_\perp\,\mathrm{Cov}(g_0,g_a)\,P_\perp),\quad
c=\mathrm{tr}(P_\perp\,\mathrm{Var}[g_0]\,P_\perp).
\]
If (A4) holds, then $b<0$, and the minimum is attained at 
$\lambda_\perp^*=-b/a>0$, yielding 
$\sigma_\perp^2(g(\lambda_\perp^*))<\sigma_\perp^2(g_0)$.
\end{lemma}

\begin{remark}[Interpretation]
The auxiliary gradient acts as a correlated control variate: adding a small multiple $\lambda g_a$ reduces the stochastic variance of $g_0$ in the subspace orthogonal to its mean direction.
\end{remark}

\begin{proposition}[Improved alignment and noise reduction]
Let $g^*=\nabla_\theta \mathcal{L}_{\text{org}}^{\text{pop}}$ be the population gradient 
of the main objective, and assume local $L$-smoothness. 
Under (A1)--(A5), there exists $\lambda\in(0,\lambda_{\max}]$ such that:
\begin{enumerate}[(i)]
\item Alignment improvement:
$\cos(\mathbb{E}[g(\lambda)],g^*)>\cos(\mu_0,g^*)$.
\item Orthogonal variance reduction:
$\sigma_\perp^2(g(\lambda))<\sigma_\perp^2(g_0)$.
\item Expected descent improvement:
\[
\mathbb{E}[\Delta\mathcal{L}_{\text{org}}]
\le 
-\eta\,\langle g^*,\mathbb{E}[g(\lambda)]\rangle
+ \tfrac{L\eta^2}{2}\,\mathbb{E}[\|g(\lambda)\|^2],
\]
so that, for sufficiently small $\eta$, the expected loss decrement per iteration is larger than with $\lambda=0$.
\end{enumerate}
\end{proposition}

\begin{proof}[Sketch]
(i) follows from $\langle \mu_0,\mu_a\rangle>0$, which guarantees that a small $\lambda>0$ increases 
alignment with $g^*$.  
(ii) follows from Lemma~2 and $b<0$.  
(iii) follows from the $L$-smoothness inequality above.  
In the small-noise regime, 
$\mathbb{E}[\cos(g(\lambda),g^*)]\!\approx\!1-\sigma_\perp^2(\lambda)/(2\|g^*\|^2)$,
so decreasing $\sigma_\perp^2$ yields higher expected alignment and stronger descent.
\end{proof}

\begin{remark}[On smoothness]
The inequality used in (iii) is standard in stochastic gradient theory:
for an $L$-smooth objective,
\[
\mathbb{E}[\mathcal{L}(\theta_{t+1})-\mathcal{L}(\theta_t)] 
\le -\eta\,\langle g^*,\mathbb{E}[g]\rangle 
+ \tfrac{L\eta^2}{2}\,\mathbb{E}[\|g\|^2].
\]
This links alignment and noise reduction directly to expected improvement.
\end{remark}

\begin{corollary}[Variance decomposition]
The per-batch variance of the combined loss is
\[
\mathrm{Var}(\mathcal{L}_{\text{org}}+\lambda\mathcal{L}_{\text{ST}})
=\mathrm{Var}(\mathcal{L}_{\text{org}})+\lambda^2\mathrm{Var}(\mathcal{L}_{\text{ST}})
+2\lambda\,\mathrm{Cov}(\mathcal{L}_{\text{org}},\mathcal{L}_{\text{ST}}).
\]
Even if this total variance grows, Lemma~2 guarantees that the variance of the 
\emph{main gradient component orthogonal to its target direction} decreases,
explaining empirically why $\mathcal{L}_{\text{org}}$ appears smoother when optimized jointly with $\mathcal{L}_{\text{ST}}$.
\end{corollary}

\begin{remark}[Practical verification]
In practice, one can estimate
\[
\widehat b = 
\mathrm{tr}(P_\perp\,\widehat{\mathrm{Cov}}(g_0,g_a)\,P_\perp)
\quad\text{and}\quad
\widehat\sigma_\perp^2(\lambda)
= \mathrm{tr}(P_\perp\,\widehat{\mathrm{Var}}[g(\lambda)]\,P_\perp),
\]
on mini-batch windows. 
If $\widehat b<0$ and $\widehat\sigma_\perp^2(\lambda_\perp^*)<\widehat\sigma_\perp^2(0)$, 
the assumptions are empirically satisfied.
\end{remark}

\paragraph{Interpretation.}
The auxiliary InfoNCE term on $(X_E,Y_E)$ acts as a 
\emph{bias-shifting regularizer}: it provides a correlated gradient $\mu_a$ 
that reorients the descent direction toward the true semantic optimum $g^*$ 
while canceling orthogonal stochastic noise. 
This produces a more stable and semantically consistent alignment 
between visual and textual modalities.
\\ \\
\section{Theoretical proof 1028 - MARCO}
\section{Why it is working}
To analyze the theoretical properties of our approach, we adopt an information--theoretic perspective. 
Our goal is to maximize the mutual information $I(X,Y)$, where $X$ denotes the image representation and $Y$ the textual representation of a common semantic concept $Z$. 
Let $f$ and $g$ be deterministic functions that extract from $X$ the edge representation $X_E$, and from $Y$ the textual description of structural properties $Y_E$. 
In terms of representational complexity, $X_E$ and $Y_E$ are simplified versions of $X$ and $Y$, as they have a smaller effective vocabulary: 
$X_E$ is a binary $\{0,1\}$ edge map, while $Y_E$ omits any word expressing chromaticity. 
Since $f$ and $g$ are deterministic transformations, the Data Processing Inequality (DPI) implies that
\[
I(X_E, Y_E) \le I(X, Y).
\] 
In our loss formulation of Eq.~(14) (main paper),
\begin{align}
\mathcal{L}_{\mathrm{ours}}
&= \beta\,\mathcal{L}_{\text{org}}
+ \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}
+ \lambda_{\text{RS}}(t)\,\mathcal{L}_{\text{RS}}
+ \lambda_{\text{CK}}(t)\,\mathcal{L}_{\text{chunk}},
\label{eq:ourloss}
\end{align}
the mutual information $I(X,Y)$ is estimated through the lower bound 
$\log(N) - \mathcal{L}_{\text{org}}$, while $I(X_E,Y_E)$ is estimated by 
$\log(N) - \mathcal{L}_{\text{ST}}$, with $N$ denoting the batch size. 
Empirically, we observed that the variance of $\mathcal{L}_{\text{org}}$ 
(computed as the variance of its values over the training iterations) 
is smaller when it is optimized within $\mathcal{L}_{\mathrm{ours}}$ 
than when it is minimized alone. 
Furthermore, the gradients of $\mathcal{L}_{\text{org}}$ and $\mathcal{L}_{\text{ST}}$ 
are positively correlated, exhibiting a high cosine similarity.
The positive gradient correlation indicates that the auxiliary loss operates on a subspace of the same semantic dependency between images and texts. 
Although $I(X_E, Y_E)$ is lower than $I(X, Y)$, it captures the most stable and strongly shared information---edges and structural descriptions---thus acting as an \emph{information bottleneck} that filters nuisance variability such as color, texture, or lexical noise. 
Optimizing both losses jointly therefore injects a low-variance, semantically consistent gradient into the main optimization. 
This explains why the variance of $\mathcal{L}_{\text{org}}$ decreases when it is trained within $\mathcal{L}_{\mathrm{ours}}$: the auxiliary term regularizes the optimization by aligning updates with the stable information shared by both modalities. 
At the same time, the total loss may show higher variance because it aggregates multiple stochastic sources. 
Overall, the auxiliary InfoNCE term on $(X_E,Y_E)$ acts as a \emph{bias-shifting regularizer}: it slightly increases the stochasticity of the total objective while shifting the mean gradient toward the true semantic direction that maximizes $I(X,Y)$. 
This leads to a more reliable and semantically grounded alignment between the image and text representations.





\\
\\

STOP HERE



In this section, we formally demonstrate that incorporating disentangled visual and textual information into the alignment process yields measurable benefits. Although this paper focuses on edge information, the proposed approach and its proof are general and apply to any type of disentangled information.

We begin with the overall loss defined in Eq.~(14) (main paper):
\begin{align}
\mathcal{L_{\mathrm{ours}}}
&= \beta\,\mathcal{L}_{\text{org}}
+ \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}
+ \lambda_{\text{RS}}(t)\,\mathcal{L}_{\text{RS}}
+ \lambda_{\text{CK}}(t)\,\mathcal{L}_{\text{chunk}}.
\end{align}\label{eq:ourloss}
For clarity, we initially focus on the first two components, 
$\beta\,\mathcal{L}_{\text{org}} + \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}$, while temporarily disregarding the constant weight $\beta$ and the time-dependent factor $\lambda_{\text{ST}}(t)$.  
This simplifies the expression to: 
\begin{equation}
\mathcal{L_{\mathrm{ours}}}\simeq \mathcal{L}_{\text{org}} + \mathcal{L}_{\text{ST}}.
\end{equation}\label{eq:shortloss}
The remaining terms will be examined later.

For the sake of clarity, we rename $\mathcal{L}_{\mathrm{org}}\rightarrow \mathcal{L}_{XY}$ to highlight we are dealing with the alignment of the two domains $X$ and $Y$, and $\mathcal{L}_{ST}\rightarrow \mathcal{L}_{{X_E}{Y_E}}$ to highlight that we are disentangling from the original domains an \emph{extraction} ($E$). In our case, $X_E$ is the edge image and $Y_E$ the edge oriented text, which are extracted from the RGB image $X$ and initial text $Y$, respectively. 

The benefit of adding disentangled information can be better analyzed considering the information theory. From~\cite{math_lower_bound}, contrastive losses can be interpreted as the negative of a lower bound on the mutual information estimator $\widehat{I}$, that is, $\widehat{I}=\log N - \mathcal{L}$; in our case this brings to:
\begin{align}
\widehat{I}_{XY} &= \log N - \mathcal{L}_{\text{XY}}\\
\widehat{I}_{EE} &= \log N - \mathcal{L}_{{X_E}{Y_E}}.
\label{eq:bound_losses}
\end{align}
where $N$ is the size of the batch, which is equal for both the losses. In Eq.(\ref{eq:shortloss}) the two losses are summed together, 
so we will do with their information theoretic counterpart, obtaining:
\begin{equation}
2\log N-(\widehat{I}_{XY}+\widehat{I}_{{X_E}{Y_E}})=\mathcal{L}_{XY}+\mathcal{L}_{{X_E}{Y_E}}
\end{equation}\label{eq:oursMI}
It is evident that minimizing the losses of Eq.~(\ref{eq:shortloss}) corresponds to maximizing the lower bound estimates of the mutual information terms $\widehat{I}_{XY}+\widehat{I}_{{X_E}{Y_E}}$. Two observations could be assessed from Eq.~(\ref{eq:oursMI}): 
actually, we can demonstrate (see the additional material) that $\widehat{I}_{{X_E}{Y_E}}\leq \widehat{I}_{XY}$  and that $\widehat{I}_{{X_E}{Y_E}}$ does not add any new information in the system, but is a specification of the information managed by the more general $\widehat{I}_{XY}$. Technically this means: $I\big( (X, X_E) ; (Y, Y_E) \big) = I(X; Y)$.  The proofs exploit the fact that we have stochastic functions with independent noise $X_E = f(X,\eta_X),Y_E = g(Y,\eta_Y)$ and use the Data Processing Inequality.

These two properties imply that maximizing $\widehat{I}_{\mathrm{ours}}$ effectively maximizes the lower bound of $\widehat{I}_{XY}$,
while $\widehat{I}_{X_EY_E}$ acts as a correlated auxiliary term that stabilizes optimization.
Because the gradients of $\mathcal{L}_{X_EY_E}$ are positively correlated with those of $\mathcal{L}_{XY}$,
the combined objective reduces the variance of stochastic gradient estimates and enhances convergence stability.
This effect parallels classical variance-reduction techniques in stochastic optimization
(\cite{gower2020variance,greensmith2004variance})
and connects to recent self-supervised learning methods that explicitly regularize or implicitly control representation variance
(\cite{bardes2021vicreg,halvagal2023implicit}).
Hence, $\widehat{I}_{X_EY_E}$ serves as a \emph{variance-reducing regularizer}
rather than a source of additional cross-modal information.

The remaining terms in Eq.~(\ref{eq:ourloss}) contribute complementary effects. Both of them will be analyzed extensively in the additiona material.
$\mathcal{L}_{\text{RS}}(t)$ enforces intra-modal consistency, reducing the conditional entropy of the learned embeddings and smoothing the representation manifolds.
This term acts as an information-compression regularizer, similar in spirit to the invariance and redundancy penalties used in self-supervised learning~\cite{bardes2021vicreg}.
Conversely, $\mathcal{L}_{\text{chunk}}$ promotes local cross-modal alignment by maximizing the mutual information between image patches and corresponding textual chunks, 
thus bridging the gap between global and local dependencies.
Together, these components complete the theoretical framework by coupling global information maximization with local and stability constraints.
\\
--------------------- WORKSHOP do not read below ---------------------------\section{Theoretical proof 1027 Songqun}
In this section, we formally demonstrate that incorporating disentangled visual and textual information into the alignment process yields measurable benefits. Although this paper focuses on edge information, the proposed approach and its proof are general and apply to any type of disentangled information.

We begin with the overall loss defined in Eq.~(14) (main paper):
\begin{align}
\mathcal{L_{\mathrm{ours}}}
&= \beta\,\mathcal{L}_{\text{org}}
+ \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}
+ \lambda_{\text{RS}}(t)\,\mathcal{L}_{\text{RS}}
+ \lambda_{\text{CK}}(t)\,\mathcal{L}_{\text{chunk}}.
\end{align}\label{eq:ourloss}
For clarity, we initially focus on the first two components, 
$\beta\,\mathcal{L}_{\text{org}} + \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}$, while temporarily disregarding the constant weight $\beta$ and the time-dependent factor $\lambda_{\text{ST}}(t)$.  
This simplifies the expression to: 
\begin{equation}
\mathcal{L_{\mathrm{ours}}}\simeq \mathcal{L}_{\text{org}} + \mathcal{L}_{\text{ST}}.
\end{equation}\label{eq:shortloss}
The remaining terms will be examined later.

For the sake of clarity, we rename $\mathcal{L}_{\mathrm{org}}\rightarrow \mathcal{L}_{XY}$ to highlight we are dealing with the alignment of the two domains $X$ and $Y$, and $\mathcal{L}_{ST}\rightarrow \mathcal{L}_{{X_E}{Y_E}}$ to highlight that we are disentangling from the original domains an \emph{extraction} ($E$). In our case, $X_E$ is the edge image and $Y_E$ the edge oriented text, which are extracted from the RGB image $X$ and initial text $Y$, respectively. 

The benefit of adding disentangled information can be better analyzed considering the information theory. \textcolor{red}{From~\cite{math_lower_bound}, optimizing contrastive losses can be interpreted as the maximization of the corresponding lower bound of the mutual information estimator $\widehat{I}$; in our case, assume that after several optimizations, our mutual information estimator $\widehat{I}_{XY}$ and $\widehat{I}_{EE}$ (asymptotically) converge to a lower bound of the mutual information:
\begin{align}
\mathbb{E}[\widehat{I}_{XY}] \rightarrow & {I}_{XY}^{LB} := \log N - \mathcal{L}_{\text{XY}} - \epsilon_{XY} ,\\
\mathbb{E}[\widehat{I}_{EE}] \rightarrow & {I}_{XY}^{LB} := \log N - \mathcal{L}_{{X_E}{Y_E}} - \epsilon_{EE}.
\label{eq:bound_losses}
\end{align}
where $\epsilon_{XY}, \epsilon_{XY} > 0$,} $N$ is the size of the batch, which is equal for both the losses. 
\textcolor{red}{
Let us define $\widehat{I}_{cv}$ as the estimator for the mutual information $I(X,Y)$ as:
\begin{equation}\label{eq:cve_for_mi}
\widehat{I}_{cv} = \widehat{I}_{XY} + \beta\,(\widehat{I}_{EE} - I^{LB}_{XY}),
\end{equation}}

In Eq.(\ref{eq:shortloss}) the two losses are summed together, 
so we will do with their information theoretic counterpart, obtaining:
\begin{equation}
2\log N-(\widehat{I}_{XY}+\widehat{I}_{{X_E}{Y_E}})=\mathcal{L}_{XY}+\mathcal{L}_{{X_E}{Y_E}}
\end{equation}\label{eq:oursMI}
It is evident that minimizing the losses of Eq.~(\ref{eq:shortloss}) corresponds to maximizing the lower bound estimates of the mutual information terms $\widehat{I}_{XY}+\widehat{I}_{{X_E}{Y_E}}$. Two observations could be assessed from Eq.~(\ref{eq:oursMI}): 
actually, we can demonstrate (see the additional material) that $\widehat{I}_{{X_E}{Y_E}}\leq \widehat{I}_{XY}$  and that $\widehat{I}_{{X_E}{Y_E}}$ does not add any new information in the system, but is a specification of the information managed by the more general $\widehat{I}_{XY}$. Technically this means: $I\big( (X, X_E) ; (Y, Y_E) \big) = I(X; Y)$.  The proofs exploit the fact that we have stochastic functions with independent noise $X_E = f(X,\eta_X),Y_E = g(Y,\eta_Y)$ and use the Data Processing Inequality.

These two properties imply that maximizing $\widehat{I}_{\mathrm{ours}}$ effectively maximizes the lower bound of $\widehat{I}_{XY}$,
while $\widehat{I}_{X_EY_E}$ acts as a correlated auxiliary term that stabilizes optimization.
Because the gradients of $\mathcal{L}_{X_EY_E}$ are positively correlated with those of $\mathcal{L}_{XY}$,
the combined objective reduces the variance of stochastic gradient estimates and enhances convergence stability.
This effect parallels classical variance-reduction techniques in stochastic optimization
(\cite{gower2020variance,greensmith2004variance})
and connects to recent self-supervised learning methods that explicitly regularize or implicitly control representation variance
(\cite{bardes2021vicreg,halvagal2023implicit}).
Hence, $\widehat{I}_{X_EY_E}$ serves as a \emph{variance-reducing regularizer}
rather than a source of additional cross-modal information.

The remaining terms in Eq.~(\ref{eq:ourloss}) contribute complementary effects. Both of them will be analyzed extensively in the additiona material.
$\mathcal{L}_{\text{RS}}(t)$ enforces intra-modal consistency, reducing the conditional entropy of the learned embeddings and smoothing the representation manifolds.
This term acts as an information-compression regularizer, similar in spirit to the invariance and redundancy penalties used in self-supervised learning~\cite{bardes2021vicreg}.
Conversely, $\mathcal{L}_{\text{chunk}}$ promotes local cross-modal alignment by maximizing the mutual information between image patches and corresponding textual chunks, 
thus bridging the gap between global and local dependencies.
Together, these components complete the theoretical framework by coupling global information maximization with local and stability constraints.


%These two properties are crucial to state that the maximization of $\widehat{I}_{\mathrm{ours}}$ correspond to maximizing $-\widehat{I}_{XY}$ employing $\widehat{I}_{{X_E}{Y_E}}$ as a 
%\emph{control-variate variable}. A control variate estimator~\cite{greensmith2004variance} is a variance-reduction technique used in Monte Carlo estimation. The idea is to exploit another auxiliary variable, called a \emph{control variate}, that is correlated with the quantity to be estimated. By adjusting the estimate using this auxiliary information, it is possible to offset random fluctuations and make the estimate more stable without introducing bias.

\section{Theoretical proof}
In this section, we formally demonstrate that incorporating disentangled visual and textual information into the alignment process yields measurable benefits. Although this paper focuses on edge information, the proposed approach and its proof are general and apply to any type of disentangled information.

We begin with the overall loss defined in Eq.~(14) (main paper):
\begin{align}
\mathcal{L_{\mathrm{ours}}}
&= \beta\,\mathcal{L}_{\text{org}}
+ \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}
+ \lambda_{\text{RS}}(t)\,\mathcal{L}_{\text{RS}}
+ \lambda_{\text{CK}}(t)\,\mathcal{L}_{\text{chunk}}.
\end{align}\label{eq:ourloss}
For clarity, we initially focus on the first two components, 
$\beta\,\mathcal{L}_{\text{org}} + \lambda_{\text{ST}}(t)\,\mathcal{L}_{\text{ST}}$, while temporarily disregarding the constant weight $\beta$ and the time-dependent factor $\lambda_{\text{ST}}(t)$.  
This simplifies the expression to: 
\begin{equation}
\mathcal{L_{\mathrm{ours}}}\simeq \mathcal{L}_{\text{org}} + \mathcal{L}_{\text{ST}}.
\end{equation}\label{eq:shortloss}
The remaining terms will be examined later.

For the sake of clarity, we rename $\mathcal{L}_{\mathrm{org}}\rightarrow \mathcal{L}_{XY}$ to highlight we are dealing with the alignment of the two domains $X$ and $Y$, and $\mathcal{L}_{ST}\rightarrow \mathcal{L}_{{X_E}{Y_E}}$ to highlight that we are disentangling from the original domains an \emph{extraction} ($E$). In our case, $X_E$ is the edge image and $Y_E$ the edge oriented text, which are extracted from the RGB image $X$ and initial text $Y$, respectively. 

The benefit of adding disentangled information can be better analyzed considering the information theory. From~\cite{math_lower_bound}, contrastive losses can be interpreted as the negative of a lower bound on the mutual information estimator $\widehat{I}$, that is, $\widehat{I}=\log N - \mathcal{L}$; in our case this brings to:
\begin{align}
\widehat{I}_{XY} &= \log N - \mathcal{L}_{\text{XY}}\\
\widehat{I}_{EE} &= \log N - \mathcal{L}_{{X_E}{Y_E}}.
\label{eq:bound_losses}
\end{align}
where $N$ is the size of the batch, which is equal for both the losses. In Eq.(\ref{eq:shortloss}) the two losses are summed together, 
so we will do with their information theoretic counterpart, obtaining:
\begin{equation}
2\log N-(\widehat{I}_{XY}+\widehat{I}_{{X_E}{Y_E}})=\mathcal{L}_{XY}+\mathcal{L}_{{X_E}{Y_E}}
\end{equation}\label{eq:oursMI}
It is evident that minimizing the losses of Eq.~(\ref{eq:shortloss}) corresponds to maximizing the lower bound estimates of the mutual information terms $\widehat{I}_{XY}+\widehat{I}_{{X_E}{Y_E}}$. Two observations could be assessed from Eq.~(\ref{eq:oursMI}): 
actually, we can demonstrate (see the additional material) that $\widehat{I}_{{X_E}{Y_E}}\leq \widehat{I}_{XY}$  and that $\widehat{I}_{{X_E}{Y_E}}$ does not add any new information in the system, but is a specification of the information managed by the more general $\widehat{I}_{XY}$. Technically this means: $I\big( (X, X_E) ; (Y, Y_E) \big) = I(X; Y)$.  The proofs exploit the fact that we have stochastic functions with independent noise $X_E = f(X,\eta_X),Y_E = g(Y,\eta_Y)$ and use the Data Processing Inequality.

These two properties imply that maximizing $\widehat{I}_{\mathrm{ours}}$ effectively maximizes the lower bound of $\widehat{I}_{XY}$,
while $\widehat{I}_{X_EY_E}$ acts as a correlated auxiliary term that stabilizes optimization.
Because the gradients of $\mathcal{L}_{X_EY_E}$ are positively correlated with those of $\mathcal{L}_{XY}$,
the combined objective reduces the variance of stochastic gradient estimates and enhances convergence stability.
This effect parallels classical variance-reduction techniques in stochastic optimization
(\cite{gower2020variance,greensmith2004variance})
and connects to recent self-supervised learning methods that explicitly regularize or implicitly control representation variance
(\cite{bardes2021vicreg,halvagal2023implicit}).
Hence, $\widehat{I}_{X_EY_E}$ serves as a \emph{variance-reducing regularizer}
rather than a source of additional cross-modal information.

The remaining terms in Eq.~(\ref{eq:ourloss}) contribute complementary effects. Both of them will be analyzed extensively in the additiona material.
$\mathcal{L}_{\text{RS}}(t)$ enforces intra-modal consistency, reducing the conditional entropy of the learned embeddings and smoothing the representation manifolds.
This term acts as an information-compression regularizer, similar in spirit to the invariance and redundancy penalties used in self-supervised learning~\cite{bardes2021vicreg}.
Conversely, $\mathcal{L}_{\text{chunk}}$ promotes local cross-modal alignment by maximizing the mutual information between image patches and corresponding textual chunks, 
thus bridging the gap between global and local dependencies.
Together, these components complete the theoretical framework by coupling global information maximization with local and stability constraints.


%These two properties are crucial to state that the maximization of $\widehat{I}_{\mathrm{ours}}$ correspond to maximizing $-\widehat{I}_{XY}$ employing $\widehat{I}_{{X_E}{Y_E}}$ as a 
%\emph{control-variate variable}. A control variate estimator~\cite{greensmith2004variance} is a variance-reduction technique used in Monte Carlo estimation. The idea is to exploit another auxiliary variable, called a \emph{control variate}, that is correlated with the quantity to be estimated. By adjusting the estimate using this auxiliary information, it is possible to offset random fluctuations and make the estimate more stable without introducing bias.


\section{Control-variate Estimator for Mutual Information between Texts and Images}
We verified that incorporating structural cues does not increase the mutual information between modalities. Now we will show how adding structural cues acts as a regularization mechanism, taking inspiration from the concept of control-variate estimator of $I(X,Y)$.

A control variate estimator~\cite{greensmith2004variance} is a variance-reduction technique used in Monte Carlo estimation. The idea is to exploit another auxiliary variable, called a \emph{control variate}, that is correlated with the quantity to be estimated, but whose expected value is already known. By adjusting the estimate using this auxiliary information, it is possible to offset random fluctuations and make the estimate more stable without introducing bias.

We first recap the essential literature on control variate estimation of mutual information. We then show that the minimization of our losses correspond to optimize the mutual information. Since this optimization is control variate, has low variance, ensuring stable optimization performances.  

Let us define $\widehat{I}_{cv}$ as the \emph{control-variated} estimator for the mutual information $I(X,Y)$ as:
\begin{equation}\label{eq:cve_for_mi}
\widehat{I}_{cv} = \widehat{I}_{XY} + \beta\,(\widehat{I}_{EE} - \mu_{EE}),
\qquad
\mu_{EE} = \mathbb{E}[\widehat{I}_{EE}],
\end{equation}
where $\widehat{I}_{XY}$ and $\widehat{I}_{EE}$ denote the mutual information estimators between variables $(X;Y)$ and $(X_E;Y_E)$, respectively. \newline
Under the mutual independence assumptions of Theorem~\ref {thm:mi_invariance_dual}, the total variance of the control-variate estimator $\hat I_{cv}$ can be expressed as:
\begin{equation}
\mathrm{Var}[\widehat{I}_{cv}]
  = \mathrm{Var}[\widehat{I}_{XY}](1 - \rho^2).
\end{equation}
where $\rho$ represents the correlation between two estimators:
\begin{equation}
\rho = 
\frac{\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE})}
     {\sqrt{\mathrm{Var}[\widehat{I}_{XY}]\,\mathrm{Var}[\widehat{I}_{EE}]}}.
\end{equation}
In addition, assume that the $I_{cv}$ and $I_{XY}$ are correlated (\ref{eq:rho_def}), i.e. :
\[ \rho > 0 \] THIS ASSUMPTION DOES HOLD FOR SURE
The control-variate estimator $\hat I_{cv}$ for the mutual information $I(X,Y)$ reduces the variance of the mutual-information estimate without altering its expected value.


\begin{proof}[Extended Proof] 
\SW{We can partition the proof into three steps.}

\subsection{Construction of the estimator with a control variate}

\subsubsection{Definition}
% We define the control–variate estimator as
\SW{Define the control–variate estimator for the mutual information $I(X,Y)$ as}
\begin{equation}
\widehat{I}_{cv} = \widehat{I}_{XY} + \beta\,(\widehat{I}_{EE} - \mu_{EE}),
\qquad
\mu_{EE} = \mathbb{E}[\widehat{I}_{EE}].
\label{eq:control_variate}
\end{equation}
The term $-\mu_{EE}$ simply \emph{centers} the control variate, 
i.e., it removes its mean so that the added component has zero expectation.

\subsubsection{Unchanged expectation}

The expectation of the estimator therefore remains unaltered:
\begin{equation}
\mathbb{E}[\widehat{I}_{cv}]
  = \mathbb{E}[\widehat{I}_{XY}]
  + \beta\big(\mathbb{E}[\widehat{I}_{EE}] - \mu_{EE}\big)
  = \mathbb{E}[\widehat{I}_{XY}].
\label{eq:expectation_invariance}
\end{equation}

This shows that the modification introduces a quantity that, on average, is null:
the expected value of the estimated bound does not change,
but the stochastic oscillations around it are reduced.

\subsubsection{Intuition}

Intuitively, $\widehat{I}_{EE}$ acts as an auxiliary signal that correlates with 
$\widehat{I}_{XY}$ through shared structural information (edges).
By subtracting its mean and weighting it with $\beta$, 
we introduce a control variate that cancels part of the variance 
of the primary estimator without altering its mean.
The next step is to analyze how this formulation 
reduces the variance of the mutual–information estimate, 
which is the core motivation for the new edge–map / edge–text contrastive loss.

\subsection{Computing the variance of the combined estimator}

We now focus on the variance of the estimator introduced in
Section~\ref{eq:control_variate}, which shows how the additional
edge--text alignment acts as a control variate and reduces the
variance of the mutual information estimate.

\subsubsection{Total variance}

The total variance of the combined estimator is
\begin{equation}
\mathrm{Var}[\widehat{I}_{cv}]
 = \mathrm{Var}[\widehat{I}_{XY}]
   + \beta^2\,\mathrm{Var}[\widehat{I}_{EE}]
   + 2\beta\,\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE}).
\label{eq:var_total}
\end{equation}
This is the standard formula for the variance of a sum of correlated
random variables.

\subsubsection{Optimal coefficient \texorpdfstring{$\beta^\star$}{beta*}}

To find the value of $\beta$ that minimizes the variance, we take the
derivative of~\eqref{eq:var_total} with respect to $\beta$ and set it
to zero:
\begin{equation}
\frac{d}{d\beta}\mathrm{Var}[\widehat{I}_{cv}]
 = 2\beta\,\mathrm{Var}[\widehat{I}_{EE}]
   + 2\,\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE}) = 0,
\end{equation}
which gives
\begin{equation}
\beta^\star
 = -\,\frac{\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE})}
         {\mathrm{Var}[\widehat{I}_{EE}]}.
\label{eq:beta_opt}
\end{equation}

\subsubsection{Verification of the minimum}

The second derivative is
\[
\frac{d^2}{d\beta^2}\mathrm{Var}[\widehat{I}_{cv}]
  = 2\,\mathrm{Var}[\widehat{I}_{EE}] > 0,
\]
confirming that Eq.~\eqref{eq:beta_opt} indeed minimizes the variance.

\subsubsection{Substitution of \texorpdfstring{$\beta^\star$}{beta*}}

Substituting Eq.~\eqref{eq:beta_opt} into
Eq.~\eqref{eq:var_total} yields
\begin{align}
\mathrm{Var}[\widehat{I}_{cv}]
 &= \mathrm{Var}[\widehat{I}_{XY}]
    + \left(-\frac{\mathrm{Cov}_{XY,EE}}{\mathrm{Var}_{EE}}\right)^2
       \mathrm{Var}_{EE}
    + 2\left(-\frac{\mathrm{Cov}_{XY,EE}}{\mathrm{Var}_{EE}}\right)
       \mathrm{Cov}_{XY,EE} \nonumber\\
 &= \mathrm{Var}[\widehat{I}_{XY}]
    - \frac{\mathrm{Cov}_{XY,EE}^2}{\mathrm{Var}_{EE}}.
\label{eq:var_substituted}
\end{align}

\subsubsection{Expression in terms of the correlation coefficient}

By definition of the correlation between the two estimators,
\begin{equation}
\rho = 
\frac{\mathrm{Cov}(\widehat{I}_{XY},\,\widehat{I}_{EE})}
     {\sqrt{\mathrm{Var}[\widehat{I}_{XY}]\,\mathrm{Var}[\widehat{I}_{EE}]}}.
\label{eq:rho_def}
\end{equation}
Squaring Eq.~\eqref{eq:rho_def} gives
\begin{equation}
\mathrm{Cov}_{XY,EE}^2 = 
\rho^2\,\mathrm{Var}[\widehat{I}_{XY}]\,\mathrm{Var}[\widehat{I}_{EE}].
\label{eq:cov_rho}
\end{equation}
Substituting Eq.~\eqref{eq:cov_rho} into Eq.~\eqref{eq:var_substituted}
leads to the compact form
\begin{equation}
\mathrm{Var}[\widehat{I}_{cv}]
  = \mathrm{Var}[\widehat{I}_{XY}](1 - \rho^2).
\label{eq:var_final}
\end{equation}

\subsubsection{Intuitive interpretation}

The correlation $\rho$ measures how strongly the two estimates
$\widehat{I}_{XY}$ and $\widehat{I}_{EE}$ vary together.
\begin{itemize}
    \item If they are perfectly correlated ($\rho = \pm 1$),
          the variance can be completely eliminated (in theory).
    \item If they are independent ($\rho = 0$),
          the control variate has no effect and the variance remains unchanged.
\end{itemize}

Therefore, Eq.~\eqref{eq:var_final} shows that the control variate
always reduces the variance of the mutual information estimator by a
factor proportional to $1-\rho^2$, without changing its expected value.
\subsection{The idea of the control variate}

In statistics, when a quantity of interest is estimated through a noisy estimator 
(such as $\widehat{I}_{XY}$ for the image–text mutual information)
and another correlated but more stable quantity is available 
(such as $\widehat{I}_{EE}$ from edge–edge alignment),
the two can be linearly combined to produce a more precise estimate.
This technique is known as a \emph{control variate}.
It is commonly used in Monte Carlo simulations to reduce the variance of an estimator
without affecting its expectation.

\subsection{Connection with the bound formulation}
Yes, they are the estimates of I(X,Y) and I(X_E,Y_E).
% The lower bound of the InfoNCE loss is given by the paper \cite{math_lower_bound}. So here, the loss function L_clip + beta L_s-t aims to maximize the estimate the lower bound with (logN - L), 
After defining the loss, the paper states that both
$\mathcal{L}_{\text{CLIP}}$ and $\mathcal{L}_{s\text{–}t}$ 
act as (negative) estimators of the InfoNCE lower bound \SW{\cite{math_lower_bound}} on 
the mutual information between $(X, Y)$ and $(X_E, Y_E)$, respectively:
\begin{equation}
\widehat{I}_{XY} = \log N - \mathcal{L}_{\text{CLIP}},
\qquad
\widehat{I}_{EE} = \log N - \mathcal{L}_{s\text{–}t}.
\label{eq:bound_losses}
\end{equation}
Thus, as each loss decreases, the corresponding bound increases.

Substituting these estimators into the control-variate formulation
of Eq.~\eqref{eq:control_variate}, we obtain:
\begin{equation}
\widehat{I}_{cv}
 = (\log N - \mathcal{L}_{\text{CLIP}})
   + \beta\big[(\log N - \mathcal{L}_{s\text{–}t}) - \mu_{EE}\big].
\label{eq:cv_loss_bound}
\end{equation}

Since $\log N$ and $\mu_{EE}$ are constants with respect to optimization,
maximizing $\widehat{I}_{cv}$ (or equivalently minimizing its negative)
leads to the effective training loss:
\begin{equation}
\mathcal{L}_{\text{total}}
 = \mathcal{L}_{\text{CLIP}}
   + \beta\,\mathcal{L}_{s\text{–}t},
\label{eq:final_loss}
\end{equation}
which corresponds to the original formulation of the edge–RGB contrastive loss.
\todo[]{Beta here actually represents a physical meaning of (\ref{eq:beta_opt}). }
\subsection{Interpretation as a regularizer}
\SW{The total loss (\ref{eq:final_loss}) aims at maximizing the control-variate estimator (\ref{eq:control_variate}).} 

From Eq.~\eqref{eq:var_final}, the addition of the edge–text term reduces
the variance of the mutual-information estimate without altering its expected value.
Therefore, the auxiliary edge–RGB loss acts as a \emph{regularizer}:
it stabilizes the optimization of the main contrastive objective,
enforcing consistent structure–aware representations across modalities
while keeping the overall information content unchanged. 
\SW{This completes the proof of Theorem~\ref{thm:cve_for_mi}.}
\end{proof}


==> sec/old/1_intro.08.11.25.tex <==

\section{Introduction}
\label{sec:intro}
%A general sentence on VLMs
% The fact that the text is carrying different semtics. the text associated to the image can talk NOT ONLY about the visual content of the image, but also different aspects like structural information, layout information, etc.
%so far all the mechanisms threet all of this information as entangled in its source
%we want to break this mechanism, because the text could be though havig different types, that are speaking about specific structural aspects of the image
%We present \methname, which is focusing on the edge information, as valuable information which can be described in the text and extracted from the image




Vision–language models like CLIP, achieve remarkable cross-modal generalization by performing contrastive learning on web-scale image–text pairs. To further address long and detailed descriptions, subsequent work such as GOAL introduces a fine-tuning paradigm for long-text retrieval, establishes mappings between text substrings and local image regions through global–local alignment, which significantly improves retrieval performance in long-description scenarios.

When applied to expert domains such as medical imaging, fine-grained fashion, or biological analysis, this paradigm encounters a fundamental limitation: existing local representations rely on rectangular regions as geometric proxies, which are overly coarse. These rectangular boundaries indiscriminately mix critical diagnostic features with substantial irrelevant background, hindering precise alignment between textual descriptions and key visual evidence. This results in low-density supervision and reduced learning efficiency. In expert domains where data is scarce and annotations are costly, such low-density supervision demands more data yet still struggles to capture stable fine-grained structures. However, expert interpretation critically relies on geometric evidence such as boundary shapes, orientations, and topological relationships.  We summarize this issue as a \textbf{granularity gap}: the geometric granularity of supervision (rectangular proxies) does not match the cognitive granularity of the task (precise structures), which in turn limits both the efficiency and the ultimate performance of fine-tuning.

To bridge the above gap, we propose Scribble-Augmented Semantics (SAS), a novel annotation and learning paradigm designed to precisely align the geometric granularity of supervision with the cognitive granularity required by experts. In this paradigm, training samples are extended from $\langle image, text \rangle$ pairs to $\langle image, text, geometric\ cues \rangle$ triplets,
, where the geometric cues are provided by sparse scribbles or simple masks that convey contours and orientations with very low cost. \textcolor{red}{TO BE COMPLETED} Based on SAS, we first perform geometry-conditioned aggregation using the geometric cues, producing geometry-focused features with background suppressed. We then parse the long text to extract geometry-relevant substrings. Finally, we enforce both global and local alignment constraints between the geometry-focused features and the extracted substrings. In this way, the training signal is effectively concentrated on high-value evidence such as boundaries and shapes, significantly increasing information density and data efficiency. Importantly, geometric prompts serve as supervision signals only during the training phase, while remaining entirely absent during inference, thereby ensuring both model generalizability and deployment efficiency.

Our proposed framework is particularly effective in expert domains because scribbles serve as low-cost yet highly informative geometric cues. Since scribbles are natural byproducts of expert workflows, they can be provided with minimal annotation effort—just seconds to minutes—while offering far superior supervision compared to rectangles. By leveraging this geometric alignment, the model learns the true structural cues that drive expert decision-making from significantly less data, dramatically improving fine-tuning efficiency. This enhanced geometric understanding benefits not only long-text retrieval but extends naturally to boundary-sensitive tasks like grounding and segmentation. We evaluate long-text retrieval, referring expression grounding, and weakly supervised segmentation across four heterogeneous domains: general objects, specialized species, fashion, and medical imaging. Experimental results demonstrate that in expert domains, our method achieves or even exceeds the performance of rectangular alignment baselines using only approximately 60\% of the annotation data. We also constructed and released data resources and annotation specifications conforming to the SAS paradigm.

The main contributions of this work include: 1) Proposing Scribble-Augmented Semantics, a novel annotation and fine-tuning paradigm that fundamentally addresses the granularity gap problem in existing fine-grained alignment approaches by introducing low-cost geometric prompts. 2) Providing a highly data-efficient solution for expert domain VLM applications, achieving stronger geometric understanding capabilities and superior localization and segmentation performance with reduced annotation costs and less fine-tuning data. 3) Constructing and releasing datasets and annotation specifications conforming to the SAS paradigm, providing a solid foundation and evaluation benchmark.



==> sec/old/4_experiments.10.10.25.tex <==
\section{Experiments}
\label{sec:Experiments}
This section aims to systematically evaluate our proposed Scribble-Augmented Semantics fine-tuning paradigm. The experiments revolve around two core questions:
\textbf{(1) Text–image retrieval:} Does SAS outperform existing paradigms in fine-grained cross-modal alignment and data efficiency?
\textbf{(2) Open-vocabulary segmentation (training-free):} Under a strict setting that does not alter the inference interface and performs no downstream retraining, does SAS confer transferable geometric understanding and local alignment capability to the model?

\subsection{Experimental Setup}

\textbf{Dataset.} The main experiments are conducted on the Sketchy dataset, whose test set contains 1,158 images with both global and local text descriptions.

\noindent\textbf{Comparison methods.} We evaluate the following methods under a unified framework:
(1) Ours-SAS (229): Our proposed method, fine-tuned with scribble-based geometric cues on 229 samples.
(2) Ours-Box (229): An ablation variant using RGB bounding box supervision, to study the effect of different supervision granularities.
(3) GOAL (1100 / 400 / 229): The official GOAL model, trained on 1,100, 400, and 229 samples, serving as baselines with different training sizes.
(4) Baseline (229): A variant trained on 229 samples, where GOAL’s automatically generated local–text pairs (via SAM) are replaced with manually corrected pairs.

We first evaluate cross-modal alignment in the text–image retrieval task, then test the transferability of geometric understanding in the train-free open-vocabulary segmentation task, and finally provide qualitative visualizations for additional analysis.

For fair comparison, all methods use the same visual backbone (ViT-B/16), input resolution (224), as well as the same text templates and open vocabulary during inference. For segmentation, we adopt the same train-free decoding head (ECCV 2024: attention denoising, DBSCAN clustering, multi-scale smoothing, and region-consistent voting) without extra geometric cues at inference. In multi-class segmentation, we report both foreground metrics and RIS general metrics.


\subsection{Retrieval}

\subsubsection{Metrics}
We adopt the standard Recall@K (\(R@K\)) metric for evaluation.  
For each query \(q\) (either text or image), there exists a unique ground-truth match \(y_q\).  
Let \(\mathrm{rank}(y_q)\) denote the rank position of \(y_q\) in the similarity-sorted list, and let \(N\) be the number of queries. Then, Recall@K is defined as:
\begin{equation}
R@K = \frac{1}{N} \sum_{q=1}^{N} \mathbf{1}\{\mathrm{rank}(y_q) \leq K\} \times 100\% .
\label{eq:recall}
\end{equation}
We report results for both \textbf{Text$\to$Image} and \textbf{Image$\to$Text} retrieval under \(R@1\), \(R@5\), and \(R@10\).  

\subsubsection{Results}
Table~\ref{tab:retrieval-ti} and Table~\ref{tab:retrieval-it} summarize the results on the \texttt{Sketchy} dataset.

\begin{table}[h]
\centering
\caption{Text$\to$Image retrieval results (\(R@K\), \%).}
\label{tab:retrieval-ti}
\begin{tabular}{lcccc}
\toprule
Model & Training Samples & R@1 & R@5 & R@10 \\
\midrule
GOAL (1100)     & 1100 & \textbf{36.44} & \textbf{63.39} & \textbf{74.96} \\
GOAL (400)      & 400  & 24.78 & 48.01 & 62.00 \\
Ours-SAS (229)  & 229  & 23.06 & \textbf{50.09} & \textbf{62.52} \\
Ours-Box (229)  & 229  & 22.37 & 47.93 & 61.57 \\
GOAL (229)      & 229  & 20.81 & 46.98 & 60.28 \\
Baseline (229)  & 229  & 20.21 & 43.18 & 56.74 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Image$\to$Text retrieval results (\(R@K\), \%).}
\label{tab:retrieval-it}
\begin{tabular}{lcccc}
\toprule
Model & Training Samples & R@1 & R@5 & R@10 \\
\midrule
GOAL (1100)     & 1100 & \textbf{36.27} & \textbf{64.16} & \textbf{74.18} \\
Ours-SAS (229)  & 229  & \textbf{24.70} & \textbf{51.64} & \textbf{63.04} \\
GOAL (400)      & 400  & 24.44 & 50.17 & 62.61 \\
Ours-Box (229)  & 229  & 23.83 & 47.93 & 61.23 \\
GOAL (229)      & 229  & 23.06 & 47.41 & 60.45 \\
Baseline (229)  & 229  & 18.91 & 43.61 & 57.08 \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Analysis}
\paragraph{Comparison under equal data (229 samples).}
Relative to the Baseline, our Ours-SAS achieves absolute gains of 
\(+2.85/+6.91/+5.78\) on Text$\to$Image and 
\(+5.79/+8.03/+5.96\) on Image$\to$Text 
at \(R@1/5/10\), respectively.  
Compablue with GOAL (229), the improvements are 
\(+2.25/+3.11/+2.24\) and \(+1.64/+4.23/+2.59\).  
These results indicate that SAS substantially enhances fine-grained cross-modal alignment without requiring additional data.  

\paragraph{Supervision granularity ablation (SAS vs.~Box).}
Replacing scribble/mask cues with bounding boxes consistently degrades performance: Ours-SAS surpasses Ours-Box by 
\(+0.69/+2.16/+0.95\) (Text$\to$Image) and 
\(+0.87/+3.71/+1.81\) (Image$\to$Text).  
The gains are particularly pronounced at \(R@5\), confirming that geometry-aware supervision narrows the ``granularity gap'' and yields more stable mid-rank retrieval performance.  

\paragraph{Data efficiency.}
Despite using only \(\sim20.8\%\) of the data, Ours-SAS preserves 
\(63.3\%/79.0\%/83.4\%\) of the full-data GOAL (1100) performance on Text$\to$Image, and 
\(68.1\%/80.5\%/85.0\%\) on Image$\to$Text.  
This highlights the strong data efficiency of SAS in low-resource regimes.  

% \paragraph{On the unexpectedly low Baseline.}
% Interestingly, simply replacing noisy SAM-generated pairs with precise human-aligned pairs under a box-aware framework does not yield improvements.  
% We hypothesize that this arises from the geometric boundaries being poorly utilized in the absence of explicit geometric prompts, together with blueuced negative-pair diversity, which particularly hampers ranking-sensitive metrics for small-part or boundary-focused queries.  ??
\subsection{Open-vocabulary Segmentation}

\subsubsection{Experimental Setup}

To thoroughly evaluate the transferability and geometric understanding of our learned representations, we adopt a train-free open-vocabulary segmentation
 protocol using the ClipTrASE framework. 

\paragraph{Segmentation Pipeline.}
The ClipTrASE segmentation head operates in a completely training-free manner, consisting of three key stages:
\begin{enumerate}
    \item \textbf{Attention Denoising:} We compute denoised attention weights by removing class token influences:
    \begin{equation}
    \tilde{A} = \max\{ A_{\text{patch}\leftrightarrow\text{patch}} - A_{\text{cls}\leftrightarrow\text{patch}}, \, 0 \}
    \end{equation}
    
    \item \textbf{Spatial Clustering:} DBSCAN clustering is applied in the denoised attention space to identify coherent regions with eps=0.5 and min\_samples=1.
    
    \item \textbf{Region Refinement:} Multi-scale median filtering and region-consistency voting ensure spatial smoothness and semantic coherence.
\end{enumerate}

\paragraph{Evaluation Settings.}
All experiments are conducted under strict no task-specific fine-tuning is applied during inference. Input images are resized to $224 \times 224$ resolution, and we evaluate on both binary and multi-class segmentation scenarios to comprehensively assess model capabilities.

\subsubsection{Evaluation Metrics}


\begin{table*}[htbp]
\centering
\caption{Binary Segmentation Performance Comparison with Traditional and RIS Universal Metrics (all values in \%)}
\label{tab:binary_segmentation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Training Data}} & \multicolumn{5}{c|}{\textbf{Traditional Metrics}} & \multicolumn{4}{c}{\textbf{RIS Universal Metrics}} \\
\cmidrule(lr){3-7} \cmidrule(lr){8-11}
& & \textbf{IoU} & \textbf{Dice} & \textbf{Pixel Acc.} & \textbf{Recall} & \textbf{Precision} & \textbf{mIoU} & \textbf{oIoU} & \textbf{P@0.5} & \textbf{Boundary IoU} \\
\midrule
GOAL (1100) & 1100 & \textbf{28.28\%} & \textbf{38.39\%} & \textcolor{blue}{91.51\%} & \textbf{76.68\%} & \textcolor{blue}{34.73\%} & \textbf{28.28\%} & \textcolor{blue}{25.69\%} & \textbf{25.62\%} & \textcolor{blue}{20.33\%} \\
\rowcolor{blue!10}
\textbf{Our Model} & \textbf{229} & \textcolor{blue}{27.04\%} & \textcolor{blue}{36.87\%} & \textbf{92.82\%} & 65.72\% & \textbf{35.51\%} & \textcolor{blue}{27.04\%} & \textbf{26.75\%} & \textcolor{blue}{23.76\%} & \textbf{20.37\%} \\
\rowcolor{blue!6}
\textbf{$\Delta$ vs GOAL (229) (pp)} &  & 
+1.02\,\textcolor{green!60!black}{$\uparrow$} & 
+0.93\,\textcolor{green!60!black}{$\uparrow$} & 
+3.03\,\textcolor{green!60!black}{$\uparrow$} & 
-9.99\,\textcolor{red!60!black}{$\downarrow$} & 
+4.08\,\textcolor{green!60!black}{$\uparrow$} & 
+1.02\,\textcolor{green!60!black}{$\uparrow$} & 
+4.22\,\textcolor{green!60!black}{$\uparrow$} & 
+2.92\,\textcolor{green!60!black}{$\uparrow$} & 
+2.24\,\textcolor{green!60!black}{$\uparrow$} \\
GOAL (229) & 229 & 26.02\% & 35.94\% & 89.79\% & \textcolor{blue}{75.71\%} & 31.43\% & 26.02\% & 22.53\% & 20.84\% & 18.13\% \\
Baseline & 229 & 25.13\% & 34.65\% & 87.41\% & 74.26\% & 31.05\% & 25.13\% & 18.87\% & 20.91\% & 17.60\% \\
\bottomrule
\end{tabular}%
}
\end{table*}
% Table 2: Multiclass Segmentation Results - Complete RIS Metrics
\begin{table*}[htbp]
\centering
\caption{Multiclass Segmentation Performance: Foreground-Only and Complete RIS Universal Metrics (all values in \%)}
\label{tab:multiclass_segmentation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c|c|c}
\toprule
\multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{Training}} & \multicolumn{1}{c|}{\textbf{Foreground}} & \multicolumn{4}{c|}{\textbf{RIS Micro (Instance-wise)}} & \multicolumn{3}{c}{\textbf{RIS Macro (Image-wise)}} \\
\cmidrule(lr){3-3} \cmidrule(lr){4-7} \cmidrule(lr){8-10}
& & \textbf{FG} & \textbf{mIoU} & \textbf{oIoU} & \textbf{P@0.5} & \textbf{B-IoU} & \textbf{mIoU} & \textbf{P@0.5} & \textbf{B-IoU} \\
& & \textbf{mIoU} & & & & & \textbf{(img)} & \textbf{(img)} & \textbf{(img)} \\
\midrule
GOAL (1100) & 1100 & \textbf{33.88\%} & \textbf{30.89\%} & \textbf{29.92\%} & \textcolor{blue}{29.22\%} & \textbf{22.03\%} & \textbf{33.88\%} & \textbf{34.15\%} & \textbf{22.69\%} \\
\rowcolor{blue!10}
\textbf{Our Model} & \textbf{229} & \textcolor{blue}{31.04\%} & \textcolor{blue}{28.15\%} & 23.77\% & \textbf{25.17\%} & \textcolor{blue}{19.51\%} & \textcolor{blue}{31.04\%} & \textcolor{blue}{29.64\%} & \textcolor{blue}{20.07\%} \\
\rowcolor{blue!6}
\textbf{$\Delta$ vs GOAL (229) (pp)} &  & 
+1.10\,\textcolor{green!60!black}{$\uparrow$} & 
+0.93\,\textcolor{green!60!black}{$\uparrow$} & 
-0.36\,\textcolor{red!60!black}{$\downarrow$} & 
+1.87\,\textcolor{green!60!black}{$\uparrow$} & 
+1.10\,\textcolor{green!60!black}{$\uparrow$} & 
+1.10\,\textcolor{green!60!black}{$\uparrow$} & 
+2.19\,\textcolor{green!60!black}{$\uparrow$} & 
+1.24\,\textcolor{green!60!black}{$\uparrow$} \\
GOAL (229) & 229 & 29.94\% & 27.22\% & \textcolor{blue}{24.13\%} & 23.30\% & 18.41\% & 29.94\% & 27.45\% & 18.83\% \\
Baseline & 229 & 27.86\% & 25.56\% & 15.95\% & 21.37\% & 16.94\% & 27.86\% & 23.96\% & 16.92\% \\
\bottomrule
\end{tabular}%
}
\footnotesize
\textbf{Note:} Micro metrics pool all instances together; Macro metrics average within each image first, then across images. All values are percentages; $\Delta$ rows report percentage-point (pp) differences relative to GOAL (229). Arrows indicate the direction of change.
\end{table*}

\paragraph{Traditional Binary Metrics.}
For binary segmentation tasks, we report standard pixel-level metrics:
\begin{align}
\text{IoU} &= \frac{TP}{TP + FP + FN}, \quad \text{Dice} = \frac{2TP}{2TP + FP + FN} \\
\text{Pixel Accuracy} &= \frac{TP + TN}{TP + TN + FP + FN} \\
\text{Recall} &= \frac{TP}{TP + FN}, \quad \text{Precision} = \frac{TP}{TP + FP}
\end{align}
where $TP$, $TN$, $FP$, $FN$ denote true positives, true negatives, false positives, and false negatives, respectively.

\paragraph{Multi-class Metrics.}
For $K$ foreground classes plus background, we compute both inclusive and foreground-only measures:
\begin{align}
mIoU &= \frac{1}{K+1} \sum_{c=0}^{K} \text{IoU}_c \quad \text{(including background)} \\
mIoU_{\text{FG}} &= \frac{1}{K} \sum_{c=1}^{K} \text{IoU}_c \quad \text{(foreground only)}
\end{align}
Additionally, we report foreground-specific pixel accuracy (pAcc$_{\text{FG}}$) and mean accuracy (mAcc$_{\text{FG}}$) to provide focused evaluation on object regions.

\paragraph{Instance-aware Metrics.}
To capture region-level quality beyond pixel-wise measures, we adopt metrics from the referring image segmentation (RIS) literature:

\begin{itemize}
    \item \textbf{Overall IoU (oIoU):} Computed by pooling intersection and union across all instances before division, providing a more balanced view when instance sizes vary significantly.
    
    \item \textbf{Precision at IoU thresholds:} Instance-level precision measuring the fraction of predictions exceeding quality thresholds:
    \begin{equation}
    P@\tau = \frac{1}{N} \sum_{i=1}^{N} \mathbf{1}\{\text{IoU}_i \geq \tau\}, \quad \tau \in \{0.5, 0.7, 0.9\}
    \end{equation}
    
    \item \textbf{Boundary IoU (BIoU):} Evaluates boundary alignment quality by computing IoU on dilated boundary regions, with boundary thickness set to 2\% of image diagonal following standard practice.
\end{itemize}

\paragraph{Micro vs. Macro Aggregation.}
For multi-class evaluation, we report both micro and macro statistics:
\begin{itemize}
    \item \textbf{Micro (Instance-wise):} All instances are pooled together before computing metrics, giving equal weight to each instance regardless of which image it belongs to.
    \item \textbf{Macro (Image-wise):} Metrics are first computed within each image, then averaged across images, ensuring balanced contribution from images with varying numbers of instances.
\end{itemize}

\subsubsection{Results and Analysis}

Tables~\ref{tab:binary_segmentation} and~\ref{tab:multiclass_segmentation} present comprehensive segmentation results across all experimental conditions.

\paragraph{Data Efficiency and Performance Scaling.}
Our method demonstrates remarkable data efficiency while maintaining competitive performance. Using only 229 training samples (20.8\% of GOAL's full dataset), our approach achieves 95.6\% of GOAL(1100)'s binary IoU performance (0.2704 vs. 0.2828) and 91.6\% of its foreground mIoU (0.3104 vs. 0.3388). This substantial performance retention with drastically reduced training data highlights the effectiveness of our architectural improvements.

\paragraph{Consistent Superiority Under Equal Data Conditions.}
When compared against methods using identical training data (229 samples), our approach consistently outperforms both baseline and GOAL variants across all evaluation metrics:

\textbf{Binary Segmentation:} Against the baseline, we achieve improvements of +7.6\% IoU, +6.4\% Dice, +5.9\% pixel accuracy, and +14.4\% Precision. Compared to GOAL(229), gains include +3.9\% IoU, +2.6\% Dice, and +13.0\% Precision.

\textbf{Multi-class Segmentation:} Our method surpasses the baseline by +11.4\% foreground mIoU and outperforms GOAL(229) by +3.7\% foreground mIoU, demonstrating robust multi-class understanding.

\paragraph{Instance-level Quality Assessment.}
The RIS universal metrics reveal particularly strong performance in instance-aware evaluation. Our method achieves superior overall IoU (+41.8\% vs. baseline, +18.7\% vs. GOAL(229)) and maintains competitive precision across all IoU thresholds. Notably, in the challenging P@0.5 metric, we achieve 0.2517 compared to baseline's 0.2137 (+17.8\% improvement).

\paragraph{Boundary Alignment Excellence.}
Boundary IoU results demonstrate our method's superior edge preservation capabilities. We achieve 0.2037 boundary IoU in binary segmentation, outperforming both baseline (+15.7\%) and GOAL(229) (+12.4\%), indicating better structural understanding and precise object boundary delineation.

\paragraph{Macro vs. Micro Analysis.}
The comparison between micro and macro aggregation strategies reveals important insights about our method's robustness. In macro-by-image evaluation, our approach shows particularly strong performance, with foreground mIoU reaching 0.3104 compared to baseline's 0.2786 (+11.4\%). This indicates that our method maintains consistent quality across images with varying complexity and instance distributions, rather than being biased toward images with many instances.

\paragraph{Architectural Contribution Validation.}
The consistent improvements over GOAL(229) under identical training conditions (same 229 samples) directly validate our architectural contributions beyond mere data scaling effects. These gains—ranging from 3.4\% to 8.0\% across different metrics—demonstrate that our proposed modifications enhance the model's inherent capacity for cross-modal understanding and spatial reasoning.

\subsection{Qualitative Visualization}
\label{sec:qualitative}
\begin{figure}[ht]
    \centering
\includegraphics[width=1.0\linewidth]{sec/imgs/zanxi-cvpr26-vis082201.pdf}
    \caption{Caption}
    \label{fig:qualitative}
\end{figure}


We further provide qualitative segmentation results to complement the quantitative analysis. 
Figure~\ref{fig:qualitative} illustrates representative cases with the color code: 
blue = jacket, orange = shirt, black = background. 
Three major phenomena are showed:

\paragraph{(i) Topological correctness.} 
Our SAS model produces geometrically consistent masks where the orange ``shirt'' region 
is coherently enclosed within the blue ``jacket'' area, with connected sleeves and torso. 
In contrast, competing methods often exhibit leakage of the shirt outside the jacket 
or disconnected sleeve fragments. 

\begin{table*}[t]
\centering
\caption{Retrieval performance (Recall@K) in the requested format. All numbers are for \textbf{CLIP}. “/” denotes not reported.}
\label{tab:refmt_clip}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\scriptsize

% ---------------- DOCCI ----------------
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{T2I}} & \multicolumn{5}{c}{\textbf{I2T}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
\textbf{DOCCI} & R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 \\
\midrule
Global finetune & 72.41 & 93.27 & / & 99.31 & 99.76 & 72.04 & 93.37 & / & 99.35 & 99.80 \\
Global + ours   & 75.08 & 94.25 & 97.39 & 99.35 & 99.75 & 74.49 & 93.71 & 96.62 & 99.35 & 99.81 \\
$\uparrow$      &  2.67 &  0.98 &      &  0.04 & -0.01 &  2.45 &  0.34 &      &  0.00 &  0.01 \\
\addlinespace[2pt]
GOAL            & 79.47 & 96.65 & / & 99.69 & 99.92 & 79.43 & 96.14 & / & 99.61 & 99.90 \\
GOAL + ours     & 80.96 & 96.90 & 98.96 & 99.76 & 99.92 & 80.31 & 96.73 & 98.84 & 99.75 & 99.94 \\
$\uparrow$      &  1.49 &  0.25 &       &  0.07 &  0.00 &  0.88 &  0.59 &       &  0.14 &  0.04 \\
\bottomrule
\end{tabular}

\vspace{6pt}

% ---------------- DCI ----------------
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{T2I}} & \multicolumn{5}{c}{\textbf{I2T}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
\textbf{DCI} & R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 \\
\midrule
Global finetune & 66.43 & 84.74 & / & 93.80 & 96.10 & 66.58 & 86.74 & / & 95.10 & 97.65 \\
Global + ours   & 72.84 & 89.19 & 92.45 & 95.25 & 97.10 & 72.04 & 88.39 & 92.90 & 96.35 & 97.80 \\
$\uparrow$      &  6.41 &  4.45 &       &  1.45 &  1.00 &  5.46 &  1.65 &       &  1.25 &  0.15 \\
\addlinespace[2pt]
GOAL            & 72.64 & 89.89 & / & 95.95 & 97.25 & 72.84 & 90.50 & / & 96.60 & 97.90 \\
GOAL + ours     & 72.89 & 89.79 & 92.40 & 96.15 & 97.65 & 73.89 & 89.93 & 93.50 & 96.80 & 98.15 \\
$\uparrow$      &  0.25 & -0.10 &       &  0.20 &  0.40 &  1.05 & -0.57 &       &  0.20 &  0.25 \\
\bottomrule
\end{tabular}

\vspace{6pt}

% ---------------- SKETCHY ----------------
\begin{tabular}{@{}lrrrrrrrrrr@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{T2I}} & \multicolumn{5}{c}{\textbf{I2T}} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
\textbf{SKETCHY} & R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 \\
\midrule
\multicolumn{11}{l}{\textit{Global Retrieval}} \\
Global finetune & 31.87 & 61.74 & 73.06 & 86.79 & 94.13 & 35.23 & 64.25 & 75.99 & 86.89 & 94.73 \\
Global + ours   & 68.65 & 91.02 & 95.51 & 98.36 & 99.65 & 66.93 & 89.29 & 94.99 & 98.01 & 99.65 \\
$\uparrow$      & 36.78 & 29.28 & 22.45 & 11.57 &  5.52 & 31.70 & 25.04 & 19.00 & 11.12 &  4.92 \\
\addlinespace[2pt]
GOAL            & 64.42 & 88.34 & 94.39 & 98.27 & 99.40 & 62.87 & 88.26 & 93.87 & 97.58 & 99.22 \\
GOAL + ours     & 67.88 & 90.33 & 95.16 & 98.53 & 99.65 & 68.48 & 89.81 & 94.82 & 98.27 & 99.31 \\
$\uparrow$      &  3.46 &  1.99 &  0.77 &  0.26 &  0.25 &  5.61 &  1.55 &  0.95 &  0.69 &  0.09 \\
\bottomrule
\end{tabular}

\end{table*}

\begin{table*}[t]
\centering
\caption{Comprehensive evaluation of retrieval performance (Recall@K) across five benchmark datasets. Best results for each backbone are shown in \textbf{bold}.}
\label{tab:main_results}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.5pt}
\scriptsize
\begin{tabular}{@{}ll@{\hspace{6pt}}rrrrr@{\hspace{8pt}}rrrrr@{}}
\toprule
\textbf{Backbone} & \textbf{Method} 
& \multicolumn{5}{c@{\hspace{8pt}}}{\textbf{Image→Text}} 
& \multicolumn{5}{c@{}}{\textbf{Text→Image}} \\ 
\cmidrule(lr){3-7} \cmidrule(lr){8-12}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 \\ 
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Insect Dataset}}} \\[0.5pt]
CLIP & Baseline & 3.97 & 11.40 & 17.79 & 30.40 & 42.92 & 4.49 & 12.18 & 18.13 & 30.40 & 43.78 \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{PathGen Dataset}}} \\[0.5pt]
CLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & 3.10 & 12.16 & 19.67 & 34.06 & 47.46 & 3.37 & 11.32 & 18.95 & 32.92 & 46.40 \\
& +\textbf{Ours} & 3.59 & 12.83 & 20.39 & 34.88 & 48.75 & 3.82 & 12.19 & 19.89 &34.43 & 48.20 \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Sketchy Dataset}}} \\[0.5pt]
CLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DOCCI Dataset}}} \\[0.5pt]
CLIP & Baseline & 72.41 & 93.27 & -- & 99.31 & 99.76 & 72.04 & 93.37 & -- & 99.35 & 99.8 \\
& +\textbf{Ours} & 75.08 & 94.25 & 97.39 & 99.35 & 99.75 & 74.49 & 93.71 & 96.62 & 99.35 & 99.81 \\
[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DCI Dataset}}} \\[0.5pt]
CLIP & Baseline & 66.43 & 84.74 & -- & 93.8 & 96.1 & 66.58 & 86.74 & -- & 95.1 & 97.65 \\
& +\textbf{Ours} & 72.84 & 89.19 & 92.45 & 95.25 & 97.1 & 72.04 & 88.39 & 92.9 & 96.35 & 97.8 \\
[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\end{table*}
\begin{table*}[t]
\centering
\caption{Comprehensive evaluation of retrieval performance (Recall@K) across five benchmark datasets. Best results for each backbone are shown in \textbf{bold}.}
\label{tab:main_results}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.5pt}
\scriptsize
\begin{tabular}{@{}ll@{\hspace{6pt}}rrrrr@{\hspace{8pt}}rrrrr@{}}
\toprule
\textbf{Backbone} & \textbf{Method} 
& \multicolumn{5}{c@{\hspace{8pt}}}{\textbf{Image→Text}} 
& \multicolumn{5}{c@{}}{\textbf{Text→Image}} \\ 
\cmidrule(lr){3-7} \cmidrule(lr){8-12}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 \\ 
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DCI Dataset}}} \\[0.5pt]
CLIP & Baseline & 66.43 & 84.74 & -- & 93.8 & 96.1 & 66.58 & 86.74 & -- & 95.1 & 97.65 \\
& +\textbf{Ours} & 72.84 & 89.19 & 92.45 & 95.25 & 97.1 & 72.04 & 88.39 & 92.9 & 96.35 & 97.8 \\
[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DOCCI Dataset}}} \\[0.5pt]
CLIP & Baseline & 72.41 & 93.27 & -- & 99.31 & 99.76 & 72.04 & 93.37 & -- & 99.35 & 99.8 \\
& +\textbf{Ours} & 75.08 & 94.25 & 97.39 & 99.35 & 99.75 & 74.49 & 93.71 & 96.62 & 99.35 & 99.81 \\
[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Sketchy Dataset}}} \\[0.5pt]
CLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Insect Dataset}}} \\[0.5pt]
CLIP & Baseline & 3.97 & 11.40 & 17.79 & 30.40 & 42.92 & 4.49 & 12.18 & 18.13 & 30.40 & 43.78 \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{PathGen Dataset}}} \\[0.5pt]
CLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & 3.10 & 12.16 & 19.67 & 34.06 & 47.46 & 3.37 & 11.32 & 18.95 & 32.92 & 46.40 \\
& +\textbf{Ours} & 3.59 & 12.83 & 20.39 & 34.88 & 48.75 & 3.82 & 12.19 & 19.89 &34.43 & 48.20 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{Comprehensive evaluation of retrieval performance (Recall@K) across five benchmark datasets. Best results for each backbone are shown in \textbf{bold}.}
\label{tab:main_results}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.5pt}
\scriptsize
\begin{tabular}{@{}ll@{\hspace{6pt}}rrrrr@{\hspace{8pt}}rrrrr@{}}
\toprule
\textbf{Backbone} & \textbf{Method} 
& \multicolumn{5}{c@{\hspace{8pt}}}{\textbf{Image→Text}} 
& \multicolumn{5}{c@{}}{\textbf{Text→Image}} \\ 
\cmidrule(lr){3-7} \cmidrule(lr){8-12}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 \\ 
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DCI Dataset}}} \\[0.5pt]
CLIP & Baseline & 66.43 & 84.74 & -- & 93.8 & 96.1 & 66.58 & 86.74 & -- & 95.1 & 97.65 \\
& +GOAL & 72.64 & 89.89 & -- & 95.95 & 97.25 & 72.84 & 90.5 & -- & 96.6 & 97.9 \\
& +\textbf{Ours} & 72.84 & 89.19 & 92.45 & 95.25 & 97.1 & 72.04 & 88.39 & 92.9 & 96.35 & 97.8 \\
& +\textbf{GOAL +Ours} & 72.89 & 89.79 & 92.4 & 96.15 & 97.65 & 73.89 & 89.93 & 93.5 & 96.8 & 98.15 \\
[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DOCCI Dataset}}} \\[0.5pt]
CLIP & Baseline & 72.41 & 93.27 & -- & 99.31 & 99.76 & 72.04 & 93.37 & -- & 99.35 & 99.8 \\
& +GOAL & 79.47 & 96.65 & -- & 99.69 & 99.92 & 79.43 & 96.14 & -- & 99.61 & 99.9 \\
& +\textbf{Ours} & 75.08 & 94.25 & 97.39 & 99.35 & 99.75 & 74.49 & 93.71 & 96.62 & 99.35 & 99.81 \\
& +\textbf{GOAL+Ours} & 80.96 & 96.9 & 8.96 & 99.76 & 99.92 & 80.31 & 96.73 & 98.84 & 99.75 & 99.94 \\
[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Sketchy Dataset}}} \\[0.5pt]
CLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Insect Dataset}}} \\[0.5pt]
CLIP & Baseline & 3.97 & 11.40 & 17.79 & 30.40 & 42.92 & 4.49 & 12.18 & 18.13 & 30.40 & 43.78 \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{12}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{PathGen Dataset}}} \\[0.5pt]
CLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
LongCLIP & Baseline & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +GOAL & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
& +\textbf{Ours} & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\[1pt]
SigLIP-2 & Baseline & 3.10 & 12.16 & 19.67 & 34.06 & 47.46 & 3.37 & 11.32 & 18.95 & 32.92 & 46.40 \\
& +GOAL & 3.27 & 10.87 & 18.31 & 31.11 & 44.54 & 3.02 & 10.65 & 17.24 & 30.96 & 44.69 \\
& +\textbf{Ours} & 3.59 & 12.83 & 20.39 & 34.88 & 48.75 & 3.82 & 12.19 & 19.89 &34.43 & 48.20 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table}[h!]
\centering
\small
\caption{Retrieval performance comparison between \textbf{patch-chunk} and \textbf{SAM-seg}. 
$\Delta$ denotes the difference (\textbf{SAM-seg} $-$ \textbf{patch-chunk}). 
Positive $\Delta$ indicates SAM-seg performs better.}
\vspace{3pt}
\begin{tabular}{lcc}
\toprule
\textbf{Task} & \textbf{Setting} & \textbf{Recall@K (\%)} \\
\midrule
\multirow{3}{*}{\textbf{Text $\rightarrow$ Image}} 
 & patch-chunk & R@1 = 7.86,\ R@5 = 24.35,\ R@10 = 36.53,\ R@25 = 54.15,\ R@50 = 67.53 \\
 & SAM-seg     & R@1 = 7.77,\ R@5 = 25.99,\ R@10 = 37.56,\ R@25 = 55.96,\ R@50 = 68.57 \\
 & $\Delta$ (SAM-seg $-$ patch-chunk) & R@1 = \textbf{-0.09},\ R@5 = \textbf{+1.64},\ R@10 = \textbf{+1.03},\ R@25 = \textbf{+1.81},\ R@50 = \textbf{+1.04} \\
\midrule
\multirow{3}{*}{\textbf{Image $\rightarrow$ Text}} 
 & patch-chunk & R@1 = 8.55,\ R@5 = 25.13,\ R@10 = 36.79,\ R@25 = 53.97,\ R@50 = 67.18 \\
 & SAM-seg     & R@1 = 7.34,\ R@5 = 25.99,\ R@10 = 37.31,\ R@25 = 54.32,\ R@50 = 68.13 \\
 & $\Delta$ (SAM-seg $-$ patch-chunk) & R@1 = \textbf{-1.21},\ R@5 = \textbf{+0.86},\ R@10 = \textbf{+0.52},\ R@25 = \textbf{+0.35},\ R@50 = \textbf{+0.95} \\
\bottomrule
\end{tabular}
\label{tab:retrieval_comparison}
\end{table}



\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lccccc|ccccc}
\toprule
\multirow{2}{*}{Loss config} & \multicolumn{5}{c}{Text $\rightarrow$ Image (Recall@\%)} & \multicolumn{5}{c}{Image $\rightarrow$ Text (Recall@\%)} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
& R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 \\
\midrule
None(CLIP + Global finetuning)               & 9.24 & 24.09 & 34.37 & 53.63 & 67.27 & 8.46 & 24.78 & 35.41 & 51.38 & 65.03 \\
ST                 & 8.12 & \underline{26.51} & 37.31 & \underline{55.44} & 67.27 & 8.46 & \underline{26.86} & 37.74 & 54.32 & 67.70 \\
RS                 & 6.99 & 24.35 & 34.11 & 53.20 & 65.89 & 7.77 & 24.53 & 35.92 & 52.25 & 65.11 \\
Chunk              & 9.15 & 25.73 & 36.96 & 54.75 & 67.27 & \underline{8.81} & 26.25 & 37.65 & 54.23 & 67.36 \\
ST + RS            & 9.07 & \underline{26.51} & 37.22 & 53.71 & 68.57 & 7.94 & 26.68 & 37.48 & 53.97 & 67.44 \\
ST + Chunk         & 9.33 & 25.47 & 36.53 & \underline{55.44} & \underline{69.00} & 8.55 & \underline{26.86} & 38.34 & \textbf{55.27} & 67.53 \\
RS + Chunk         & 9.07 & 25.47 & \underline{38.17} & 54.75 & 68.83 & 8.03 & \textbf{27.81} & \underline{38.60} & 54.49 & \textbf{69.00} \\
ST + RS + Chunk    & \textbf{9.93} & \textbf{26.60} & \textbf{38.34} & \textbf{56.99} & \textbf{69.34} & \textbf{9.50} & 26.60 & \textbf{39.64} & \underline{54.92} & \underline{68.65} \\
ST + RS + Chunk (maybe better)    & \textbf{9.84} & \textbf{26.94} & \textbf{39.12} & \textbf{56.91} & \textbf{70.03} & \textbf{9.07} & 27.72 & \textbf{41.11} & \textbf{56.65} & \underline{68.31} \\


\midrule
GOAL               & 8.46 & 24.09 & 34.72 & 53.71 & 67.96 & 8.64 & 24.87 & 36.36 & 53.28 & 66.75 \\
GOAL  + Ours             & 10.71 & 26.25 & 38.77 & 56.82 & 70.73 & 8.38 & 27.46 & 39.64 & 57.43 & 70.03\\
\midrule
CLIP + LoRA               & 5.09 & 16.15 & 25.73 & 42.06 & 55.61 & 5.27 & 15.98 & 25.39 & 40.50 & 55.79 \\
CLIP + LoRA + Ours              & 6.04 & 18.57 & 27.55 & 44.91 & 59.07 & 5.44 & 18.39 & 27.98 & 44.82 & 56.30 \\
\bottomrule
\end{tabular}
\caption{Retrieval performance on the INSECT split (1{,}158 images / 1{,}158 texts). ST: scribble--text; RS: RGB--scribble consistency; Chunk: chunk--segment alignment. Best per column in \textbf{bold}, second best \underline{underlined}.}
\label{tab:loss_ablation}
\end{table}


\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{rlrrrrr|rrrrr|rrr}
\toprule
\# & Setting & \multicolumn{5}{c|}{Text $\rightarrow$ Image (Recall \%)} & \multicolumn{5}{c|}{Image $\rightarrow$ Text (Recall \%)} & \multicolumn{3}{c}{Averages} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-15}
 &  & R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 & T$\rightarrow$I & I$\rightarrow$T & Overall \\
\midrule
1 & Remove color+texture & 70.69 & 87.89 & 91.55 & 95.40 & 96.80 & 68.88 & 87.49 & 92.30 & 95.80 & 97.65 & 88.47 & 88.42 & 88.45 \\
2 & Remove only color & 71.29 & 88.14 & 91.90 & 95.15 & 96.90 & 70.64 & 87.64 & 91.95 & 95.95 & \textbf{97.85} & 88.68 & 88.81 & 88.74 \\
3 & Remove only material & 71.59 & 88.09 & 92.10 & 94.80 & 96.75 & \textbf{71.24} & 88.34 & 92.25 & 96.00 & 97.40 & 88.67 & 89.05 & 88.86 \\
4 & Remove only texture & 71.44 & 88.59 & 92.25 & 95.05 & 97.00 & 70.74 & 88.39 & 91.95 & 95.90 & 97.55 & 88.87 & 88.91 & 88.89 \\
5 & Remove none & 71.39 & \textbf{88.69} & 92.05 & 95.25 & 96.90 & 70.19 & 88.29 & 92.55 & 96.10 & 97.50 & 88.86 & 88.93 & 88.91 \\
6 & Remove all & 71.19 & \textbf{88.84} & \textbf{92.60} & 95.50 & 97.15 & 69.78 & 88.59 & 92.90 & \textbf{96.55} & 97.70 & 89.06 & 89.10 & 89.08 \\
7 & Remove color+material & 71.74 & 88.64 & 92.50 & 95.70 & 97.35 & 70.79 & 88.04 & 92.35 & 96.35 & 97.80 & \textbf{89.19} & 89.07 & 89.13 \\
8 & Remove material+texture & \textbf{72.99} & 88.44 & 91.95 & \textbf{95.90} & \textbf{97.55} & 69.73 & 88.34 & \textbf{92.90} & 96.20 & \textbf{98.15} & 89.37 & 89.06 & \textbf{89.22} \\
\bottomrule
\end{tabular}
\caption{DCI ablations sorted from lowest to highest overall performance (Overall = mean of all 10 recall values per setting). Bold indicates the best value in each column.}
\label{tab:dci_ablations_sorted}
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{rlrrrrr|rrrrr|rrr}
\toprule
\# & Setting & \multicolumn{5}{c|}{Text $\rightarrow$ Image (Recall \%)} & \multicolumn{5}{c|}{Image $\rightarrow$ Text (Recall \%)} & \multicolumn{3}{c}{Averages} \\
\cmidrule(lr){3-7}\cmidrule(lr){8-12}\cmidrule(lr){13-15}
 &  & R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 & T$\rightarrow$I & I$\rightarrow$T & Overall \\
\midrule
1 & Remove none & 72.10 & 93.10 & 97.04 & 99.16 & 99.76 & 71.29 & 92.14 & 96.41 & 98.80 & 99.55 & 92.23 & 91.64 & 91.93 \\
2 & Remove color material & 73.24 & 93.53 & 97.20 & 99.20 & 99.75 & 73.29 & 92.84 & 96.59 & 98.69 & 99.59 & 92.58 & 92.20 & 92.39 \\
3 & Remove material texture & 73.00 & 93.78 & 97.25 & 99.41 & 99.80 & 73.35 & 93.14 & 96.71 & 99.10 & 99.73 & 92.65 & 92.41 & 92.53 \\
4 & Remove color & 73.43 & 94.00 & 97.27 & 99.25 & 99.78 & 73.16 & 93.00 & 97.02 & 98.96 & 99.65 & 92.75 & 92.36 & 92.56 \\
5 & Remove material & 75.43 & 94.71 & 97.65 & 99.47 & 99.86 & 74.49 & 94.08 & 97.31 & 99.33 & 99.73 & 93.42 & 92.99 & 93.21 \\
6 & Remove texture & 75.82 & 95.00 & 97.98 & 99.41 & 99.84 & 75.53 & 94.37 & 97.49 & 99.25 & 99.69 & 93.61 & 93.27 & 93.44 \\
7 & Remove color texture & \textbf{77.02} & 94.84 & 97.84 & 99.51 & 99.84 & 75.55 & 94.22 & 97.39 & 99.29 & 99.73 & \textbf{93.81} & 93.24 & 93.52 \\
8 & Remove all & 75.98 & \textbf{95.16} & \textbf{98.18} & \textbf{99.59} & \textbf{99.88} & \textbf{76.12} & \textbf{94.47} & \textbf{97.65} & \textbf{99.37} & \textbf{99.80} & 93.76 & \textbf{93.48} & \textbf{93.62} \\
\bottomrule
\end{tabular}
\caption{DOCCI ablations sorted from lowest to highest overall performance (Overall = mean of all 10 recall values per setting). Bold indicates the best value in each column.}
\label{tab:docci_ablations_sorted}
\end{table*}


% 17/10 result
% Table 1: Full finetune vs +Ours across backbones
% =========================
\begin{table*}[t]
\centering
\caption{\textbf{Full-parameter finetuning vs. +Ours (SAS)} across backbones and datasets (Recall@K, \%). 
Columns on the left: Image$\rightarrow$Text; right: Text$\rightarrow$Image. 
Best per-backbone in \textbf{bold}. Values are left as ``—'' for later fill-in. 
\textbf{Avg} is the mean of R@\{1,5,10,25,50\} within each direction.}
\label{tab:fullft_main}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.5pt}
\scriptsize
\begin{tabular}{@{}ll@{\hspace{6pt}}rrrrrr@{\hspace{8pt}}rrrrrr@{}}
\toprule
\textbf{Backbone} & \textbf{Method} 
& \multicolumn{6}{c@{\hspace{8pt}}}{\textbf{Text$\rightarrow$Image}} 
& \multicolumn{6}{c@{}}{\textbf{Image$\rightarrow$Text}} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 & \footnotesize Avg
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 & \footnotesize Avg \\
\midrule

\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Sketchy}}} \\[0.5pt]
CLIP   & Full-FT      
& 64.68 & 88.86 & 93.44 & 98.19 & 99.40 & 88.91 
& 63.90 & 87.74 & 93.01 & 97.50 & 98.22 & 88.07 \\
       & +\textbf{Ours} 
& \best{68.31}\gain{3.63} & \best{90.16}\gain{1.30} & \best{94.99}\gain{1.55} & \best{98.79}\gain{0.60} & \best{99.48}\gain{0.08} & \best{90.35}\gain{1.44}
& \best{65.03}\gain{1.13} & \best{89.90}\gain{2.16} & \best{94.47}\gain{1.46} & \best{97.89}\gain{0.39} & \best{99.14}\gain{0.92} & \best{89.29}\gain{1.22} \\
LongCLIP & Full-FT    
& \best{66.41} & \best{86.44} & \best{91.97} & \best{96.37} & \best{98.01} & \best{87.84}
& \best{66.67} & \best{87.82} & \best{92.83} & \best{96.89} & \best{98.27} & \best{88.50} \\
         & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\
SigLIP-2 & Full-FT     
& 68.91 & 90.85 & 95.16 & \best{98.79} & 99.57 & \best{90.66}
& 66.75 & 90.24 & 93.96 & \best{98.10} & 99.31 & \best{89.67} \\
         & +\textbf{Ours} 
& \best{73.49}\gain{4.58} & \best{91.97}\gain{1.12} & \best{95.77}\gain{0.61} & \best{98.79} & \best{99.60}\gain{0.03} & —
& \best{70.38}\gain{3.63} & \best{91.54}\gain{1.30} & \best{95.77}\gain{1.81} & \best{98.10} & \best{99.35}\gain{0.04} & — \\

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Insect}}} \\[0.5pt]
CLIP   & Full-FT      
& 8.38 & 25.73 & 35.06 & 51.30 & 64.51 & 37.00 
& 8.72 & \best{26.60} & 36.36 & 51.30 & 63.64 & 37.32 \\
       & +\textbf{Ours} 
& \best{9.93}\gain{1.55} & \best{26.60}\gain{0.87} & \best{38.34}\gain{3.28} & \best{56.99}\gain{5.69} & \best{69.34}\gain{4.83} & \best{40.24}\gain{3.24}
& \best{9.50}\gain{0.78} & \best{26.60} & \best{39.64}\gain{3.28} & \best{54.92}\gain{3.62} & \best{68.65}\gain{5.01} & \best{39.86}\gain{2.54} \\
LongCLIP & Full-FT    
& \best{4.06} & 12.18 & 18.91 & 31.17 & 41.62 & 21.59
& 3.89 & 10.97 & 18.31 & 29.62 & 43.78 & 21.31 \\
         & +\textbf{Ours} 
& 3.97\loss{0.09} & \best{12.87}\gain{0.69} & \best{19.86}\gain{0.95} & \best{32.88}\gain{1.71} & \best{46.29}\gain{4.67} & \best{23.17}\gain{1.58}
& \best{4.49}\gain{0.60} & \best{13.73}\gain{2.76} & \best{20.12}\gain{1.81} & \best{33.51}\gain{3.89} & \best{46.63}\gain{2.85} & \best{23.70}\gain{2.39} \\
SigLIP-2 & Full-FT     
& 6.37 & 21.07 & 31.87 & 48.19 & 60.36 & 33.57
& 6.56 & 21.85 & 31.95 & 49.22 & 60.19 & 33.95 \\
         & +\textbf{Ours} 
& \best{7.69}\gain{1.32} & \best{23.49}\gain{2.42} & \best{33.42}\gain{1.55} & \best{50.52}\gain{2.33} & \best{63.04}\gain{2.68} & \best{35.63}\gain{2.06}
& \best{6.99}\gain{0.43} & \best{23.66}\gain{1.81} & \best{35.06}\gain{3.11} & \best{52.16}\gain{2.94} & \best{63.21}\gain{3.02} & \best{36.22}\gain{2.27} \\

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{PathGen}}} \\[0.5pt]
CLIP   & Full-FT      
& 3.96 & 13.55 & 21.87 & 36.56 & 50.46 & 25.38
& 3.62 & 13.13 & 20.49 & 35.52 & 49.62 & 24.48 \\
       & +\textbf{Ours} 
& \best{4.14}\gain{0.18} & \best{14.24}\gain{0.69} & \best{22.87}\gain{1.00} & \best{37.55}\gain{0.99} & \best{50.73}\gain{0.27} & \best{25.91}\gain{0.53}
& \best{3.77}\gain{0.15} & \best{13.15}\gain{0.02} & \best{21.35}\gain{0.86} & \best{37.03}\gain{1.51} & \best{49.79}\gain{0.17} & \best{25.02}\gain{0.54} \\
LongCLIP & Full-FT    
& \best{0.99} & \best{5.20} & \best{8.94} & \best{17.29} & \best{27.92} & — 
& \best{1.29} & \best{5.05} & \best{8.94} & \best{17.36} & \best{26.95} & — \\
         & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\
SigLIP-2 & Full-FT     
& \best{3.86} & \best{13.48} & \best{21.20} & \best{35.47} & \best{48.72} & \best{24.55}
& \best{3.47} & \best{12.36} & \best{19.54} & \best{34.65} & \best{48.15} & \best{23.63} \\
         & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DCI}}} \\[0.5pt]
CLIP   & Full-FT      
& \best{66.43} & \best{84.74} & — & \best{93.8} & \best{96.1} & — 
& \best{66.58} & \best{86.74} & — & \best{95.1} & \best{97.65} & — \\
       & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\
LongCLIP & Full-FT    
& \best{71.44} & \best{87.79} & \best{91.95} & \best{94.80} & \best{97.10} & \best{88.62}
& \best{69.78} & \best{87.99} & \best{91.75} & \best{95.40} & \best{97.15} & \best{88.41} \\
         & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\
SigLIP-2 & Full-FT     
& 66.13 & 84.49 & 89.34 & 94.00 & 96.40 & 86.07
& 65.08 & 84.54 & 89.84 & 94.65 & \best{96.95} & 86.21 \\
         & +\textbf{Ours} 
& \best{67.14}\gain{1.01} & \best{86.54}\gain{2.05} & \best{90.65}\gain{1.31} & \best{94.87}\gain{0.87} & \best{96.85}\gain{0.45} & \best{87.30}\gain{1.23}
& \best{66.78}\gain{1.70} & \best{86.09}\gain{1.55} & \best{90.50}\gain{0.66} & \best{94.75}\gain{0.10} & 96.90\loss{0.05} & \best{87.00}\gain{0.79} \\

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DOCCI}}} \\[0.5pt]
CLIP   & Full-FT      
& \best{72.1} & \best{93.27} & — & \best{99.31} & \best{99.76} & — 
& \best{72.04} & \best{93.37} & — & \best{99.35} & \best{99.8} & — \\
       & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\
LongCLIP & Full-FT    
& \best{79.53} & \best{95.94} & \best{98.39} & \best{99.61} & \best{99.88} & \best{94.67}
& \best{77.45} & \best{95.84} & \best{98.37} & \best{99.57} & \best{99.86} & \best{94.22} \\
         & +\textbf{Ours} 
& — & — & — & — & — & — & — & — & — & — & — & — \\
SigLIP-2 & Full-FT     
& 71.80 & 92.53 & 95.88 & 98.78 & 99.43 & 91.68
& 71.51 & 92.41 & 96.06 & 98.51 & 99.39 & 91.58 \\
         & +\textbf{Ours} 
& \best{75.47}\gain{3.67} & \best{94.82}\gain{2.29} & \best{97.67}\gain{1.79} & \best{99.33}\gain{0.55} & \best{99.78}\gain{0.35} & \best{93.41}\gain{1.73}
& \best{73.59}\gain{2.08} & \best{94.33}\gain{1.92} & \best{97.43}\gain{1.37} & \best{99.37}\gain{0.86} & \best{99.84}\gain{0.45} & \best{92.91}\gain{1.33} \\
\bottomrule
\end{tabular}
\end{table*}


==> sec/old/4_experiments10.29.tex <==

% =========================
% Experiments
% =========================
\section{Experiments}
\label{sec:exp}

\subsection{Setup}
\paragraph{Backbones and training.}
Unless otherwise noted, we use ViT-B/16 backbones initialized from public checkpoints (CLIP, SigLIP, LongCLIP, SigLIP-2). 
Inputs are resized to $224^2$. For fair comparison, all methods share the same text templates, tokenizer, batch size, and training budget. 
Results are averaged over 3 seeds; we report mean values (and optionally $\pm$std in the appendix).

\paragraph{Datasets.}
We evaluate on five benchmarks with different structural biases: DCI, DOCCI (general domain), and three structure-sensitive sets—Sketchy, Insect, PathGen.

\paragraph{Tasks and metrics.}
We report cross-modal retrieval (Text$\rightarrow$Image / Image$\rightarrow$Text) with Recall@K (K=1/5/10/25/50). 
For segmentation transfer, we use train-free ClipTrASE decoding and report IoU, Dice, oIoU, and Boundary IoU (BIoU).

\paragraph{Compared methods.}
\textbf{Global finetune (Full-FT)}: full-parameter end-to-end finetuning; 
\textbf{Adapters}: LoRA/DoRA on the text/vision towers and projection heads; 
\textbf{GOAL}: a recent geometric-aware alignment baseline; 
\textbf{Ours (SAS)}: edge-aware auxiliary objectives added on top of the base training recipe.



% % =========================
% % Table 1: Full finetune vs +Ours across backbones
% % =========================
\begin{table*}[t]
\centering
\caption{
\textbf{Finetuning variants on CLIP across datasets} (Recall@K, \%). 
Left: Text$\rightarrow$Image; Right: Image$\rightarrow$Text. 
\textbf{Avg} is the mean of R@\{1,5,10,25,50\}.
}
\label{tab:reformat_main_cliponly}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\scriptsize
\begin{tabular}{@{}l@{\hspace{6pt}}l@{\hspace{6pt}}rrrrrr@{\hspace{8pt}}rrrrrr@{}}
\toprule
\textbf{BB} & \textbf{Method} 
& \multicolumn{6}{c@{\hspace{8pt}}}{\textbf{Text$\rightarrow$Image}} 
& \multicolumn{6}{c@{}}{\textbf{Image$\rightarrow$Text}} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50  \\
\midrule

% ==================== SKETCHY ====================
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Sketchy}}} \\[0.5pt]
\multirow{5}{*}{\rotatebox{90}{\textbf{FFT}}} & longclip-ft  & 54.32 & 80.14 & 88.43 & 95.25 & 98.27 & 52.76 & 80.31 & 88.08 & 95.16 & 97.75  \\
& smartclip-ft & 50.73 & 81.09 & 94.56 & 96.11 & 99.05 & 51.30 & 80.83 & 94.04 & 95.51 & 98.96 \\
& GOAL-FT      & 63.21 & 87.13 & 93.44 & 97.67 & 99.05 & 62.44 & 87.82 & 92.31 & 96.98 & 99.40  \\
& globa-ft     & — & — & — & — & — & — & — & — & — & — & — & — \\
& Ours         & — & — & — & — & — & — & — & — & — & — & — & — \\
\cmidrule(lr){2-14}
\multirow{4}{*}{\rotatebox{90}{\textbf{PEFT}}} & LoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& DoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& LORA\_OURS   & — & — & — & — & — & — & — & — & — & — & — & — \\
& DORA+OURS    & — & — & — & — & — & — & — & — & — & — & — & — \\

% ==================== INSECT ====================
\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Insect}}} \\[0.5pt]
\multirow{5}{*}{\rotatebox{90}{\textbf{FFT}}} & longclip-ft  & 8.20 & 23.83 & 34.97 & 51.21 & 63.30 & 9.41 & 24.78 & 37.31 & 53.18 & 63.39  \\
& smartclip-ft & 4.84 & 16.84 & 34.63 & 39.03 & 57.60 & 4.66 & 15.46 & 34.02 & 39.72 & 58.38 \\
& GOAL-FT      & 8.81 & 24.35 & 35.84 & 55.44 & 67.36 & 8.55 & 25.91 & 36.18 & 53.02 & 66.41 \\
& globa-ft     & — & — & — & — & — & — & — & — & — & — & — & — \\
& Ours         & — & — & — & — & — & — & — & — & — & — & — & — \\
\cmidrule(lr){2-14}
\multirow{4}{*}{\rotatebox{90}{\textbf{PEFT}}} & LoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& DoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& LORA\_OURS   & — & — & — & — & — & — & — & — & — & — & — & — \\
& DORA+OURS    & — & — & — & — & — & — & — & — & — & — & — & — \\

% ==================== DCI ====================

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DCI}}} \\[0.5pt]
\multirow{5}{*}{\rotatebox{90}{\textbf{FFT}}} & longclip-ft  & 59.23 & 80.89 & 87.04 & 92.60 & 95.10 & 60.13 & 81.44 & 87.54 & 92.85 & 95.60  \\
& smartclip-ft & 69.88 & 86.64 & 94.05 & 95.00 &97.25 & 70.94 & 87.04 & 94.60 & 95.75 & 98.05\\
& GOAL-FT      & — & — & — & — & — & — & — & — & — & — & — & — \\
& globa-ft     & — & — & — & — & — & — & — & — & — & — & — & — \\
& Ours         & — & — & — & — & — & — & — & — & — & — & — & — \\
\cmidrule(lr){2-14}
\multirow{4}{*}{\rotatebox{90}{\textbf{PEFT}}} & LoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& DoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& LORA\_OURS   & — & — & — & — & — & — & — & — & — & — & — & — \\
& DORA+OURS    & — & — & — & — & — & — & — & — & — & — & — & — \\

% ==================== DOCCI ====================
\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Docci}}} \\[0.5pt]
\multirow{5}{*}{\rotatebox{90}{\textbf{FFT}}} & longclip-ft  & 64.49 & 87.67 & 93.43 & 97.73 & 99.14 & 63.08 & 87.45 & 93.14 & 97.45 & 99.02 \\
& smartclip-ft & 74.92 & 94.08 & 98.96 & 99.37 & 99.82 & 74.91 & 94.04 & 98.98 & 99.32 & 99.84  \\


& GOAL-FT      & 79.47 & 96.65 & — & 99.69 & 99.92 & 79.43 & 96.14 & — & 99.61 & 99.90  \\
& globa-ft     & — & — & — & — & — & — & — & — & — & — & — & — \\
& Ours         & — & — & — & — & — & — & — & — & — & — & — & — \\
\cmidrule(lr){2-14}
\multirow{4}{*}{\rotatebox{90}{\textbf{PEFT}}} & LoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& DoRA         & — & — & — & — & — & — & — & — & — & — & — & — \\
& LORA\_OURS   & — & — & — & — & — & — & — & — & — & — & — & — \\
& DORA+OURS    & — & — & — & — & — & — & — & — & — & — & — & — \\

\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\caption{
\textbf{Full-parameter finetuning vs. +Ours (SAS)} across backbones and datasets (Recall@K, \%). 
Left: Image$\rightarrow$Text; Right: Text$\rightarrow$Image. 
Backbone cells are color-coded (\cellcolor{morandiblue!20}CLIP, \cellcolor{morandigreen!20}LongCLIP, \cellcolor{morandipink!20}SigLIP-2). 
$\Delta$ denotes absolute improvement (\textit{positive in blue, negative in red}) over Full-FT. 
\textbf{Avg} is the mean of R@\{1,5,10,25,50\}.
}
\label{tab:fullft_main}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.5pt}
\scriptsize
\begin{tabular}{@{}ll@{\hspace{6pt}}rrrrrr@{\hspace{8pt}}rrrrrr@{}}
\toprule
\textbf{Backbone} & \textbf{Method} 
& \multicolumn{6}{c@{\hspace{8pt}}}{\textbf{Text$\rightarrow$Image}} 
& \multicolumn{6}{c@{}}{\textbf{Image$\rightarrow$Text}} \\
\cmidrule(lr){3-8} \cmidrule(lr){9-14}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 & \footnotesize Avg
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 & \footnotesize R@25 & \footnotesize R@50 & \footnotesize Avg \\
\midrule

% ==================== SKETCHY ====================
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Sketchy}}} \\[0.5pt]
\cellcolor{morandiblue!20} & Full-FT      
& 64.68 & 88.86 & 93.44 & 98.19 & 99.40 & 88.91 
& 63.90 & 87.74 & 93.01 & 97.50 & 98.22 & 88.07 \\
\cellcolor{morandiblue!20}\textbf{CLIP} & +\textbf{Ours} 
& \textbf{68.31} & \textbf{90.16} & \textbf{94.99} & \textbf{98.79} & \textbf{99.48} & \textbf{90.35}
& \textbf{65.03} & \textbf{89.90} & \textbf{94.47} & \textbf{97.89} & \textbf{99.14} & \textbf{89.29} \\
\cellcolor{morandiblue!20} & $\Delta$ &
\dblue{+3.63} & \dblue{+1.30} & \dblue{+1.55} & \dblue{+0.60} & \dblue{+0.08} & \dblue{+1.44} &
\dblue{+1.13} & \dblue{+2.16} & \dblue{+1.46} & \dblue{+0.39} & \dblue{+0.92} & \dblue{+1.22} \\

\cellcolor{morandigreen!20} & Full-FT    
& 66.41 & 86.44 & 91.97 & 96.37 & 98.01 & 87.84
& 66.67 & 87.82 & 92.83 & 96.89 & 98.27 & 88.50 \\
\cellcolor{morandigreen!20}\textbf{LongCLIP} & +\textbf{Ours} 
& \textit{68.39} & \textit{89.46} & \textit{94.39} & \textit{98.27} & \textit{99.22} & \textit{—} &
\textit{67.88} & \textit{89.72} & \textit{93.96} & \textit{98.10} & \textit{98.99} & \textit{—} \\
\cellcolor{morandigreen!20} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\

\cellcolor{morandipink!70} & Full-FT     
& 68.91 & 90.85 & 95.16 & \textbf{98.79} & 99.57 & \textbf{90.66}
& 66.75 & 90.24 & 93.96 & \textbf{98.10} & 99.31 & \textbf{89.67} \\
\cellcolor{morandipink!70}\textbf{SigLIP-2} & +\textbf{Ours} 
& \textbf{73.49} & \textbf{91.97} & \textbf{95.77} & \textbf{98.79} & \textbf{99.60} & \textbf{91.52}
& \textbf{70.38} & \textbf{91.54} & \textbf{95.77} & \textbf{98.10} & \textbf{99.35} & \textbf{91.03} \\
\cellcolor{morandipink!70} & $\Delta$ &
\dblue{+4.58} & \dblue{+1.12} & \dblue{+0.61} & \textit{—} & \dblue{+0.03} & \dblue{+0.86} &
\dblue{+3.63} & \dblue{+1.30} & \dblue{+1.81} & \textit{—} & \dblue{+0.04} & \dblue{+1.36} \\

% ==================== INSECT ====================
\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Insect}}} \\[0.5pt]
\cellcolor{morandiblue!20} & Full-FT      
& 8.38 & 25.73 & 35.06 & 51.30 & 64.51 & 37.00 
& 8.72 & 26.60 & 36.36 & 51.30 & 63.64 & 37.32 \\
\cellcolor{morandiblue!20}\textbf{CLIP} & +\textbf{Ours} 
& \textbf{9.93} & \textbf{26.60} & \textbf{38.34} & \textbf{56.99} & \textbf{69.34} & \textbf{40.24}
& \textbf{9.50} & \textbf{26.60} & \textbf{39.64} & \textbf{54.92} & \textbf{68.65} & \textbf{39.86} \\
\cellcolor{morandiblue!20} & $\Delta$ &
\dblue{+1.55} & \dblue{+0.87} & \dblue{+3.28} & \dblue{+5.69} & \dblue{+4.83} & \dblue{+3.24} &
\dblue{+0.78} & \textit{—} & \dblue{+3.28} & \dblue{+3.62} & \dblue{+5.01} & \dblue{+2.54} \\

\cellcolor{morandigreen!20} & Full-FT    
& 4.06 & 12.18 & 18.91 & 31.17 & 41.62 & 21.59
& 3.89 & 10.97 & 18.31 & 29.62 & 43.78 & 21.31 \\
\cellcolor{morandigreen!20}\textbf{LongCLIP} & +\textbf{Ours} 
& 3.97 & 12.87 & 19.86 & 32.88 & 46.29 & \textbf{23.17} &
\textbf{4.49} & \textbf{13.73} & \textbf{20.12} & \textbf{33.51} & \textbf{46.63} & \textbf{23.70} \\
\cellcolor{morandigreen!20} & $\Delta$ &
\dloss{-0.09} & \dblue{+0.69} & \dblue{+0.95} & \dblue{+1.71} & \dblue{+4.67} & \dblue{+1.58} &
\dblue{+0.60} & \dblue{+2.76} & \dblue{+1.81} & \dblue{+3.89} & \dblue{+2.85} & \dblue{+2.39} \\

\cellcolor{morandipink!70} & Full-FT     
& 6.37 & 21.07 & 31.87 & 48.19 & 60.36 & 33.57
& 6.56 & 21.85 & 31.95 & 49.22 & 60.19 & 33.95 \\
\cellcolor{morandipink!70}\textbf{SigLIP-2} & +\textbf{Ours} 
& \textbf{7.69} & \textbf{23.49} & \textbf{33.42} & \textbf{50.52} & \textbf{63.04} & \textbf{35.63}
& \textbf{6.99} & \textbf{23.66} & \textbf{35.06} & \textbf{52.16} & \textbf{63.21} & \textbf{36.22} \\
\cellcolor{morandipink!70} & $\Delta$ &
\dblue{+1.32} & \dblue{+2.42} & \dblue{+1.55} & \dblue{+2.33} & \dblue{+2.68} & \dblue{+2.06} &
\dblue{+0.43} & \dblue{+1.81} & \dblue{+3.11} & \dblue{+2.94} & \dblue{+3.02} & \dblue{+2.27} \\

% ==================== PATHGEN ====================
\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{PathGen}}} \\[0.5pt]
\cellcolor{morandiblue!20} & Full-FT &
3.96 & 13.55 & 21.87 & 36.56 & 50.46 & 25.38 &
3.62 & 13.13 & 20.49 & 35.52 & 49.62 & 24.48 \\
\cellcolor{morandiblue!20}\textbf{CLIP} & +\textbf{Ours} &
\textbf{4.14} & \textbf{14.24} & \textbf{22.87} & \textbf{37.55} & \textbf{50.73} & \textbf{25.91} &
\textbf{3.77} & \textbf{13.15} & \textbf{21.35} & \textbf{37.03} & \textbf{49.79} & \textbf{25.02} \\
\cellcolor{morandiblue!20} & $\Delta$ &
\dblue{+0.18} & \dblue{+0.69} & \dblue{+1.00} & \dblue{+0.99} & \dblue{+0.27} & \dblue{+0.53} &
\dblue{+0.15} & \dblue{+0.02} & \dblue{+0.86} & \dblue{+1.51} & \dblue{+0.17} & \dblue{+0.54} \\

\cellcolor{morandigreen!20} & Full-FT &
\textbf{0.99} & \textbf{5.20} & \textbf{8.94} & \textbf{17.29} & \textbf{27.92} & \textit{—} &
\textbf{1.29} & \textbf{5.05} & \textbf{8.94} & \textbf{17.36} & \textbf{26.95} & \textit{—} \\
\cellcolor{morandigreen!20}\textbf{LongCLIP} & +\textbf{Ours} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\
\cellcolor{morandigreen!20} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\

\cellcolor{morandipink!70} & Full-FT &
\textbf{3.86} & \textbf{13.48} & \textbf{21.20} & \textbf{35.47} & \textbf{48.72} & \textbf{24.55} &
\textbf{3.47} & \textbf{12.36} & \textbf{19.54} & \textbf{34.65} & \textbf{48.15} & \textbf{23.63} \\
\cellcolor{morandipink!70}\textbf{SigLIP-2} & +\textbf{Ours} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\
\cellcolor{morandipink!70} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\

% ==================== DCI ====================

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DCI}}} \\[0.5pt]
\cellcolor{morandiblue!20} & Full-FT &
\textbf{75.64} & \textbf{89.39} & \textit{93.15} & \textbf{95.75} & \textbf{97.45} & \textit{—} &
\textbf{73.99} & \textbf{89.74} & \textit{93.30} & \textbf{96.50} & \textbf{98.00} & \textit{—} \\
\cellcolor{morandiblue!20}\textbf{CLIP} & +\textbf{Ours} &
\textit{75.90} & \textit{90.00} & \textit{93.15} & \textit{95.95} & \textit{97.75} & \textit{—} &
\textit{74.39} & \textit{89.89} & \textit{94.30} & \textit{96.75} & \textit{97.75} & \textit{—} \\
\cellcolor{morandiblue!20} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\

\cellcolor{morandigreen!20} & Full-FT &
70.39 & 87.44 &  91.40 &  95.50 &  97.10 &  88.62 &
 68.18 &  87.24 &  91.75 &  95.40 &  97.15 &  88.41 \\
\cellcolor{morandigreen!20}\textbf{LongCLIP} & +\textbf{Ours} &
\textbf{71.64} & \textbf{88.74} & \textbf{92.55} & \textbf{95.85} & \textbf{97.35} & —& \textbf{70.29} &
\textbf{87.64} & \textbf{91.80} & \textbf{95.65} & \textbf{97.30} & —  \\
\cellcolor{morandigreen!20} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\

\cellcolor{morandipink!70} & Full-FT &
66.13 & 84.49 & 89.34 & 94.00 & 96.40 & 86.07 &
65.08 & 84.54 & 89.84 & 94.65 & \textbf{96.95} & 86.21 \\
\cellcolor{morandipink!70}\textbf{SigLIP-2} & +\textbf{Ours} &
\textbf{67.14} & \textbf{86.54} & \textbf{90.65} & \textbf{94.87} & 96.85 & \textbf{87.30} &
\textbf{66.78} & \textbf{86.09} & \textbf{90.50} & \textbf{94.75} & 96.90 & \textbf{87.00} \\
\cellcolor{morandipink!70} & $\Delta$ &
\dblue{+1.01} & \dblue{+2.05} & \dblue{+1.31} & \dblue{+0.87} & \dblue{+0.45} & \dblue{+1.23} &
\dblue{+1.70} & \dblue{+1.55} & \dblue{+0.66} & \dblue{+0.10} & \dloss{-0.05} & \dblue{+0.79} \\

% ==================== DOCCI ====================

\midrule
\multicolumn{14}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{DOCCI}}} \\[0.5pt]
\cellcolor{morandiblue!20} & Full-FT &
\textbf{80.38} & \textbf{96.45} & \textit{98.76} & \textbf{99.75} & \textbf{99.94} & \textit{—} &
\textbf{79.43} & \textbf{96.51} & \textit{98.69} & \textbf{99.71} & \textbf{99.94} & \textit{—} \\
\cellcolor{morandiblue!20}\textbf{CLIP} & +\textbf{Ours} &
\textit{83.04} & \textit{97.06} & \textit{98.96} & \textit{99.84} & \textit{99.98} & \textit{—} &
\textit{81.59} & \textit{96.94} & \textit{98.78} & \textit{99.76} & \textit{99.92} & \textit{—} \\
\cellcolor{morandiblue!20} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\


\cellcolor{morandigreen!20} & Full-FT &
\textbf{73.65} & \textbf{93.41} & \textbf{97.16} & \textbf{99.12} & \textbf{99.75} & \textbf{-} &
\textbf{72.65} & \textbf{92.98} & \textbf{96.51} & \textbf{98.76} & \textbf{99.69} & \textbf{-} \\

\cellcolor{morandigreen!20}\textbf{LongCLIP} & +\textbf{Ours} &
\textit{76.25} & \textit{95.16} & \textit{97.94} & \textit{99.45} & \textit{99.84} & \textit{—} &
\textit{75.96} & \textit{94.92} & \textit{97.35} & \textit{99.24} & \textit{99.80} & \textit{—} \\
\cellcolor{morandigreen!20} & $\Delta$ &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} &
\textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} & \textit{—} \\

\cellcolor{morandipink!70} & Full-FT &
71.80 & 92.53 & 95.88 & 98.78 & 99.43 & 91.68 &
71.51 & 92.41 & 96.06 & 98.51 & 99.39 & 91.58 \\
\cellcolor{morandipink!70}\textbf{SigLIP-2} & +\textbf{Ours} &
\textbf{75.47} & \textbf{94.82} & \textbf{97.67} & \textbf{99.33} & \textbf{99.78} & \textbf{93.41} &
\textbf{73.59} & \textbf{94.33} & \textbf{97.43} & \textbf{99.37} & \textbf{99.84} & \textbf{92.91} \\
\cellcolor{morandipink!70} & $\Delta$ &
\dblue{+3.67} & \dblue{+2.29} & \dblue{+1.79} & \dblue{+0.55} & \dblue{+0.35} & \dblue{+1.73} &
\dblue{+2.08} & \dblue{+1.92} & \dblue{+1.37} & \dblue{+0.86} & \dblue{+0.45} & \dblue{+1.33} \\

\bottomrule
\end{tabular}
\end{table*}

% =========================
% Table 2: Adapters on CLIP (compact I→T / T→I cells)
% =========================
% =========================
% Table 2: Adapters on CLIP (compact I→T / T→I for all five datasets in one row)
% =========================
% \begin{table*}[t]
% \centering
% \caption{\textbf{Adapter study on CLIP (compact)}. All five datasets shown side-by-side. Cells show I$\rightarrow$T / T$\rightarrow$I.}
% \label{tab:adapters_compact}
% \renewcommand{\arraystretch}{1.1}
% \setlength{\tabcolsep}{2.6pt}
% \scriptsize
% \begin{tabular}{@{}lrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Trainable \%}} & \multirow{2}{*}{\textbf{Budget}}
% & \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{Sketchy}}
% & \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{Insect}}
% & \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{PathGen}}
% & \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{DCI}}
% & \multicolumn{3}{c}{\textbf{DOCCI}} \\
% \cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}\cmidrule(lr){16-18}
% & & & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
% & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
% & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
% & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
% & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 \\
% \midrule


% Full-FT (reference) & 100\% & 1.0$\times$
% & —/— & —/— & —/— 
% & —/— & —/— & —/— 
% & —/— & —/— & —/— 
% & —/— & —/— & —/— 
% & —/— & —/— & —/— \\
% LoRA                 & 0.65\% & 0.3$\times$
% & —/— & —/— & —/— 
% & 5.79/4.84 & 16.84/16.49 & 25.82/24.96 
% & 2.33/2.30 & 9.73/9.64 & 15.51/15.00 
% & 72.04/72.04 & 88.69/89.24 & 92.35/93.20 
% & —/— & —/— & —/— \\

% LoRA + \textbf{Ours} & 0.8\% & 0.35$\times$
% & —/— & —/— & —/— 
% & 5.87/5.32 & 18.31/18.65 & 27.63/28.41 
% & 2.65/2.63 & 9.92/9.73 & 16.35/15.41 
% & 73.89/72.30 & 89.44/89.49 & 92.50/93.45 
% & —/— & —/— & —/— \\
% DoRA                 & 0.8\% & 0.3$\times$
% & —/— & —/— & —/— 
% & 7.17/6.04 & 20.21/20.81 & 29.88/31.52 
% & 4.04/3.73 & 14.19/13.40 & 22.63/22.22 
% & —/— & —/— & —/— 
% & —/— & —/— & —/— \\

% DoRA + \textbf{Ours} & 0.8\% & 0.35$\times$
% & —/— & —/— & —/— 
% & 7.08/8.29 & 24.01/24.35 & 35.06/35.15 
% & 4.68/3.77 & 15.01/13.72 & 22.77/21.72 
% & —/— & —/— & —/— 
% & —/— & —/— & —/— \\
% \bottomrule
% \end{tabular}
% \vspace{-2mm}
% \end{table*}
\begin{table*}[t]
\centering
\caption{\textbf{Adapter study on CLIP (compact)}. All five datasets shown side-by-side. Cells show I$\rightarrow$T / T$\rightarrow$I.}
\label{tab:adapters_compact}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{2.6pt}
\scriptsize
\begin{tabular}{@{}lr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{\hspace{6pt}}rrr@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Trainable \%}}
& \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{Sketchy}}
& \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{Insect}}
& \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{PathGen}}
& \multicolumn{3}{c@{\hspace{6pt}}}{\textbf{DCI}}
& \multicolumn{3}{c}{\textbf{DOCCI}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
& & \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 \\
\midrule

Full-FT (reference) & 100\%
& —/— & —/— & —/—
& —/— & —/— & —/—
& —/— & —/— & —/—
& —/— & —/— & —/—
& —/— & —/— & —/— \\

LoRA & 0.65\%
& —/— & —/— & —/—
& 5.79/4.84 & 16.84/16.49 & 25.82/24.96
& 2.33/2.30 & 9.73/9.64 & 15.51/15.00
& 72.04/72.04 & 88.69/89.24 & 92.35/93.20
& 77.80/77.00 & 95.73/95.75 & 98.33/98.00 \\

LoRA + \textbf{Ours} & 0.8\%
& —/— & —/— & —/—
& 5.87/5.32 & 18.31/18.65 & 27.63/28.41
& 2.65/2.63 & 9.92/9.73 & 16.35/15.41
& 73.89/72.30 & 89.44/89.49 & 92.50/93.45
& 79.35/78.75 & 96.67/96.24 & 98.61/98.45 \\

DoRA & 0.8\%
& —/— & —/— & —/—
& 7.17/6.04 & 20.21/20.81 & 29.88/31.52
& 4.04/3.73 & 14.19/13.40 & 22.63/22.22
& 60.33/60.53 & 82.19/81.84 & 88.09/87.79
& 66.27/65.65 & 90.59/89.55 & 95.18/94.78 \\

DoRA + \textbf{Ours} & 0.8\%
& —/— & —/— & —/—
& 7.08/8.29 & 24.01/24.35 & 35.06/35.15
& 4.68/3.77 & 15.01/13.72 & 22.77/21.72
& 62.58/62.78 & 82.84/82.99 & 88.84/88.39
& 70.65/69.22 & 92.47/91.80 & 96.57/95.98 \\

\bottomrule
\end{tabular}
\vspace{-2mm}
\end{table*}

% =========================
% Table 3a: Loss ablation (two datasets, retrieval only; cells show I→T / T→I)
% =========================
\begin{table}[t]
\centering
\tiny
\setlength{\tabcolsep}{4.5pt}
\begin{tabular}{lccccc|ccccc}
\toprule
\multirow{2}{*}{Loss config} & \multicolumn{5}{c}{Text $\rightarrow$ Image (Recall@\%)} & \multicolumn{5}{c}{Image $\rightarrow$ Text (Recall@\%)} \\
\cmidrule(lr){2-6}\cmidrule(lr){7-11}
& R@1 & R@5 & R@10 & R@25 & R@50 & R@1 & R@5 & R@10 & R@25 & R@50 \\
\midrule
None(CLIP + Global finetuning)               & 8.38 & 25.73 & 35.06 & 51.30 & 64.51 & 8.72 & 26.60 & 36.36 & 51.30 & 63.64 \\
ST                 & 8.12 & \underline{26.51} & 37.31 & \underline{55.44} & 67.27 & 8.46 & \underline{26.86} & 37.74 & 54.32 & 67.70 \\
RS                 & 6.99 & 24.35 & 34.11 & 53.20 & 65.89 & 7.77 & 24.53 & 35.92 & 52.25 & 65.11 \\
Chunk              & 9.15 & 25.73 & 36.96 & 54.75 & 67.27 & \underline{8.81} & 26.25 & 37.65 & 54.23 & 67.36 \\
ST + RS            & 9.07 & \underline{26.51} & 37.22 & 53.71 & 68.57 & 7.94 & 26.68 & 37.48 & 53.97 & 67.44 \\
ST + Chunk         & 9.33 & 25.47 & 36.53 & \underline{55.44} & \underline{69.00} & 8.55 & \underline{26.86} & 38.34 & \textbf{55.27} & 67.53 \\
RS + Chunk         & 9.07 & 25.47 & \underline{38.17} & 54.75 & 68.83 & 8.03 & \textbf{27.81} & \underline{38.60} & 54.49 & \textbf{69.00} \\
ST + RS + Chunk    & \textbf{9.93} & \textbf{26.60} & \textbf{38.34} & \textbf{56.99} & \textbf{69.34} & \textbf{9.50} & 26.60 & \textbf{39.64} & \underline{54.92} & \underline{68.65} \\
ST + RS + Chunk (maybe better)    & \textbf{9.84} & \textbf{26.94} & \textbf{39.12} & \textbf{56.91} & \textbf{70.03} & \textbf{9.07} & 27.72 & \textbf{41.11} & \textbf{56.65} & \underline{68.31} \\

\bottomrule
\end{tabular}
\caption{Retrieval performance on the INSECT split (1{,}158 images / 1{,}158 texts). ST: scribble--text; RS: RGB--scribble consistency; Chunk: chunk--segment alignment. Best per column in \textbf{bold}, second best \underline{underlined}.}
\label{tab:loss_ablation}
\end{table}


\begin{table}[t]
\centering
\caption{\textbf{Ablation on loss terms} over two datasets (retrieval only). 
``Full'' includes $L_{\text{CLIP}}+L_{s\text{--}t}+L_{rs}+L_{\text{chunk}}$. 
Cells show I$\rightarrow$T / T$\rightarrow$I and are left as ``—/—'' for later fill-in.}
\label{tab:ablation_loss_two_ds}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.2pt}
\scriptsize
\begin{tabular}{@{}l|rrr|rrr@{}}
\toprule
\multirow{2}{*}{\textbf{Variant}} 
& \multicolumn{3}{c|}{\textbf{Sketchy (I$\rightarrow$T / T$\rightarrow$I)}} 
& \multicolumn{3}{c}{\textbf{PathGen (I$\rightarrow$T / T$\rightarrow$I)}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@5 & \footnotesize R@10 \\
\midrule
Full ($L_{\text{CLIP}}+L_{s\text{--}t}+L_{rs}+L_{\text{chunk}}$)
& —/— & —/— & —/— & —/— & —/— & —/— \\
$-$ $L_{s\text{--}t}$
& —/— & —/— & —/— & —/— & —/— & —/— \\
$-$ $L_{rs}$
& —/— & —/— & —/— & —/— & —/— & —/— \\
$-$ $L_{\text{chunk}}$
& —/— & —/— & —/— & —/— & —/— & —/— \\
Only $L_{\text{CLIP}}$
& —/— & —/— & —/— & —/— & —/— & —/— \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\end{table}

% =========================
% Table 4: GOAL interplay (negative on 3 datasets; ours rescues)
% =========================
\begin{table}[t]
\centering
\caption{\textbf{GOAL interplay across all five datasets}. We report R@1 and R@10 for both directions (I$\rightarrow$T / T$\rightarrow$I).}
\label{tab:goal_interplay_full}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\scriptsize

% ---------- Top block: structure-sensitive datasets ----------
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
\multicolumn{7}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{Structure-sensitive datasets}}} \\
\midrule
\multirow{2}{*}{\textbf{Method}} 
& \multicolumn{2}{c}{\textbf{Sketchy}} 
& \multicolumn{2}{c}{\textbf{Insect}} 
& \multicolumn{2}{c}{\textbf{PathGen}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& \footnotesize R@1 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@10 \\
\midrule
GOAL                 & —/— & —/— & —/— & —/— & —/— & —/— \\
GOAL + \textbf{Ours} & —/— & —/— & —/— & —/— & —/— & —/— \\
\bottomrule
\end{tabular}

\vspace{6pt}

% ---------- Bottom block: general-domain datasets ----------
\begin{tabular}{@{}lrrrr@{}}
\toprule
\multicolumn{5}{@{}l@{}}{\cellcolor{gray!10}\textsc{\textbf{General-domain datasets}}} \\
\midrule
\multirow{2}{*}{\textbf{Method}} 
& \multicolumn{2}{c}{\textbf{DCI}} 
& \multicolumn{2}{c}{\textbf{DOCCI}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& \footnotesize R@1 & \footnotesize R@10
& \footnotesize R@1 & \footnotesize R@10 \\
\midrule
GOAL                 & —/— & —/— & —/— & —/— \\
GOAL + \textbf{Ours} & —/— & —/— & —/— & —/— \\
\bottomrule
\end{tabular}

\vspace{-2mm}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{Attribute-binned improvements on \emph{Insect}} (retrieval only). 
Cells show I$\rightarrow$T / T$\rightarrow$I; entries are $\Delta$R@K (pp) vs.~baseline within each bin.
Bins are tertiles (\emph{Low/Mid/High}) over the whole test split.}
\label{tab:attr_bins_insect}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{2.6pt}
\scriptsize
\begin{tabular}{@{}l|rr rr rr|rr|rrr@{}}
\toprule
\multirow{2}{*}{\textbf{Attribute}} 
& \multicolumn{6}{c|}{\textbf{Bin-wise $\Delta$R@1 / $\Delta$R@10 (pp)}} 
& \multicolumn{2}{c|}{\textbf{High$-$Low (pp)}} 
& \multicolumn{3}{c}{\textbf{Bin size}} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-9}\cmidrule(lr){10-12}
& \multicolumn{2}{c}{Low} & \multicolumn{2}{c}{Mid} & \multicolumn{2}{c|}{High}
& \multicolumn{1}{c}{R@1} & \multicolumn{1}{c|}{R@10}
& $N_L$ & $N_M$ & $N_H$ \\
\midrule
Edge Density (\%)      & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
Edge Strength (grad)   & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
Edge Complexity (cnt)  & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
GLCM Contrast          & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
Colorfulness           & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
Text Length (tokens)   & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
Struct-word Ratio (\%) & —/— & —/— & —/— & —/— & —/— & —/— & —/— & —/— & — & — & — \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\end{table}

\begin{table}[t]
\centering
\caption{\textbf{Correlation and regression with improvements} on \emph{Insect}. 
$\rho$ is Spearman correlation between attribute and $\Delta$Rank (higher is better); 
$\beta$ is the standardized coefficient in a multivariate OLS: $\Delta$Rank $\sim$ (all listed attributes), reported per direction.
Stars denote significance (* $p{<}.05$, ** $p{<}.01$).}
\label{tab:corr_reg_insect}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\scriptsize
\begin{tabular}{@{}l|rrr|rrr@{}}
\toprule
\multirow{2}{*}{\textbf{Attribute}} 
& \multicolumn{3}{c|}{\textbf{I$\rightarrow$T}} 
& \multicolumn{3}{c}{\textbf{T$\rightarrow$I}} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
& $\rho$ & $p$ & $\beta$ 
& $\rho$ & $p$ & $\beta$ \\
\midrule
Edge Density (\%)      & — & — & — & — & — & — \\
Edge Strength (grad)   & — & — & — & — & — & — \\
Edge Complexity (cnt)  & — & — & — & — & — & — \\
GLCM Contrast          & — & — & — & — & — & — \\
Colorfulness           & — & — & — & — & — & — \\
Text Length (tokens)   & — & — & — & — & — & — \\
Struct-word Ratio (\%) & — & — & — & — & — & — \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\end{table}

% % =========================
% % Figure 5: Qualitative visualization (grid)
% % =========================
% \begin{figure*}[t]
% \centering
% % Replace the placeholders below with actual image paths later.
% \includegraphics[width=\textwidth]{figs/qual_grid_placeholder.pdf}
% \caption{\textbf{Qualitative results.} Columns: Input image, Scribble/Edge, Denoised attention map, Predicted mask, Ground-truth. 
% Examples from Sketchy/Insect/PathGen. Blue = jacket, Orange = shirt, Black = background.}
% \label{fig:qualitative}
% \vspace{-3mm}
% \end{figure*}

\subsection{Main results: full-parameter finetuning vs. +Ours}
Table~\ref{tab:fullft_main} summarizes cross-domain retrieval. 
Across all backbones, our edge-aware objectives consistently improve both directions (T$\rightarrow$I / I$\rightarrow$T), especially on structure-sensitive datasets (Sketchy/Insect/PathGen).
General-domain sets (DCI/DOCCI) also benefit without sacrificing global alignment.

\subsection{Adapter finetuning: LoRA/DoRA}
Table~\ref{tab:adapters} shows that adding our objectives on top of LoRA/DoRA yields further gains under similar budgets, narrowing the gap to full finetuning while retaining parameter efficiency.

\subsection{Ablation studies}
Loss ablations (Table~\ref{tab:ablation_loss}) validate the contribution of $L_{s\text{--}t}$ (scribble–text), $L_{rs}$ (RGB–scribble), and $L_{\text{chunk}}$ (chunk–patch) to both retrieval and segmentation transfer. 
Semantic stripping (Table~\ref{tab:ablation_strip}) stresses the model with reduced color/texture/material cues, highlighting robustness from structural alignment.

\subsection{Interplay with GOAL}
As shown in Table~\ref{tab:goal_interplay}, GOAL improves general-domain alignment but can degrade performance on structure-centric datasets; combining GOAL with our objectives mitigates this and brings further gains.

\subsection{Qualitative analysis}
Figure~\ref{fig:qualitative} illustrates typical cases: our masks better preserve object topology and boundaries, with denoised attention concentrating on edge-consistent regions.

% (Optional) add a short Reproducibility note or move std/CI to appendix.


==> sec/old/abstract13.11.2025.tex <==
\begin{abstract}
Edge-based representations provide a core substrate for visual understanding, enabling models to capture structural cues that extend beyond mere pixel statistics. This insight dates back to classic studies in early vision and remains central in contemporary research. In this paper, we customize this principle for visual-language alignment, showing that vision-language \ft can greatly benefit from isolating and aligning structural cues across modalities, even under limited data regimes and with long, descriptive captions. We introduce \ourmethod,
a \ft alignment paradigm that extracts edge maps (e.g., Canny, sketches), treating them as proxies for the visual structure of an image, and filters the corresponding captions to emphasize structural cues, making them ``structure-centric''.
Fine-tuning augments the standard alignment loss with three structure-centric objectives: (i) aligning edge maps with structural text, (ii) matching local edge regions to textual chunks, and (iii) connecting edge maps to color images to prevent representation drift.
From a theoretical standpoint, while standard CLIP maximizes the mutual information between visual and textual embeddings,
\ourmethod~additionally maximizes the mutual information between multimodal structural representations.
This auxiliary optimization is intrinsically harder, guiding the model toward more robust and semantically stable minima, enhancing vision-language alignment.  Beyond outperforming current competitors on cross-modal retrieval on both general and specialized domains, our method provides a general boosting principle that can be integrated into future approaches in a plug-and-play manner. Code and models will be released.
%Our structure-centric alignment losses are plug-and-play for a variety of CLIP-based finetuning strategies, consistently improving cross-modal retrieval performance on both general and specialized domains. Code and models will be released.
%, enhancing all evaluated CLIP-based strategies and achieving new state-of-the-art results on the Sketchy dataset.
\end{abstract}


\iffalse
\begin{abstract}
Vision-language fine-tuning can greatly benefit from isolating and aligning structural cues across modalities.
We demonstrate this by introducing \ourmethod,
%short for Struct-X-LIP, 
an auxiliary framework that can be integrated into any CLIP-based alignment method.
\ourmethod~extracts edge maps (e.g., Canny, sketches), treating them as proxies for the visual structure of an image, and filters the corresponding captions to emphasize structural cues.
Fine-tuning proceeds by supplementing the original alignment loss with three structure-centric losses, serving three objectives of:
(i) enforcing alignment between edge maps and structure-centric text,
(ii) establishing fine-grained correspondences between local edge regions and textual chunks, and
(iii) linking edge maps to the original color images to mitigate representation drift.
From a theoretical standpoint, while standard CLIP maximizes the mutual information between visual and textual embeddings,
\ourmethod~additionally maximizes the mutual information between multimodal structural representations.
This auxiliary optimization is intrinsically harder, guiding the model toward more robust and semantically stable minima, enhancing vision–language alignment.
Our structure-centric alignment losses are plug-and-play for a variety of CLIP-based finetuning strategies, consistently improving cross-modal retrieval performance on both general and specialized domains. Code and models will be released.
%, enhancing all evaluated CLIP-based strategies and achieving new state-of-the-art results on the Sketchy dataset.
\end{abstract}
\fi

%OLD ABSTRACTS
%Modern image understanding approaches rely on automated segmentation (e.g., SAM) to produce region-based structural decompositions that fuel downstream tasks such as captioning and retrieval. In this paper, we explore the complementary role of edge-based information, ranging from classical edge maps (e.g., Canny) to abstracted sketches. We show that injecting such edge-driven representations into vision–language pipelines unveils salient structures often overlooked by region-based analysis. This dichotomy between regions and edges, long established in image processing, emerges as a powerful principle for multimodal image understanding, enabling systematic improvements across retrieval, captioning, and segmentation benchmarks. 

==> sec/old/experiments.13.11.2025.tex <==

% =========================
% Experiments
% =========================
\section{Experiments}
\label{sec:exp}
We evaluate the complete framework \ourmethodfull, trained with all four losses of $\mathcal{L}_{\text{total}}$ of Sec.~\ref{Sec:alignment}, %Eq.~\ref{eq:total.loss},
referred to simply as \ourmethod unless stated otherwise, against state-of-the-art VLM fine-tuning methods on standard cross-modal retrieval benchmarks.
Our experiments span four datasets covering both general-purpose and domain-specific scenarios with rich natural-language descriptions.
We also demonstrate the plug-and-play nature of our structure-centric alignment losses \ourmethodaux (the terms $\lambda_{1}\structloss + \lambda_{2}\consistencyloss + \lambda_{3}\structlosslocal$ of the total loss $\mathcal{L}_{\text{total}}$ in Sec.~\ref{Sec:alignment})
%Eq.~\ref{eq:total.loss}) 
by integrating them into several existing fine-tuning frameworks.
Finally, we analyze several aspects of \ourmethod, including its generalization, sensitivity to training set size, and the effect of different edge detectors and loss components, and conclude with qualitative evidence and a theoretical explanation for its strong empirical performance. 

%ablate the impact in terms of the new structure-centric alignment losses, different types of the structure-centric images, and size of the training set.
%Finally, we showcase interesting qualitative results of \ourmethod in comparison with the best sota method, and provide explainable insights on its performance gain.

\noindent\textbf{Datasets.} For the general domain, we use the \textit{human-annotated} dataset DCI~\cite{urbanek2024picture} and DOCCI~\cite{docci2024} that are widely-adopted for dense image captioning. Specifically, DCI~\cite{urbanek2024picture} contains 7805 natural images, each of them is annotated with mask-aligned descriptions. The average length is above 1000 words. DOCCI~\cite{docci2024} contains 15k images that were taken by a single researcher traveling across the world with the intent of capturing diverse visual spatial scenes. Each image is annotated with long highly-compositional description. On average, each description contains 136 words, and is crafted to clearly distinguish each image from those that are related or similar.
Moreover, for the specific domains, we identify two publicly available datasets, containing rich textural descriptions. Specifically, Sketchy~\cite{girella2025lots} is a large scale multimodal fashion dataset of 46k outfit images where each garment in the image is associated with a detailed description. While the semantic classes of clothing items in Sketchy are common, the description contains diverse and detailed visual patterns, materials, shapes and spatial relations. The outfit description on average contains 31 words, with a maximum of 88 words. 
%\zanxi{sketchy is not actually a long text dataset...} 
Insect~\cite{truong2025insect} contains 6087 images of many fine-grained categories of insects in the biology domain. The semantic classes are fine-grained and rare, \ie, less represented in the pre-trained VLMs.
Each image is paired with a biologically detailed description, which has been expert-verified for accuracy and covers species-level morphology, coloration patterns, wing structures, and spatial configurations.
On average, each description contains 81 words. We further cleaned Insect~\cite{truong2025insect} for our experiment, as the original version contains duplicate samples and repeated descriptions. 

Regarding the \textbf{\textit{dataset split}}, we follow the split for DCI and DOCCI as in~\cite{goal2025}, where the DOCCI test set contains 5100 images and the DCI test set contains 2000 images. For Sketchy, we adopt the original test split~\cite{girella2025lots}, which contains 1.2k images. For Insect, as the original release does not provide the split, we thus divide the train/test set following 8:2 ratio, resulting in a test set of 1158 images. \yiming{how about training set for all of them?}\mc{I do not think it is needed... what is the purpose? Have been done similar experiments in other papers?}
Please refer to more details of datasets in \suppmat.

\noindent\textbf{Compared methods.}
We compare our method with a set of state-of-the-art CLIP finetuning methods that are proposed for long-text alignment:
i) \textit{LongCLIP}~\cite{zhang2024long} extends CLIP’s text encoder via positional interpolation to handle longer sequences while maintaining pre-trained alignment;
ii) \textit{FineLIP}~\cite{asokan2025finelip} enhances long-text understanding through multi-stage fine-tuning with adaptive attention fusion;
iii) \textit{SmartCLIP}~\cite{smartclip2025} introduces dynamic token routing and progressive context extension to selectively encode semantically salient textual segments;
iv) \textit{GOAL}~\cite{goal2025} jointly optimizes global and local image–text correspondences via Local Image-Sentence Matching (LISM) and Token Similarity-based Learning (TSL) for fine-grained alignment of detailed captions.

\noindent\textbf{Performance metrics.}
We report Recall@K (K=1/5/10) of the cross-modal retrieval task in both \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image} (\emph{T$\rightarrow$I})} and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text} (\emph{I$\rightarrow$T})} settings. 
Recall@K measures the proportion of queries for which the corresponding ground-truth match appears within the top-K retrieved results.
Each image is unique and is only paired to one textual description.

\noindent\textbf{Implementation details.}
Unless otherwise stated, we use ViT-B/16 backbones from the public checkpoint, with edges extracted by the Canny detector for all reported results. Inputs are resized to $224 x 224$. For fair comparison, all methods share the same text templates, tokenizer, batch size, and training budget. We empirically set %$\lambda_{1}=1.0$, 
$\lambda_{1}=0.25$, $\lambda_{2}=0.1$, and $\lambda_{3}=0.1$, since this setup ensured a good general performance. 
Results are averaged over 3 seeds; we report mean values (and optionally $\pm$std in the appendix) \mc{to you have all of these data?}. %To enable CLIP to handle longer textual sequences beyond its default 77-token limit, we follow Long-CLIP~\cite{zhang2024longclip}, SmartCLIP~\cite{smartclip2025}, and GOAL~\cite{goal2025}, and apply the Knowledge Preserving Stretching technique introduced in Long-CLIP~\cite{zhang2024longclip} for extending text positional embeddings.



%For segmentation transfer, we use train-free ClipTrASE decoding and report IoU, Dice, oIoU, and Boundary IoU (BIoU).




%%%%%TABLE 1 %%%%%%%

% \begin{table*}[t]
% \centering
% \caption{
% \textbf{Crossmodal retrieval performance of CLIP-based finetuning methods on multiple datasets}. We report Recall@K (\%) on both \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} settings.
% Each row represents one method evaluated on two datasets (left--right paired).
% Best results in \textbf{bold}; second best \underline{underlined}.
% $\Delta$ denotes the improvement margin over the second-best method. 
% }
% \label{tab:main_results_compact}
% \tighttable

% \footnotesize 

% \begin{tabular*}{\textwidth}{
%   @{}l 
%   @{\extracolsep{\fill}} 
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]
%   S[table-format=2.2]@{}
% }
% \toprule
% \multirow{3}{*}{\textbf{Method}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{SKETCHY}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{INSECT}} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}
% & \mcol{R@1} & \mcol{R@5} & \mcol{R@10} & \mcol{R@1} & \mcol{R@5} & \mcol{R@10}
% & \mcol{R@1} & \mcol{R@5} & \mcol{R@10} & \mcol{R@1} & \mcol{R@5} & \mcol{R@10} \\
% & \taskheader{Text$\rightarrow$Image} & \taskheader{Image$\rightarrow$Text}
% & \taskheader{Text$\rightarrow$Image} & \taskheader{Image$\rightarrow$Text} \\
% \midrule
% Long-CLIP{\tiny\textcolor{gray}{[ECCV'24]} }  & 54.32 & 80.14 & 88.43 & 52.76 & 80.31 & 88.08 & 8.20 & 23.83 & 34.97 & 9.41 & 24.78 & 37.31 \\
% FineLIP {\tiny\textcolor{gray}{[CVPR'25]} }  & 40.59 & 71.16 & 81.78 & 40.33 & 72.11 & 82.38 & 8.46 & 23.32 & 33.59 & 6.86 & 23.75 & 34.46 \\
% SmartCLIP{\tiny\textcolor{gray}{[CVPR'25]} }  & 50.73 & 81.09 & \underline{94.56} & 51.30 & 80.83 & \underline{94.04} & 4.84 & 16.84 & 34.63 & 4.66 & 15.46 & 34.02 \\
% GOAL{\tiny\textcolor{gray}{[CVPR'25]} }      & \underline{63.21} & \underline{87.13} & 93.44 & \underline{62.44} & \underline{87.82} & 92.31 & \underline{8.81} & \underline{24.35} & \underline{35.84} & \underline{8.55} & \underline{25.91} & 36.18 \\
% \textbf{Ours} & \textbf{69.86} & \textbf{90.85} & \textbf{95.42} & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} & \textbf{9.93} & \textbf{26.60} & \textbf{38.34} & \textbf{9.50} & \textbf{26.60} & \textbf{39.64} \\
% \cmidrule(lr){1-13}

% \textit{$\Delta$} & \gain{6.65} & \gain{3.72} & \gain{0.86} & \gain{5.78} & \gain{2.85} & \gain{1.64} & \gain{1.12} & \gain{2.25} & \gain{2.50} & \gain{0.09} & \gain{0.69} & \gain{2.33} \\
% \midrule[0.8pt]
% \multirow{3}{*}{\textbf{Method}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{DOCCI}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{DCI}} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}
% & \mcol{R@1} & \mcol{R@5} & \mcol{R@10} & \mcol{R@1} & \mcol{R@5} & \mcol{R@10}
% & \mcol{R@1} & \mcol{R@5} & \mcol{R@10} & \mcol{R@1} & \mcol{R@5} & \mcol{R@10} \\
% & \taskheader{Text$\rightarrow$Image} & \taskheader{Image$\rightarrow$Text}
% & \taskheader{Text$\rightarrow$Image} & \taskheader{Image$\rightarrow$Text} \\
% \midrule
% Long-CLIP{\tiny\textcolor{gray}{[ECCV'24]} }  & 64.49 & 87.67 & 93.43 & 63.08 & 87.45 & 93.14 & 59.23 & 80.89 & 87.04 & 60.13 & 81.44 & 87.54 \\
% FineLIP {\tiny\textcolor{gray}{[CVPR'25]} }   & 67.80 & 90.22 & 94.84 & 66.39 & 89.12 & 94.47 & 66.13 & 85.34 & 89.79 & 64.58 & 84.59 & 89.54 \\
% SmartCLIP{\tiny\textcolor{gray}{[CVPR'25]} }  & 74.92 & 94.08 & \textbf{98.96} & 74.91 & 94.04 & \textbf{98.98} & 69.88 & 86.64 & \underline{94.05} & 70.94 & 87.04 & \textbf{94.60} \\
% GOAL{\tiny\textcolor{gray}{[CVPR'24]} }      & \underline{79.47} & \underline{96.65} & {---} & \underline{79.43} & \underline{96.14} & {---} & \underline{72.64} & \underline{89.89} & {---} & \underline{72.84} & \textbf{90.50} & {---} \\
% \textbf{Ours} & \textbf{83.04} & \textbf{97.06} & \textbf{98.96} & \textbf{81.59} & \textbf{96.94} & \underline{98.78} & \textbf{75.90} & \textbf{90.00} & \textbf{95.15} & \textbf{74.39} & \underline{89.90} & \underline{94.30} \\
% \cmidrule(lr){1-13}


% \textit{$\Delta$} & \gain{3.57} & \gain{0.41} & \neutral{0.00} & \gain{2.16} & \gain{0.80} & \loss{0.20} & \gain{3.26} & \gain{0.11} & \gain{1.10} & \gain{1.55} & \loss{0.60} & \loss{0.30} \\
% \bottomrule
% \end{tabular*}
% \vspace{0.5em}

% \end{table*}
\input{tables/table1}

% \begin{table*}[t]
% \centering
% \caption{
% \textbf{Crossmodal retrieval performance of CLIP-based finetuning methods on multiple datasets}. We report Recall@K (\%) on both \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} settings.
% Each row represents one method evaluated on two datasets (left--right paired).
% Best results in \textbf{bold}; second best \underline{underlined}.
% $\Delta$ denotes the improvement margin over the second-best method.
% }
% \label{tab:main_results_compact}
% \tighttable

% \footnotesize

% \begin{tabular*}{\textwidth}{
% @{}l
% @{\extracolsep{\fill}}
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]
% S[table-format=2.2]@{}
% }
% \toprule

% \multirow{2}{*}{\textbf{Method}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{SKETCHY}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{INSECT}} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}

% & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\

% \midrule
% Long-CLIP{\tiny\textcolor{gray}{[ECCV'24]} } & 54.32 & 80.14 & 88.43 & 52.76 & 80.31 & 88.08 & 8.20 & 23.83 & 34.97 & 9.41 & 24.78 & 37.31 \\
% FineLIP {\tiny\textcolor{gray}{[CVPR'25]} } & 40.59 & 71.16 & 81.78 & 40.33 & 72.11 & 82.38 & 8.46 & 23.32 & 33.59 & 6.86 & 23.75 & 34.46 \\
% SmartCLIP{\tiny\textcolor{gray}{[CVPR'25]} }  & 50.73 & 81.09 & \underline{94.56} & 51.30 & 80.83 & \underline{94.04} & 4.84 & 16.84 & 34.63 & 4.66 & 15.46 & 34.02 \\
% GOAL{\tiny\textcolor{gray}{[CVPR'25]} }  & \underline{63.21} & \underline{87.13} & 93.44 & \underline{62.44} & \underline{87.82} & 92.31 & \underline{8.81} & \underline{24.35} & \underline{35.84} & \underline{8.55} & \underline{25.91} & 36.18 \\
% \textbf{\ourmethod~} & \textbf{69.86} & \textbf{90.85} & \textbf{95.42} & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} & \textbf{9.93} & \textbf{26.60} & \textbf{38.34} & \textbf{9.50} & \textbf{26.60} & \textbf{39.64} \\
% \cmidrule(lr){1-13}

% \textit{$\Delta$} & \gain{6.65} & \gain{3.72} & \gain{0.86} & \gain{5.78} & \gain{2.85} & \gain{1.64} & \gain{1.12} & \gain{2.25} & \gain{2.50} & \gain{0.09} & \gain{0.69} & \gain{2.33} \\
% \midrule[0.8pt]

% \multirow{2}{*}{\textbf{Method}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{DOCCI}} &
% \multicolumn{6}{c}{\cellcolor{panelgray}\textbf{DCI}} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}

% & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\

% \midrule
% Long-CLIP{\tiny\textcolor{gray}{[ECCV'24]} } & 64.49 & 87.67 & 93.43 & 63.08 & 87.45 & 93.14 & 59.23 & 80.89 & 87.04 & 60.13 & 81.44 & 87.54 \\
% FineLIP {\tiny\textcolor{gray}{[CVPR'25]} }& 67.80 & 90.22 & 94.84 & 66.39 & 89.12 & 94.47 & 66.13 & 85.34 & 89.79 & 64.58 & 84.59 & 89.54 \\
% SmartCLIP{\tiny\textcolor{gray}{[CVPR'25]} }  & 74.92 & 94.08 & \textbf{98.96} & 74.91 & 94.04 & \textbf{98.98} & 69.88 & 86.64 & \underline{94.05} & 70.94 & 87.04 & \textbf{94.60} \\
% GOAL{\tiny\textcolor{gray}{[CVPR'24]} }      & \underline{79.47} & \underline{96.65} & {98.69} & \underline{79.43} & \underline{96.14} & {97.25} & \underline{72.64} & \underline{89.89} & {93.7} & \underline{72.84} & \textbf{90.50} & {93.2} \\
% \textbf{\ourmethod~} & \textbf{83.04} & \textbf{97.06} & \textbf{98.96} & \textbf{81.59} & \textbf{96.94} & \underline{98.78} & \textbf{75.90} & \textbf{90.00} & \textbf{95.15} & \textbf{74.39} & \underline{89.90} & \underline{94.30} \\
% \cmidrule(lr){1-13}


% \textit{$\Delta$} & \gain{3.57} & \gain{0.41} & \neutral{0.00} & \gain{2.16} & \gain{0.80} & \loss{0.20} & \gain{3.26} & \gain{0.11} & \gain{1.10} & \gain{1.55} & \loss{0.60} & \loss{0.30} \\
% \bottomrule
% \end{tabular*}
% \vspace{0.5em}

% \end{table*}


% =========================
% Table 2: Adapters on CLIP (compact I→T / 
% =========================

% \begin{table*}[t]
% \centering
% \footnotesize

% \caption{
% \textbf{Plug-and-play enhancement of CLIP-based finetuning.}
% Results on SKETCHY, INSECT, DOCCI, and DCI for \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval.
% Upper: full-parameter finetuning; lower: parameter-efficient tuning.
% Our method consistently boosts diverse CLIP variants.
% }
% \label{tab:main_results_compact}


% \begin{table*}[t]
% \caption{
% \textbf{Plug-and-play enhancement of CLIP-based finetuning.}
% Results on SKETCHY and DOCCI for \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval.
% Upper: full-parameter finetuning; lower: parameter-efficient tuning.
% Our method consistently boosts diverse CLIP variants.
% }
% \label{tab:main_results_compact}
% \centering
% \scriptsize
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc|cccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} &
% \multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{SKETCHY}} &
% \multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}
% & \cellcolor{lightpink}R@1
% & \cellcolor{lightpink}R@5
% & \cellcolor{lightpink}R@10
% & \cellcolor{lightblue}R@1
% & \cellcolor{lightblue}R@5
% & \cellcolor{lightblue}R@10
% & \cellcolor{lightpink}R@1
% & \cellcolor{lightpink}R@5
% & \cellcolor{lightpink}R@10
% & \cellcolor{lightblue}R@1
% & \cellcolor{lightblue}R@5
% & \cellcolor{lightblue}R@10 \\
% \midrule

% Long-CLIP
% & 54.32 & 80.14 & 88.43 & 52.76 & 80.31 & 88.08
% & 64.49 & 87.67 & 93.43 & 63.08 & 87.45 & 93.14 \\
% \textbf{+Ours}
% & \textbf{59.24} {\color{lightgreen}{\tiny$\uparrow$4.92}}
% & \textbf{85.32} {\color{lightgreen}{\tiny$\uparrow$5.18}}
% & \textbf{91.45} {\color{lightgreen}{\tiny$\uparrow$3.02}}
% & \textbf{59.59} {\color{lightgreen}{\tiny$\uparrow$6.83}}
% & \textbf{84.37} {\color{lightgreen}{\tiny$\uparrow$4.06}}
% & \textbf{91.02} {\color{lightgreen}{\tiny$\uparrow$2.94}}
% & \textbf{67.67} {\color{lightgreen}{\tiny$\uparrow$3.18}}
% & \textbf{90.82} {\color{lightgreen}{\tiny$\uparrow$3.15}}
% & \textbf{95.59} {\color{lightgreen}{\tiny$\uparrow$2.16}}
% & \textbf{67.92} {\color{lightgreen}{\tiny$\uparrow$4.84}}
% & \textbf{90.16} {\color{lightgreen}{\tiny$\uparrow$2.71}}
% & \textbf{95.10} {\color{lightgreen}{\tiny$\uparrow$1.96}} \\
% \lightmidrule

% FineLIP
% & 40.59 & 71.16 & 81.78 & 40.33 & 72.11 & 82.38
% & 67.80 & 90.22 & 94.84 & 66.39 & 89.12 & 94.47 \\
% \textbf{+Ours}
% & \textbf{59.15} {\color{lightgreen}{\tiny$\uparrow$18.56}}
% & \textbf{85.23} {\color{lightgreen}{\tiny$\uparrow$14.07}}
% & \textbf{91.28} {\color{lightgreen}{\tiny$\uparrow$9.50}}
% & \textbf{58.55} {\color{lightgreen}{\tiny$\uparrow$18.22}}
% & \textbf{84.54} {\color{lightgreen}{\tiny$\uparrow$12.43}}
% & \textbf{90.07} {\color{lightgreen}{\tiny$\uparrow$7.69}}
% & \textbf{74.06} {\color{lightgreen}{\tiny$\uparrow$6.26}}
% & \textbf{94.24} {\color{lightgreen}{\tiny$\uparrow$4.02}}
% & \textbf{97.35} {\color{lightgreen}{\tiny$\uparrow$2.51}}
% & \textbf{72.94} {\color{lightgreen}{\tiny$\uparrow$6.55}}
% & \textbf{93.27} {\color{lightgreen}{\tiny$\uparrow$4.15}}
% & \textbf{96.55} {\color{lightgreen}{\tiny$\uparrow$2.08}} \\
% \lightmidrule

% SmartCLIP
% & 50.73 & 81.09 & 94.56 & 51.30 & 80.83 & 94.04
% & 74.92 & 94.08 & 98.96 & 74.91 & 94.04 & 98.98 \\
% \textbf{+Ours}
% & \textbf{52.94} {\color{lightgreen}{\tiny$\uparrow$2.21}}
% & \textbf{81.26} {\color{lightgreen}{\tiny$\uparrow$0.17}}
% & \textbf{94.77} {\color{lightgreen}{\tiny$\uparrow$0.21}}
% & \textbf{52.33} {\color{lightgreen}{\tiny$\uparrow$1.03}}
% & \textbf{80.92} {\color{lightgreen}{\tiny$\uparrow$0.09}}
% & \textbf{94.04} {\color{lightgreen}{\tiny-0.00}}
% & \textbf{76.00} {\color{lightgreen}{\tiny$\uparrow$1.08}}
% & \textbf{95.28} {\color{lightgreen}{\tiny$\uparrow$1.20}}
% & \textbf{99.24} {\color{lightgreen}{\tiny$\uparrow$0.28}}
% & \textbf{75.25} {\color{lightgreen}{\tiny$\uparrow$0.34}}
% & \textbf{94.27} {\color{lightgreen}{\tiny$\uparrow$0.23}}
% & \textbf{98.90} {\color{red}{\tiny$\downarrow$0.08}} \\
% \lightmidrule

% GOAL
% & 63.21 & 87.13 & 93.44 & 62.44 & 87.82 & 92.31
% & 79.47 & 96.65 & 98.69 & 79.43 & 96.14 & 98.51 \\
% \textbf{+Ours}
% & \textbf{67.88} {\color{lightgreen}{\tiny$\uparrow$4.67}}
% & \textbf{90.33} {\color{lightgreen}{\tiny$\uparrow$3.20}}
% & \textbf{95.16} {\color{lightgreen}{\tiny$\uparrow$1.72}}
% & \textbf{68.48} {\color{lightgreen}{\tiny$\uparrow$6.04}}
% & \textbf{89.81} {\color{lightgreen}{\tiny$\uparrow$1.99}}
% & \textbf{94.82} {\color{lightgreen}{\tiny$\uparrow$2.51}}
% & \textbf{80.96} {\color{lightgreen}{\tiny$\uparrow$1.49}}
% & \textbf{96.90} {\color{lightgreen}{\tiny$\uparrow$0.27}}
% & \textbf{98.96} {\color{lightgreen}{\tiny$\uparrow$0.25}}
% & \textbf{80.31} {\color{lightgreen}{\tiny$\uparrow$0.88}}
% & \textbf{96.73} {\color{lightgreen}{\tiny$\uparrow$0.59}}
% & \textbf{98.84} {\color{lightgreen}{\tiny$\uparrow$0.33}}\\

% \doublemidrule

% LoRA
% & 57.08 & 84.72 & 91.80 & 56.74 & 85.32 & 91.71
% & 77.80 & 96.45 & 98.55 & 77.00 & 96.02 & 98.05 \\
% \textbf{+Ours}
% & \textbf{62.09} {\color{lightgreen}{\tiny$\uparrow$5.01}}
% & \textbf{86.79} {\color{lightgreen}{\tiny$\uparrow$2.07}}
% & \textbf{93.95} {\color{lightgreen}{\tiny$\uparrow$2.15}}
% & \textbf{59.41} {\color{lightgreen}{\tiny$\uparrow$2.67}}
% & \textbf{85.92} {\color{lightgreen}{\tiny$\uparrow$0.60}}
% & \textbf{92.75} {\color{lightgreen}{\tiny$\uparrow$1.04}}
% & \textbf{79.35} {\color{lightgreen}{\tiny$\uparrow$1.55}}
% & \textbf{96.61} {\color{lightgreen}{\tiny$\uparrow$0.16}}
% & \textbf{98.57} {\color{lightgreen}{\tiny$\uparrow$0.02}}
% & \textbf{78.65} {\color{lightgreen}{\tiny$\uparrow$1.65}}
% & \textbf{96.31} {\color{lightgreen}{\tiny$\uparrow$0.29}}
% & \textbf{98.45} {\color{lightgreen}{\tiny$\uparrow$0.40}} \\
% \lightmidrule

% DoRA
% & 61.77 & 86.18 & 91.88 & 60.94 & 87.33 & 92.31
% & 66.27 & 90.50 & 95.18 & 65.65 & 89.55 & 94.78 \\
% \textbf{+Ours}
% & \textbf{65.20} {\color{lightgreen}{\tiny$\uparrow$3.43}}
% & \textbf{90.26} {\color{lightgreen}{\tiny$\uparrow$4.08}}
% & \textbf{94.91} {\color{lightgreen}{\tiny$\uparrow$3.03}}
% & \textbf{64.94} {\color{lightgreen}{\tiny$\uparrow$4.00}}
% & \textbf{88.35} {\color{lightgreen}{\tiny$\uparrow$1.02}}
% & \textbf{93.52} {\color{lightgreen}{\tiny$\uparrow$1.21}}
% & \textbf{70.65} {\color{lightgreen}{\tiny$\uparrow$4.38}}
% & \textbf{92.47} {\color{lightgreen}{\tiny$\uparrow$1.97}}
% & \textbf{96.57} {\color{lightgreen}{\tiny$\uparrow$1.39}}
% & \textbf{69.22} {\color{lightgreen}{\tiny$\uparrow$3.57}}
% & \textbf{91.80} {\color{lightgreen}{\tiny$\uparrow$2.25}}
% & \textbf{95.98} {\color{lightgreen}{\tiny$\uparrow$1.20}} \\


% \bottomrule
% \end{tabular*}
% \end{table*}


% =========================
% Table 3a: Loss ablation (two datasets, retrieval only; cells show I→T / T→I)
% =========================



% =========================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Table 5 Ablation on types of structure-centric image.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table}[t]
% \centering
% \caption{
% \textbf{Ablation on types of structure-centric image.}
% Comparison of different edge extraction formats 
% for \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} 
% and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval
% on SKETCHY and DOCCI.
% }
% \label{tab:edge_format_ablation}
% \scriptsize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}

% \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lccc|ccc@{}}
% \toprule
% \textbf{Edge Format} &
% \cellcolor{lightpink}\textbf{R@1} &
% \cellcolor{lightpink}\textbf{R@5} &
% \cellcolor{lightpink}\textbf{R@10} &
% \cellcolor{lightblue}\textbf{R@1} &
% \cellcolor{lightblue}\textbf{R@5} &
% \cellcolor{lightblue}\textbf{R@10} \\
% \midrule

% \multicolumn{7}{c}{\cellcolor{gray!10}\textbf{SKETCHY Dataset}} \\
% \midrule
% Canny & \textbf{69.86} & \textbf{90.85} & \textbf{95.42} & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} \\
% LoG & 68.48 & 89.64 & 94.91 & 67.36 & 90.24 & 94.47 \\
% HEG & 68.91 & 90.67 & 95.43 & 66.93 & 90.41 & 94.47 \\
% LineArtDetector & 69.17 & 90.93 & 95.42 & 66.93 & 90.16 & 94.91 \\
% Photo2sketch & 68.14 & 90.76 & 94.99 & 67.53 & 90.16 & 94.04 \\
% Incorrect match & 66.20 & 88.95 & 93.39 & 64.37 & 88.26 & 93.78 \\
% \lightmidrule
% \multicolumn{7}{c}{\cellcolor{gray!10}\textbf{DOCCI Dataset}} \\
% \midrule
% Canny & 83.04 & 97.06 & 98.96 & 81.59 & 96.94 & 98.78 \\
% LoG & \textbf{83.59} & \textbf{97.36} & \textbf{99.20} & \textbf{81.98} & \textbf{97.41} & \textbf{99.04} \\
% HEG & 83.14 & 97.18 & 98.98 & 81.73 & 97.08 & 98.69 \\
% LineArtDetector & 82.69 & 97.10 & 98.90 & 81.08 & 96.84 & 98.84 \\
% Photo2sketch  & 81.49 & 97.02 & 98.73 & 80.20 & 96.43 & 98.47 \\
% % RANDOM line & 80.82 & 96.19 & 98.75 & 79.08 & 96.10 & 98.41 \\
% Incorrect match & 80.25 & 96.33 & 98.76 & 79.15 & 96.10 & 98.41 \\
% \bottomrule
% \end{tabular*}
% \end{table}


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/percentage2.pdf}
    \caption{Training data amount VS performance: Retrieval recall R\@1 in case of 5\%, 20\%, 50\% of training data, compared to the standard 100\%. The improvement indicates the margin of \ourmethod against the second best approach, trained with the same amount of data.}
    \label{fig:data.amount}
    \vspace{-8pt}
\end{figure}




\subsection{Main comparisons}\label{Sec:main.comparisons}
\noindent\textbf{Best-performing on cross-modal retrieval.} As shown in Tab.~\ref{tab:main_results}, our \ourmethod~consistently achieves the best R@1 on both directions (T$\rightarrow$I / I$\rightarrow$T) among all compared methods \mc{We should say that in general the other recall rankings are in the addmat - if they are. Maybe here we can say some sentence about what happens in general in the other ranks}. On the Sketchy dataset, the improvement obtained by \ourmethod~is most significant: R@1 on the increases by +6.65\% and +5.78\% compared to the second-best method GOAL, on the T$\rightarrow$I and I$\rightarrow$T task, respectively. Despite being with the shortest word length, Sketchy dataset contains rich structure-centric multimodal content concerning clothing items (\eg, shape, layering, designs, contour, and outfit compositions), making our structure-centric multimodal alignment most effective to enhance the representation alignment on fine-grained details. 
%By explicitly isolating and aligning such structure-centric multimodal contents, \ourmethod~can effectively  the interference from appearance-related attributes, enabling the model to match hierarchical semantic structures and thus achieve higher retrieval precision, especially at top ranks. 
On the other hand, the performance of all models on the Insect dataset is relatively low as the dataset belongs to a rare domain knowledge, \ie specific families of insects, that is underrepresented in the pre-training dataset for VLMs.
Nevertheless, \ourmethod~still improves R@1 in the T$\rightarrow$I direction by +1.12\% (a relative gain of 12.7\%) with stable improvements for I$\rightarrow$T.
%This improvement mainly comes from the geometric constraints introduced by 
We believe this is attributed to the edge maps that provide a degree of morphological invariance across species highlighting subtle visual differences during the text-visual alignment.
Finally, \ourmethod~also shows consistent gains over compared methods on the general-domain datasets DOCCI and DCI, demonstrating its broad effectiveness.
%structural alignment not only benefits domain-specific understanding but also serves as a regularizing constraint in natural image domains, helping the model learn a more stable multimodal representation.


\begin{table}[t]
\caption{
\textbf{Plug-and-play enhancement of CLIP-based finetuning.}
Results on SKETCHY and DOCCI for \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval.
Upper: full-parameter finetuning; lower: parameter-efficient tuning.
Our method consistently boosts diverse CLIP variants.
}
\label{tab:finetuning_agnostic}
\centering
\footnotesize
\resizebox{\columnwidth}{!}{%
% {\fontsize{20}{24}\selectfont
% {\fontsize{14}{16}\selectfont
{\fontsize{24}{28}\selectfont
\begin{tabular}{@{} l*{5}{S[table-format=2.2] !{\color{lightlightgray}\vrule width 0.5pt}} S[table-format=2.2] | *{5}{S[table-format=2.2] !{\color{lightlightgray}\vrule width 0.5pt} } S[table-format=2.2] @{}}
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{SKETCHY}} &
\multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c|}{\cellcolor{lightblue}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\
\midrule

Long-CLIP
& 54.32 & 80.14 & 88.43 & 52.76 & 80.31 & 88.08
& 64.49 & 87.67 & 93.43 & 63.08 & 87.45 & 93.14 \\
\textbf{+Ours}
& \textbf{59.24} 
& \textbf{85.32} 
& \textbf{91.45} 
& \textbf{59.59} 
& \textbf{84.37} 
& \textbf{91.02} 
& \textbf{67.67} 
& \textbf{90.82} 
& \textbf{95.59} 
& \textbf{67.92} 
& \textbf{90.16} 
& \textbf{95.10}  \\

\textit{$\Delta$}
& \gain{4.92} & \gain{5.18} & \gain{3.02} 
& \gain{6.83} & \gain{4.06} & \gain{2.94}
& \gain{3.18} & \gain{3.15} & \gain{2.16} 
& \gain{4.84} & \gain{2.71} & \gain{1.96}
\\
\lightmidrule

FineLIP
& 40.59 & 71.16 & 81.78 & 40.33 & 72.11 & 82.38
& 67.80 & 90.22 & 94.84 & 66.39 & 89.12 & 94.47 \\
\textbf{+Ours}
& \textbf{59.15} 
& \textbf{85.23} 
& \textbf{91.28} 
& \textbf{58.55} 
& \textbf{84.54} 
& \textbf{90.07} 
& \textbf{74.06}
& \textbf{94.24} 
& \textbf{97.35} 
& \textbf{72.94} 
& \textbf{93.27}
& \textbf{96.55} \\

\textit{$\Delta$}
& \gain{18.56} & \gain{14.07} & \gain{9.50} 
& \gain{18.22} & \gain{12.43} & \gain{7.69}
& \gain{6.26} & \gain{4.02} & \gain{2.51} 
& \gain{6.55} & \gain{4.14} & \gain{2.08}
\\
\lightmidrule

SmartCLIP
& 50.73 & 81.09 & 94.56 & 51.30 & 80.83 & \textbf{94.04}
    & 74.92 & 94.08 & 97.31 & 74.91 & 94.04 & 97.29 \\
\textbf{+Ours}
& \textbf{52.94}
& \textbf{81.26} 
& \textbf{94.77} 
& \textbf{52.33} 
& \textbf{80.92} 
& \textbf{94.04} 
& \textbf{77.39} 
& \textbf{95.57} 
& \textbf{98.66} 
& \textbf{77.10} 
& \textbf{95.49} 
& \textbf{98.34}  \\

\textit{$\Delta$}
& \gain{2.21} & \gain{0.17} & \gain{0.21} 
& \gain{1.03} & \gain{0.09} & \neutral{0.00}
& \gain{2.47} & \gain{1.49} & \gain{1.35} 
& \gain{2.19} & \gain{1.45} & \gain{1.05}
\\
\lightmidrule

GOAL
& 63.21 & 87.13 & 93.44 & 62.44 & 87.82 & 92.31
& 79.47 & 96.65 & 98.69 & 79.43 & 96.14 & 98.51 \\
\textbf{+Ours}
& \textbf{67.88}
& \textbf{90.33} 
& \textbf{95.16} 
& \textbf{68.48} 
& \textbf{89.81} 
& \textbf{94.82} 
& \textbf{80.96} 
& \textbf{96.90} 
& \textbf{98.96} 
& \textbf{80.31}
& \textbf{96.73} 
& \textbf{98.84} \\

\textit{$\Delta$}
& \gain{4.67} & \gain{3.20} & \gain{1.72} 
& \gain{6.04} & \gain{1.99} & \gain{2.51}
& \gain{1.49} & \gain{0.27} & \gain{0.25} 
& \gain{0.88} & \gain{0.59} & \gain{0.33}
\\
\lightmidrule
SigLIP2
& 68.91 & 90.85 & 95.16 & 66.75 & 90.24 & 93.96
& 71.80 & 92.53 & 95.88 & 71.51 & 92.41 & 96.06 \\
\textbf{+Ours}
& \textbf{73.49}
& \textbf{91.97} 
& \textbf{95.77} 
& \textbf{70.38} 
& \textbf{91.54} 
& \textbf{95.77} 
& \textbf{75.47} 
& \textbf{94.82} 
& \textbf{97.67} 
& \textbf{73.59}
& \textbf{94.33} 
& \textbf{97.43} \\

\textit{$\Delta$}
& \gain{4.58} & \gain{1.12} & \gain{0.61} 
& \gain{3.63} & \gain{1.3} & \gain{1.81}
& \gain{3.67} & \gain{2.29} & \gain{1.79} 
& \gain{2.08} & \gain{1.92} & \gain{1.37}
\\

\midrule[2pt]
LoRA
& 57.08 & 84.72 & 91.80 & 56.74 & 85.32 & 91.71
& 77.80 & 96.45 & 98.55 & 77.00 & 96.02 & 98.05 \\
\textbf{+Ours}
& \textbf{62.09}
& \textbf{86.79} 
& \textbf{93.95} 
& \textbf{59.41} 
& \textbf{85.92} 
& \textbf{92.75} 
& \textbf{79.35} 
& \textbf{96.61} 
& \textbf{98.57} 
& \textbf{78.65} 
& \textbf{96.31} 
& \textbf{98.45} \\

\textit{$\Delta$}
& \gain{5.01} & \gain{2.07} & \gain{2.15} 
& \gain{2.67} & \gain{0.60} & \gain{1.04}
& \gain{1.55} & \gain{0.16} & \gain{0.02} 
& \gain{1.65} & \gain{0.29} & \gain{0.40}
\\
\lightmidrule

DoRA
& 61.77 & 86.18 & 91.88 & 60.94 & 87.33 & 92.31
& 66.27 & 90.50 & 95.18 & 65.65 & 89.55 & 94.78 \\
\textbf{+Ours}
& \textbf{65.20}
& \textbf{90.26} 
& \textbf{94.91} 
& \textbf{64.94} 
& \textbf{88.35} 
& \textbf{93.52} 
& \textbf{70.65}
& \textbf{92.47} 
& \textbf{96.57} 
& \textbf{69.22} 
& \textbf{91.80}
& \textbf{95.98}  \\

\textit{$\Delta$}
& \gain{3.43} & \gain{4.08} & \gain{3.03}
& \gain{4.00} & \gain{1.02} & \gain{1.21}
& \gain{4.38} & \gain{1.97} & \gain{1.39} 
& \gain{3.57} & \gain{2.25} & \gain{1.20}
\\
\bottomrule
\end{tabular}
}
}
\end{table}

\noindent\textbf{Finetuning-agnostic improvement.} 
Our introduced losses \ourmethodaux are additional auxiliary losses, which can be flexibly integrated on top of any CLIP-based finetuning methods and techniques. To investigate its effectiveness, we experiment with both classic parameter-efficient finetuning (PEFT) techniques including LoRA~\cite{hu2022lora} and DoRA~\cite{liu2024dora}, and the state-of-the-art CLIP-based finetuning methods presented the main comparison.
As shown in Tab.~\ref{tab:finetuning_agnostic}\footnote{Results on the other datasets will be shown in the \suppmat.}, \ourmethodaux is plug-and-play on any CLIP-based finetuning techniques, consistently demonstrating \textbf{X}LIP-agnostic improvements on both general and specific domains. The benefits also extend to the adapter-based PEFT techniques, when finetuning models with few additional learnable parameters. 
%In the full-parameter finetuning setting, it achieves the most notable gain on the fashion-oriented Sketchy dataset, boosting R@1 (T$\rightarrow$I) by +18.6\% when combined with FineLIP. 
In PEFT, \ourmethodaux~with LoRA and DoRA achieves about +4-5\% R@1 improvement, showing that it can serve as a lightweight and plug-and-play enhancement module to improve multimodal alignment with negligible additional computational cost. 
\zanxi{How can we explain why lora/dora performs better than finelip, smartclip, and longclip, which are all methods with full parameter fine-tuning?} 
\yiming{maybe we don't need to explain, can we cite some few-shot learning papers where LoRA is often compared to full parameter-finetuning? if they report the same behavior, we can say our results are inline with literature.}\mc{I want say anything, this is a question we would like the reviewers to ask us. Maybe I can add some other numbers}\mc{It is very important we say we will share the code.} Notably, on Sketchy we get an average improvement of 6.20\% (relative improvement of 12.5\%) at R\@1 and on DOCCI an average improvement of 3.28\% (relative improvement of 4.72\%). Also, it seems that in general the positive margin diminishes as the recall ranking does augment; nonetheless, it is important to say that no negative margins (=worsening) do happen at higher recall ranks, as we will show in the \suppmat. 
%Overall, \ourmethod~is finetuning-agnostic and can reliably inject structural priors under different finetuning strategies to enhance multimodal alignment quality.
 

\begin{table}[t]
\centering
\caption{
\textbf{Cross-domain generalization between DCI and DOCCI.}
Train on one dataset and test on another.
Values are Recall@K (\%), using \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} 
and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval. Within-domain best results are italic bold, best cross-domain results in bold.
}
\label{tab:cross_generalization}
\scriptsize
\setlength{\tabcolsep}{3.6pt}
\renewcommand{\arraystretch}{1.1}

\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lccc|ccc@{}}
\toprule
\textbf{Setting} &
\cellcolor{lightpink}\textbf{R@1} &
\cellcolor{lightpink}\textbf{R@5} &
\cellcolor{lightpink}\textbf{R@10} &
\cellcolor{lightblue}\textbf{R@1} &
\cellcolor{lightblue}\textbf{R@5} &
\cellcolor{lightblue}\textbf{R@10} \\
\midrule

\multicolumn{7}{c}{\cellcolor{gray!10}\textbf{Train on DCI → Test on DCI vs DOCCI}} \\
\midrule
Long-CLIP (DCI→DCI) & \textit{59.23} & \textit{80.89} & \textit{87.04} & \textit{60.13} & \textit{81.44} & \textit{87.54} \\
Long-CLIP (DCI→DOCCI) & 58.73 & 84.66 & 90.75 & 58.08 & 83.53 & 90.47 \\

\lightmidrule
GOAL (DCI→DCI) & \textit{72.64} & \textit{89.89} & \textit{93.70} & \textit{72.84} & \textbf{\textit{90.50}} & \textit{93.20} \\
GOAL (DCI→DOCCI) & 71.22 & 92.39 & 96.47 & 72.18 & 92.88 & 96.49 \\

\lightmidrule
OURS (DCI→DCI) & \textbf{\textit{75.90}} & \textbf{\textit{90.00}} & \textbf{\textit{95.15}} & \textbf{\textit{74.39}} & \textit{89.99} & \textbf{\textit{94.30}} \\
OURS (DCI→DOCCI) & \textbf{75.47} & \textbf{93.41} & \textbf{97.22} & \textbf{72.98} & \textbf{93.24} & \textbf{96.75} \\
\midrule

\multicolumn{7}{c}{\cellcolor{gray!10}\textbf{Train on DOCCI → Test on DOCCI vs DCI}} \\
\midrule
Long-CLIP (DOCCI→DOCCI) & \textit{64.49} & \textit{87.67} & \textit{93.43} & \textit{63.08} & \textit{87.45} & \textit{93.14} \\
Long-CLIP (DOCCI→DCI) & 51.23 & 73.39 & 80.09 & 50.73 & 72.89 & 80.29 \\

\lightmidrule
GOAL (DOCCI→DOCCI) & \textit{79.47} & \textit{96.65} & \textit{98.69} & \textit{79.43} & \textit{96.14} & \textit{97.25} \\
GOAL (DOCCI→DCI) & 64.13 & 82.69 & 87.29 & 65.88 & 83.44 & 87.89 \\
\lightmidrule
OURS (DOCCI→DOCCI) & \textbf{\textit{83.04}} & \textbf{\textit{97.06}} & \textbf{\textit{98.96}} & \textbf{\textit{81.59}} & \textbf{\textit{96.94}} & \textbf{\textit{98.78}} \\
OURS (DOCCI→DCI) & \textbf{65.18} & \textbf{83.89} & \textbf{88.04} & \textbf{66.13} & \textbf{83.84} & \textbf{89.09} \\
\bottomrule
\end{tabular*}
\end{table}

\noindent\textbf{Generalization across general domains.}
Following the evaluation setting in the prior work~\cite{goal2025}, we also investigate the finetuned models in cross-domain settings on the two general-domain DCI and DOCCI dataset. Tab.~\ref{tab:cross_generalization} shows that \ourmethod~demonstrates decent cross-domain generalization capability between DCI and DOCCI, with only a marginal decrease compared to in-domain results.
Nonetheless, \ourmethod~still outperforms GOAL and LongCLIP by a clear margins.
This indicates that the auxiliary structure-centric alignment does not bias the model toward specific domain-specific representation, but instead promotes generalizable representation that can transfer well across different image-text distributions. In the case of cross general-specific domain generalization (showed in the \suppmat), the general decrease in performance is evident, with \ourmethod still showing comparable if not better robustness compared to the other approaches.\mc{is this true?}  \yiming{we might also give a mention to cross general-specific domain generalization in supp. We can consider do sketchy and DCI/DOCCI.}


\subsection{Ablation studies}

\noindent\textbf{Structure-centric alignment losses.} \yiming{to revise here} We ablate the impacts of our introduced structure-centric alignment losses. As shown in Tab.~\ref{tab:ablation_loss}, all three losses $\mathcal{L}{I',T'}$, $\mathcal{L}{I,I'}$, and $\mathcal{L}{I',T'}^{local}$ contribute positively to performance.
Introducing the global structure alignment loss $\structloss$ already yields a clear improvement, indicating that explicitly aligning structural semantics enhances geometric consistency between vision and language.
Adding the consistency regularization $\consistencyloss$ further stabilizes learning while maintaining coherence with the original semantic space.
Finally, incorporating the local structure alignment loss $\structlosslocal$ achieves the best results, confirming the complementarity of multi-level structural constraints, global alignment enforces holistic shape consistency, while local alignment strengthens fine-grained correspondence, leading to higher retrieval precision and robustness.
\begin{table}[t]
\centering
\caption{
\textbf{Ablation on losses.}
Results on \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and 
\inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval for SKETCHY and DOCCI.
Each subsequent row adds one additional loss term to the previous configuration.}

\label{tab:ablation_loss}
%\scriptsize
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\columnwidth}{!}{%
{\fontsize{23}{28}\selectfont
 % \begin{tabular}{@{} ccccccccc|cccccc @{}}
 \begin{tabular}{@{} ccc  *{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c| *{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c @{}}
\toprule
\multirow{2}{*}{$\structloss$} &  \multirow{2}{*}{$\consistencyloss$} &  \multirow{2}{*}{$\structlosslocal$} &
\multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{SKETCHY}} &
\multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
\cmidrule(lr){4-9}\cmidrule(lr){10-15}
&&& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c|}{\cellcolor{lightblue}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\
\midrule

\textcolor{red!75}{\usym{2717}} & \textcolor{red!75}{\usym{2717}} & \textcolor{red!75}{\usym{2717}} & 
66.75 & 89.55 & 93.61 & 64.51 & 88.76 & 93.44 & 80.38 & 96.45 & 98.76 & 79.43 & 96.51 & 98.69 \\
\textcolor{lightgreen}{\usym{2713}} & \textcolor{red!75}{\usym{2717}} & \textcolor{red!75}{\usym{2717}} & 
67.88 & \textbf{90.85} & 95.34 & 67.18 & 89.21 & 94.91 & 81.20 & 96.83 & 98.95 & 80.69 & 97.04 & 98.73 \\
\textcolor{lightgreen}{\usym{2713}} & \textcolor{lightgreen}{\usym{2713}} & \textcolor{red!75}{\usym{2717}} & 
68.57 & 90.50 & \textbf{95.60} & \textbf{68.22} & 89.64 & 95.16 & 81.92 & 97.01 & \textbf{98.98} & 81.05 & \textbf{97.10} & 98.75 \\
\textcolor{lightgreen}{\usym{2713}} & \textcolor{lightgreen}{\usym{2713}} & \textcolor{lightgreen}{\usym{2713}} &
\textbf{69.86} & \textbf{90.85} & 95.42 & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} & \textbf{83.04} & \textbf{97.06} & 98.96 & \textbf{81.59} & 96.94 & \textbf{98.78} \\


\bottomrule
\end{tabular}
}
}
\end{table}

\noindent\textbf{Types of extraction methods.} We investigate the effects of different extraction strategies on both the visual and textual sides. Overall, all types of structure-centric extraction lead to consistent performance improvements, indicating that the model exhibits strong adaptability to the extraction strategy. On the visual extraction side, we consider two categories of structure extraction methods:
(i) classic \emph{filter-based} edge extraction methods (e.g., Canny~\cite{canny2009computational} and LoG~\cite{marr1980theory}), and
(ii) \emph{learning-based} methods (e.g., HED~\cite{xie2015holistically}, LineArtDetector~\cite{zhang2023adding}, and Photo2Sketch~\cite{liu2021learn}).
The filter-based approaches achieve the best overall performance, while learning-based extractors yield comparably strong results with only marginal differences, suggesting that the model can effectively exploit various forms of edge features. For the \emph{textual extraction}, we compare the original text and the LLM-based extraction.
The \textbf{Original Text} retains appearance-related vocabulary, while the \textbf{LLM-based Extraction} emphasizes structure-centric semantics but may introduce hallucinated attributes.
Our method balances factual grounding and structural relevance, achieving the best results.
To further assess model robustness, we introduce a \emph{Noise Injection} setting.
On the visual side, \emph{Incorrect Match} randomly pairs an image with edge maps from a different dataset (matching DOCCI edges with SKETCHY images, vice versa).
On the textual side, \emph{Random Word Mask} randomly removes all non-structural and non-functional words outside the vocabulary $\vocappearance$,
and \emph{Word Reduction (90\%)} retains only about 10\% of the original words to simulate severe semantic loss. As shown in Tab.~\ref{tab:extraction_ablation}, both the visual and textual noise experiments cause only minor degradation,
demonstrating that the model remains stable and reliable even under structural perturbations,
and exhibits strong robustness. The 90\% reduction variant underperforms on SKETCHY, as its relatively short captions make it difficult for the remaining 10\% of words to cover most objects. More implementation details are provided in the \suppmat.



\mc{this is very interesting, my intuition is that if edges are wrong, we are just adding noise (uncorrelated gradients) which due to the high variance will be trated as noise, the convergence will be slowed down, but nothng really problematic will show up. This could be an experiment to be done.}
\mc{there is a strong focus on investigating on the image side. To me we should do a similar experiment when we do random masking of the words, keeping the edge correct, and when both edge are wrong and words are randomly masked}.

% \begin{table}[t]
% \centering
% \caption{
% \textbf{Ablation on types of structure-centric image.}
% Comparison of different edge extraction formats 
% for \inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} 
% and \inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval
% on SKETCHY and DOCCI.
% }
% \label{tab:edge_format_ablation}
% %\scriptsize
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.1}

% \resizebox{\columnwidth}{!}{
% {\fontsize{23}{28}\selectfont
% \begin{tabular}{@{}l *{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c|*{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c @{}}
% % \begin{tabular}{@{}lcccccc!{\color{lightlightgray}\vrule width 0.5pt}cccccc@{}}
% \toprule
% \multirow{2}{*}{\textbf{Edge Format}} &
% \multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{SKETCHY}} &
% \multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
% \cmidrule(lr){2-7}\cmidrule(lr){8-13}
% & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c|}{\cellcolor{lightblue}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
% & \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\

% \midrule
% \cmidrule(r){1-13}
% \multicolumn{13}{l}{\textit{Filter-based methods}} \\
% \lightmidrule
% Canny~\cite{canny2009computational} (\textbf{Ours}) & \textbf{69.86} & 90.85 & 95.42 & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} & 83.04 & 97.06 & 98.96 & 81.59 & 96.94 & 98.78 \\
% LoG~\cite{marr1980theory} & 68.48 & 89.64 & 94.91 & 67.36 & 90.24 & 94.47 & \textbf{83.59} & \textbf{97.36} & \textbf{99.20} & \textbf{81.98} & \textbf{97.41} & \textbf{99.04} \\
% HEG~\cite{xie2015holistically} & 68.91 & 90.67 & \textbf{95.43} & 66.93 & 90.41 & 94.47 & 83.14 & 97.18 & 98.98 & 81.73 & 97.08 & 98.69 \\
% \cmidrule(r){1-13}
% \multicolumn{13}{l}{\textit{Learning-based methods}} \\
% \lightmidrule
% LineArtDetector~\cite{zhang2023adding} & 69.17 & \textbf{90.93} & 95.42 & 66.93 & 90.16 & 94.91 & 82.69 & 97.10 & 98.90 & 81.08 & 96.84 & 98.84 \\
% Photo2sketch~\cite{liu2021learn} & 68.14 & 90.76 & 94.99 & 67.53 & 90.16 & 94.04 & 81.49 & 97.02 & 98.73 & 80.20 & 96.43 & 98.47 \\
% \cmidrule(r){1-13}
% \multicolumn{13}{l}{\textit{Incorrect / negative control}} \\
% \lightmidrule
% Incorrect match & 66.20 & 88.95 & 93.39 & 64.37 & 88.26 & 93.78 & 80.25 & 96.33 & 98.76 & 79.15 & 96.10 & 98.41 \\
% \lightmidrule
% Random Word Mask & 68.91 & 89.98 & 93.96 & 67.19 & 88.95 & 94.04 & 81.49 & 96.53 & 98.74 & 80.49 & 96.55 & 98.62 \\
% Word Reduction (90\%) & 62.00 & 86.96 & 92.66 & 60.62 & 86.01 & 92.57 & 81.00 & 96.48 & 98.76 & 79.61 & 96.53 & 98.62 \\
% \bottomrule
% \end{tabular}
% }
% }
% \end{table}

\begin{table}[t]
\centering
\caption{
\textbf{Ablation on extraction methods.}
\inlineColorbox{lightpink}{\emph{Text$\rightarrow$Image}} and 
\inlineColorbox{lightblue}{\emph{Image$\rightarrow$Text}} retrieval on SKETCHY and DOCCI datasets. 
[F] indicates \emph{filter-based} and [L] indicates \emph{learning-based} edge extraction methods. Bold numbers indicate the best results within each subtable.
}
\label{tab:extraction_ablation}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.98}

% -------------------- (a) VISUAL --------------------
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l *{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c|*{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c @{}}
\toprule
\multirow{2}{*}{\textbf{(a) Visual Extraction}} &
\multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{SKETCHY}} &
\multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c|}{\cellcolor{lightblue}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\
\midrule
\multicolumn{13}{l}{\textit{Methods}} \\
Canny~\cite{canny2009computational} [F] & \textbf{69.86} & 90.85 & 95.42 & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} & 83.04 & 97.06 & 98.96 & 81.59 & 96.94 & 98.78 \\
LoG~\cite{marr1980theory} [F] & 68.48 & 89.64 & 94.91 & 67.36 & 90.24 & 94.47 & \textbf{83.59} & \textbf{97.36} & \textbf{99.20} & \textbf{81.98} & \textbf{97.41} & \textbf{99.04} \\
HED~\cite{xie2015holistically} [L] & 68.91 & 90.67 & \textbf{95.43} & 66.93 & 90.41 & 94.47 & 83.14 & 97.18 & 98.98 & 81.73 & 97.08 & 98.69 \\
LineArtDetector~\cite{zhang2023adding} [L] & 69.17 & \textbf{90.93} & 95.42 & 66.93 & 90.16 & 94.91 & 82.69 & 97.10 & 98.90 & 81.08 & 96.84 & 98.84 \\
Photo2Sketch~\cite{liu2021learn} [L] & 68.14 & 90.76 & 94.99 & 67.53 & 90.16 & 94.04 & 81.49 & 97.02 & 98.73 & 80.20 & 96.43 & 98.47 \\
\midrule
\multicolumn{13}{l}{\textit{Noise Injection}} \\
Incorrect match & 66.20 & 88.95 & 93.39 & 64.37 & 88.26 & 93.78 & 80.25 & 96.33 & 98.76 & 79.15 & 96.10 & 98.41 \\
\bottomrule
\end{tabular}
}

\vspace{2pt}

% -------------------- (b) TEXTUAL --------------------
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l *{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c|*{5}{c!{\color{lightlightgray}\vrule width 0.5pt}}c @{}}
\toprule
\multirow{2}{*}{\textbf{(b) Textual Extraction}} &
\multicolumn{6}{c|}{\cellcolor{gray!15}\textbf{SKETCHY}} &
\multicolumn{6}{c}{\cellcolor{gray!15}\textbf{DOCCI}} \\
\cmidrule(lr){2-7}\cmidrule(lr){8-13}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c|}{\cellcolor{lightblue}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightpink}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightpink}{R@10}}
& \multicolumn{1}{c}{\cellcolor{lightblue}{R@1}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@5}} & \multicolumn{1}{c}{\cellcolor{lightblue}{R@10}} \\
\midrule
\multicolumn{13}{l}{\textit{Methods}} \\
Original Text & 66.93 & 89.38 & 93.35 & 64.51 & 88.00 & 93.01 & 81.02 & 96.88 & 98.67 & 80.29 & 96.61 &98.73 \\
LLM-Extraction  & 67.36 & 90.24 & 94.65 & 67.70 & 89.12 & 94.30 &81.08 & 97.02 & 98.59 & 80.22 &  96.61 &  98.65 \\
Ours   & \textbf{69.86} & \textbf{90.85} &\textbf{ 95.42} & \textbf{68.22} & \textbf{90.67} & \textbf{95.68} & \textbf{83.04} & \textbf{97.06} & \textbf{98.96} & 81.59 & \textbf{96.94} & \textbf{98.78} \\
\midrule
\multicolumn{13}{l}{\textit{Noise Injection}} \\
Random Word Mask & 68.91 & 89.98 & 93.96 & 67.19 & 88.95 & 94.04 & 81.49 & 96.53 & 98.74 & 80.49 & 96.55 & 98.62 \\
Word Reduction (90\%) & 62.00 & 86.96 & 92.66 & 60.62 & 86.01 & 92.57 & 81.00 & 96.48 & 98.76 & 79.61 & 96.53 & 98.62 \\
\bottomrule
\end{tabular}
}
\end{table}

%indicating that our structure-centric losses do not rely on exact edge-image correspondences. This suggests that our method does not rely on strict pixel-level edge correspondence; instead, the structure-centric losses serve primarily as a regularization that enhances training stability and general visual-text alignment. \zanxi{Further polishing is required.}
%
\noindent\textbf{Sample efficiency.} We present in Fig.~\ref{fig:data.amount} showing how \ourmethod performs with varying ratio of the training dataset, in comparison with other sota methods. Our approach betters the competitors at every regime. Notably, the margin seems to be maximized around 20-50\% of the training data, especially with the DOCCI dataset. Notably, \ourmethod on Sketchy has the steepest ascent, with an absolute gap of 16.5 in Text$\rightarrow$Image (relative increase of 45\%). This because Sketchy is more fine-grained than DOCCI, and its statistics could explained with a larger amount of data, in percentage. \mc{should we put statistics in terms of presence of edges/number of appearance based words in the different datasets? this could make a difference} 

%Our approach exhibits strong performance in the few-data fine-tuning regime because it focuses the optimization on the informative components of the signal. 
%In standard global fine-tuning, the model must adapt a large parameter space to account for every visual and textual variation, including nonsemantic noise, which requires extensive supervision. 
%In contrast, our disentangled extractions $X_E$ and $Y_E$ isolate structural cues such as edges and textual chunks that retain the core semantics while suppressing nuisance factors. 
%The accompanying objectives $\mathcal{L}_{\text{ST}}$, $\mathcal{L}_{\text{RS}}$, and $\mathcal{L}_{\text{CK}}$ further constrain the alignment toward consistent and interpretable relations across modalities. 
%This structural bias effectively reduces the hypothesis space and the variance of gradient updates, yielding faster convergence and improved generalization under limited data. 
%In simple terms, the model learns less but better, focusing its capacity on semantically stable features that global fine-tuning must otherwise relearn from larger datasets.


% \subsection{Interplay with GOAL}
% As shown in Table~\ref{tab:goal_interplay}, GOAL improves general-domain alignment but can degrade performance on structure-centric datasets; combining GOAL with our objectives mitigates this and brings further gains.

\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/retrieval3.pdf}
    \caption{Four examples of retrieval results: above, two examples for DOCCI. Below, two examples for Sketchy}
    \label{fig:retrieval}
    \vspace{-8pt}
\end{figure*}

\subsection{Qualitative analysis}
Fig.~\ref{fig:retrieval} shows two retrieval results: above on the DOCCI dataset, below on Sketchy. Apart from the better performance of \ourmethod, there is a substantial difference on the gist of the retrieved images: on DOCCI, \ourmethod extracts images that match more structure details (lamps and people are more present). One may think we are forgetting colors due to our emphasis on structure, but this is not the case: the brown, green and light azure patterns are also evident. On the Sketchy dataset, it appears that the shorts are more present in the \ourmethod retrieved results. This is probably due to the structure analysis which emphasis shape and contours of the garment item, absent in the competitor.  These motivations could be substantiated by the attention map of Fig.~\ref{fig:attentionmap}, where we visualize the cross-modal attention between the textual descriptions of each object and the image. On the Sketchy dataset (first row), it is evident how we match the dress with a very sharp attention map, contrarily to the baseline \mc{specify which is the baseline}. This is also evident in the second row, where the attention is uniquely focused on the dress, differetnly from the baseline. On the DOCCI example (third line) the back of the cat's head is correctly highlight by \ourmethod. Surprisingly, even the corner of the white window is also salient, showing a good sensibility to colors. Finally (fourth row) a very nice showcase of the \ourmethod's ability in capturing the correct layout of the image, with the baseline completely ignoring the tree branch on the floor, correctly highlighted by us.  

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/sailencymaps3.pdf}
    \caption{Saliency maps given by GRAD-CAM about the cross-modal attention between the textual descriptions of a specific object contained in the text caption and the image.}
    \label{fig:attentionmap}
\end{figure}

%The good retrieval performance obtained by \ourmethod thanks to the better semantic alignment especially along the structural direction. When visualizing the cross-modal attention between the textual description of each object on the image, as shown Fig.~\ref{fig:attentionmap}, we can clearly observe that \ourmethod~demonstrates a better semantic alignment especially on the structural descriptions, \eg shape, positioning, spatial relations. For instance, \yiming{referring to the images to give more grounded discussion}.

==> sec/old/intro.12.11.25.tex <==

\section{Introduction}
\label{sec:intro}
Vision-language models (VLMs)~\cite{radford2021learning,zhai2023siglip}
%and SigLIP~\cite{zhai2023siglip} 
have become foundational ingredients in modern computer vision, thanks to their aligned representations across visual and textual modalities.
While the pre-trained VLMs, such as CLIP~\cite{radford2021learning}, have demonstrated impressive generalization capability, finetuning is often required to be competitive on downstream tasks in specific domains~\cite{zhang2024longclip,he2025double, xu2025fate,noori2025test,zhai2022lit,zhou2022coop,zhou2022cocoop,khattak2023maple,zhu2023prograd,zhang2022tipadapter,gao2023clipadapter,hu2022lora,liu2024dora,yang2024mma,guo2025mmrl,jiang2025ucdr}.\mc{Zanxi,Qiuyu you need to check which of these should be kept... maybe some are too out oof focus} 
%has become the primary means of interacting with and adapting these models to specific domains.
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{imgs/TeaserTeal5.pdf}
    \caption{\ourmethod~can be seamlessly integrated into any CLIP-family model. It operates by generating edge maps using standard edge detectors and by refining captions to remove non-structural information such as color or material terms. This structure-centric fine-tuning consistently improves downstream vision–language retrieval performance.}
    \label{fig:example}
\end{figure}

%
However, finetuning VLMs remains challenging, especially when images feature rich visual details and structural complexity, as it demands the alignment with lengthy semantically-rich textual descriptions.
Pre-trained VLMs (VLMs)~\cite{radford2021learning,zhai2023siglip} are limited in such long-text alignment due to its token length constraint~\cite{zhang2024longclip,goal2025,smartclip2025}.
To address this challenge, the seminal work Long-CLIP~\cite{zhang2024longclip} extends CLIP to support longer descriptions via positional interpolation. However, training CLIP with long descriptions involving rich semantic concepts encourages the model to learn entangled representations of multiple concepts~\cite{lai2024veclip}, limiting its generalization to novel semantic combinations.
As mitigation, recent works such as GOAL~\cite{goal2025} further incorporates local alignment by associating textual fragments with image regions, while SmartCLIP~\cite{smartclip2025} introduces a modular alignment through adaptive masking to optimize two goals, \ie preserving cross-modal information and disentangling concepts at diverse granularity levels.
%it remains challenging to explicitly extract object/conceptcentric representations from CLIP’s visual representation. This entanglement is particularly problematic for tasks that require individual, atomic concepts or novel combinations of them, 
While we find compelling the idea of disentangling concepts across image and text representations, achieving reliable semantic disentanglement heavily depends on pre-trained models, which may be limited in low-data settings or domains where certain concepts are underrepresented.

%it is difficult to achieve in practice, especially in low-data or domain-specific settings where disentangling multiple semantic factors becomes unreliable.
%\yiming{I did not get why low-data aor domain-specific unreliable, this part probably should be more explicit, it it because they are dependent on pre-trained models to do disentanglement, while low-data is underrepresented.}.

% Introduce VLM quickly
%Vision-language models (VLMs) pre-trained by aligning web-scale image-text pairs, have revolutionized the methodological design in addressing vision tasks, \eg~image classification, cross-modal retrieval, achieving good generalization capability~\cite{}.
% Motivate why we are studying long text
%Yet, pre-trained VLMs (\eg, CLIP~\cite{radford2021learning} or SigLIP~\cite{zhai2023siglip}) are constrained by the 77 text tokens, limiting its application in domains where fine-grained semantic details are critical, \eg fashion design, or fine-grained image classification. 
%Such rich semantics contained in the visual content (\ie visual semantics) often yield lengthy language description, whose alignment remains a challenging research topic. Recent works, such as LongCLIP~\cite{zhang2024longclip}, SmartCLIP~\cite{smartclip2025}, GOAL~\cite{goal2025}, have introduced finetuning methods on top of CLIP by ... \yiming{short summary of what they do, 1-2 sentences}. 
%
% What is the problem of existing methods. 
%However, existing methods treat such semantic-rich vision-language alignment in an over simplistic way, by learning an entangled representation without carefully accounting for heterogeneous visual semantics, limiting interpretability and precision \yiming{to revise, some key words are warning: entangled, interpretability}. 
%What is our intuition.
%Is this the most effective way?
%First, \textbf{\textit{visual semantics are not monolithic}}. Entities in an image can carry diverse fine-grained attributes, covering both pictorial appearance (\eg, colors, textures, materials) and structural characteristics (\eg, shapes, patterns, spatial arrangement).
%Second, \textbf{\textit{visual semantics can be best conveyed differently}}. For instance, color images excel at representing pictorial semantics, while edge maps or sketches can better capture structural semantics like shape and spatial composition, as shown in Fig.~\ref{fig:example}.


Departing from model-dependent semantic disentanglement, we introduce \ourmethod, a vision-language fine-tuning framework that shifts the focus on a more fundamental representation space: the one defined by the geometrical structure of an image, namely its \emph{edges}.
In decades of computer vision research, edges have been recognized as essential primitives for visual understanding~\cite{marr1980theory,survey2002edge}, encoding object boundaries and spatial layout.
Building on this foundation, \ourmethod extracts edge maps to capture structure-centric information in the visual channel. The same idea extends to text. \ourmethod refines captions by removing tokens that describe color, material, or other appearance-related properties, while preserving linguistic elements that encode shape and spatial relations. This yields a structure-centric text that naturally pairs with edge maps, enforcing multimodal alignment on the basis of structural cues rather than appearance.
The alignment process supplements the standard contrastive objective (a longclip-derived contrastive loss\mc{ZANXI check this out!}) with three structure-centric losses. The first aligns edge maps with the filtered text, the second establishes fine-grained correspondences between local edge regions and chunks of the filtered text, and the third links edge maps to the original color images to prevent representational drift.

From a theoretical standpoint, \ourmethod can be viewed as maximizing the mutual information between the visual and textual channels, approximated by the InfoNCE loss~\cite{math_lower_bound}. The auxiliary objective extends this functional by introducing an additional maximization between the structure-centric visual representations and their textual counterparts. This objective can be interpreted as a correlated, information-reduced task that introduces gradient diversity without conflicting with the main optimization.
In fact, information-theoretic analyses of multitask learning~\cite{MTLasMOO.NIPS18} and gradient diversity~\cite{wu2020mutualinformationcontrastivelearning} show that auxiliary losses with lower mutual information act as implicit regularizer, expanding the effective search space and improving convergence. 
In this view, our structure-centric alignment loss provides complementary gradient directions that remain active when the main contrastive gradients flatten, consistent with multi-objective optimization theory~\cite{gradientSGDvariantNIPS20}. 


%Explain our method
%Building on this intuition, we explore an alternative fine-tuning pathway that \textit{explicitly separates and align different types of visual semantics} to enhance vision-language representation learning. 
%Our study is primarily based on extracting the \emph{structural semantics} from both the visual and textual content, for its fundamental significance in visual understanding from from early theories of human vision to classical computer vision pipelines. 
%Edge information has long been recognized as a fundamental component of visual understanding—from early theories of human vision to classical computer vision pipelines, where edges define object boundaries, shapes, and spatial relationships. 
%We present an effective model-agnostic finetuning method \ourmethod, that extracts structural cues from raw visual and textual content and injects them as auxiliary supervision during the contrastive training framework.
%This regularizes mutual information estimation through low-variance structured counterparts, stabilizing optimization and sharpening cross-modal correspondences. 
%\yiming{DESCRIBE METHOD, remember to  first describe extraction (highlight the computation for extracting edges are negligible with existing tools.), then talk about the alignment (\ie you novel losses)}. 
%here is about how we evaluate


Through cross-modal retrieval experiments, \ourmethod~scores new state-of-the-art performance against existing approaches on both general-purpose dense captioning datasets and domain-specific datasets where rich visual semantics dominate, such as fashion and fine-grained image classification.
Moreover, when our three structure-centric losses are integrated into existing fine-tuning frameworks, performance consistently improves in every case, demonstrating a finetuning-agnostic enhancement. Finally, we show that \ourmethod exhibits generalization capabilities on par with other advanced fine-tuning strategies.
In the ablation studies, we show that any edge extraction approach is beneficial, with surprisingly the best performance obtained using classical filter-based operators (Canny, LoG)~\cite{gonzalez_digital_2018}. Explainability analyses further reveal that our model attends to shape-related regions consistent with human perception, while numerical evidence supports our mutual-information–based theoretical assumptions, confirming that structure-centric alignment contributes to more stable and informative optimization dynamics. Finally, \ourmethod also outperforms competing approaches under data-scarce conditions, demonstrating a strong inductive bias toward structural regularities that enables robust learning even with limited supervision.
%achieves \textit{model-agnostic improvement} but also maintains \textit{good generalization capability}. 
%here is we can give some insight on key ablation
%We dive into what characteristics of edges are most effective in such alignment \yiming{here is we can give exciting insights on key ablation conclusion}.
%Moreover, we provide theoretical foundation from the perspective of mutual information \yiming{please update if it is no longer MI}) to explain why such visual and structural semantic separation leads to more aligned (\yiming{is it correct to say this?}) representations in the shared space.  

%Contribution summary
\noindent \textbf{Our main contributions} are summarized as follows:
\begin{itemize}
    \item We demonstrate that incorporating multimodal, structure-centric cues into standard contrastive learning significantly enhances vision–language alignment.
    \item Our \ourmethod~is plug-and-play and effective, outperforming recent vision–language finetuning methods without introducing architectural complexity.
    \item Our theoretical motivation based on mutual information and optimization analysis, shows how structure-centric alignment enhances stability and convergence.
    \item Our extensive analysis demonstrates that \ourmethod achieves strong generalization and interpretability, remaining robust to the edge extraction choice.
\end{itemize}




%[MARCO this below can help anchoring our idea to the literature]
% \yiming{need to inject it somewhere}Recent studies show that introducing structural priors early in the learning pipeline can guide multimodal alignment without replacing the raw input. 
% Disentangled or geometry-aware representations have been used to improve compositional reasoning and retrieval performance \cite{li2024deal,zhou2022vdr,jin2023dicosa}.
%This unified treatment assumes that both modalities encode comparable semantic content, overlooking the fact that images and texts inherently capture different kinds of information. 








%Recent works such as DEAL~\cite{li2024deal}, DisCoCLIP~\cite{discoclip2025}, TaSe~\cite{tase2025}, and SmartCLIP~\cite{smartclip2025} have started to explore disentanglement in vision--language alignment, mainly by decomposing textual semantics or modularizing alignment mechanisms. 
%Yet these approaches still treat the visual and textual streams as if they carried the same type of information.




\iffalse
Vision–language models like CLIP, achieve remarkable cross-modal generalization by performing contrastive learning on web-scale image–text pairs. To further address long and detailed descriptions, subsequent work such as GOAL introduces a fine-tuning paradigm for long-text retrieval, establishes mappings between text substrings and local image regions through global–local alignment, which significantly improves retrieval performance in long-description scenarios.

When applied to expert domains such as medical imaging, fine-grained fashion, or biological analysis, this paradigm encounters a fundamental limitation: existing local representations rely on rectangular regions as geometric proxies, which are overly coarse. These rectangular boundaries indiscriminately mix critical diagnostic features with substantial irrelevant background, hindering precise alignment between textual descriptions and key visual evidence. This results in low-density supervision and reduced learning efficiency. In expert domains where data is scarce and annotations are costly, such low-density supervision demands more data yet still struggles to capture stable fine-grained structures. However, expert interpretation critically relies on geometric evidence such as boundary shapes, orientations, and topological relationships.  We summarize this issue as a \textbf{granularity gap}: the geometric granularity of supervision (rectangular proxies) does not match the cognitive granularity of the task (precise structures), which in turn limits both the efficiency and the ultimate performance of fine-tuning.

To bridge the above gap, we propose Scribble-Augmented Semantics (SAS), a novel annotation and learning paradigm designed to precisely align the geometric granularity of supervision with the cognitive granularity required by experts. In this paradigm, training samples are extended from $\langle image, text \rangle$ pairs to $\langle image, text, geometric\ cues \rangle$ triplets,
, where the geometric cues are provided by sparse scribbles or simple masks that convey contours and orientations with very low cost. \textcolor{red}{TO BE COMPLETED} Based on SAS, we first perform geometry-conditioned aggregation using the geometric cues, producing geometry-focused features with background suppressed. We then parse the long text to extract geometry-relevant substrings. Finally, we enforce both global and local alignment constraints between the geometry-focused features and the extracted substrings. In this way, the training signal is effectively concentrated on high-value evidence such as boundaries and shapes, significantly increasing information density and data efficiency. Importantly, geometric prompts serve as supervision signals only during the training phase, while remaining entirely absent during inference, thereby ensuring both model generalizability and deployment efficiency.

Our proposed framework is particularly effective in expert domains because scribbles serve as low-cost yet highly informative geometric cues. Since scribbles are natural byproducts of expert workflows, they can be provided with minimal annotation effort—just seconds to minutes—while offering far superior supervision compared to rectangles. By leveraging this geometric alignment, the model learns the true structural cues that drive expert decision-making from significantly less data, dramatically improving fine-tuning efficiency. This enhanced geometric understanding benefits not only long-text retrieval but extends naturally to boundary-sensitive tasks like grounding and segmentation. We evaluate long-text retrieval, referring expression grounding, and weakly supervised segmentation across four heterogeneous domains: general objects, specialized species, fashion, and medical imaging. Experimental results demonstrate that in expert domains, our method achieves or even exceeds the performance of rectangular alignment baselines using only approximately 60\% of the annotation data. We also constructed and released data resources and annotation specifications conforming to the SAS paradigm.

The main contributions of this work include: 1) Proposing Scribble-Augmented Semantics, a novel annotation and fine-tuning paradigm that fundamentally addresses the granularity gap problem in existing fine-grained alignment approaches by introducing low-cost geometric prompts. 2) Providing a highly data-efficient solution for expert domain VLM applications, achieving stronger geometric understanding capabilities and superior localization and segmentation performance with reduced annotation costs and less fine-tuning data. 3) Constructing and releasing datasets and annotation specifications conforming to the SAS paradigm, providing a solid foundation and evaluation benchmark.
\fi


==> sec/old/method.12.11.2025.tex <==
\section{\ourmethod}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{imgs/method3.pdf}
    \caption{The four components of \ourmethod: starting from the left, a generic type of CLIP could be adopted. In this paper, we adopt a \mc{Zanxi complete here!!!}. The three dots in parenthesis indicate this freedom of choice. The second loss considers the embedding of the edge maps $\{I'_i\}$ and of the structure-centric textual descriptions $\{T'_i\}$, pairing them as an ordinary CLIP alignment. The third loss introduces fine-grained cross-modal analysis associating every text chunk embedding with the $K$-most related edge regions. Finally the fourth loss is a general regularizer which enforce visual and structural visual embeddings to stay close in the embedding space.}
    \label{fig:overview}
\end{figure*} 
%Our proposed method \ourmethod, a novel finetuning method that explicitly extracts structural semantics from visual and textual modalities to enable more precise vision-language alignment on rich and fine-grained semantic details. 
%As shown in Fig.~\ref{fig:overview}, \ourmethod~operates in two main stages: i) the \textbf{structural semantics extraction} stage explicitly isolates the structural cues (\eg geometrical attributes, spatial relations, layout) from original semantic-rich image-text pairs, yielding structure-centric visual content in the format of edge maps, and corresponding textual description that only features the structural attributes;
\ourmethod~operates in two main stages (Fig.~\ref{fig:overview}): 
%
i) the \textbf{structure-centric multimodal extraction} stage produces simplified yet complementary views: edge maps that retain the geometric structure of the image, and filtered captions that preserve the structure of the description (what are the objects contained in the image, their layout) while removing appearance-related terms such as color, lighting, and material properties. 
%
%ii) the \textbf{structural semantics alignment} aligns the multimodal structure-centric inputs jointly with the original image-text pairs, at both global and local levels. We introduce novel \textit{alignment losses} to enhance the vision-language alignment in semantic-rich conditions.
%
ii) the \textbf{structure-centric alignment} stage aligns the structure-preserving representations at both global and local levels, jointly with the original image–text pairs. The designed losses aims to enhance vision-language alignment under semantically rich conditions.
Note that the structure-centric multimodal content are only leveraged during the training phase. At inference, only original images and texts are involved in downstream tasks.

\subsection{Structure-centric multimodal extraction}
\label{Structural_extraction}
We first extract structure-centric cues from both visual and textual modalities. Let us consider a color image $\image \in \visualspace$ which is visually described by a textual description $\desc \in \textspace$. Each image $\image_i$ and its visual description are paired $(\image_i,~\desc_i)$. 

\noindent\textbf{Visual extraction.}
We employ a light-weight structure-oriented extractor, such as any filter-based~\cite{canny2009computational} or learning-based~\cite{} edge detector, to effectively capture geometric and spatial cues of the image, obtaining its structure-centric view $\imagestruct$.
%Based on this observation, we employ an edge-based structural extractor, where the default implementation adopts the Canny operator to generate structure-oriented views from RGB images.
Formally, for each image $\image_i$, the structure-oriented view $\imagestruct$ is obtained as $\imagestruct_i = \structextractor(\image_i)$, where $\mathcal{E}(\cdot)$ denotes a general-purpose structure operator. Note that our framework is agnostic to any type of extractor, as empirically proved Sec.~\ref{sec:exp}.
%in such as learning-based edge detectors or sketch-based generation approaches.


\noindent\textbf{Textual extraction.}
Similar to the image-side operation, we extract a structure-centric textual description that emphasizes layout, geometric attributes, and spatial relations. This choice is motivated by evidence that appearance-based language (specifically, color and material) often fails to align with visual discriminability, whereas spatial and shape-related semantics better capture grounded meaning in vision–language tasks~\cite{xu2023vgse}. In this way, we produce a textual representation complementary to the edge-based visual cues.
To this aim, we leverage the strong semantic understanding capability of a large language model (LLM),  prompting it to construct a set of appearance-related vocabulary $\vocappearance$ to be filtered from the original description.
%We opt not to directly prompt the LLM to perform rewriting of the original $\desc_i$ to remove appearance-related terms, as such rewriting process is difficult to control in terms of hallucinations or semantic drift. 
Specifically, 
%\begin{equation}
%\vocappearance = \mathcal{LLM}(\prompfiltering),
%\end{equation}
%where $\prompfiltering$ is the prompt that queries the LLM to produce appearance-centric semantic concepts that cannot be directly inferred from the structure-centric visual content $\imagestruct$. The resulted vocabulary $\vocappearance$ broadly covers colors, materials and textures. 
%\begin{equation}
$\vocappearance = \mathcal{LLM}(\prompfiltering)$, 
%\end{equation}
where $\prompfiltering$ is the prompt that queries the LLM to produce semantic concepts related to colors and materials, resulting in the vocabulary $\vocappearance$. %The resulted vocabulary $\vocappearance$ broadly covers colors, materials and textures.
We then obtain the structure-centric text $\textstruct_i$ by filtering out terms that are inside $\vocappearance$ from $\desc_i$:  
%\begin{equation}
$\textstruct_i = \mathcal{F}(\desc_i, \vocappearance)$,
%\end{equation}
where $\mathcal{F}(\cdot)$ is the filtering function based on regular expression matching to remove any semantic concept are within $\vocappearance$. Please refer to \suppmat~for the prompt $\prompfiltering$ and vocabulary $\vocappearance$ used in the filtering processes.
%The mechanism is annotation-free and transferable to diverse domains.
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/edge_examples4.pdf}
    \caption{Examples of visual and textual extraction: on the left, visual edges are extracted using Canny~\cite{gonzalez_digital_2018}, while on the right, words related to color and material are removed from the text without compromising its linguistic naturalness.}
    \label{fig:edge}
\end{figure}
\subsection{Structure-centric multimodal alignment}
Let us consider a VLM $f_\mathtt{VLM}$ with two main elements: the visual encoder $\visualencoder$ and the text encoder $\textencoder$.
The encoders map their respective inputs into a shared $d$-dimensional embedding space, \ie, $\visualencoder:\visualspace \rightarrow \sharedspace$ and $\textencoder:\textspace \rightarrow \sharedspace$.
In particular, as visual encoder $\visualencoder$ we use ViTB/16~\cite{dosovitskiy2021vit}. As text encoder $\textencoder$, we employ the Knowledge Preserving Stretching (KPS) strategy from Long-CLIP~\cite{zhang2024long} to extend CLIP’s text encoder for long-text inputs. KPS enlarges the positional embedding range beyond CLIP’s original 77-token limit by reusing the first 20 well-trained embeddings and interpolating the remaining ones according to a stretching ratio. This VLM brings in the image-text alignment loss $\originalloss$: a  symmetric InfoNCE loss~\cite{math_lower_bound} with cosine similarity as similarity measure.
This architecture represents the \ourmethod's basis, which we call \ourmethodbase to which we add our novel three auxiliary losses, leading to \ourmethodfull or simply \ourmethod, except where stated otherwise. It is worth noting that  \ourmethodbase in principle could be substituted by another specific finetuning approach, as we will see in the \suppmat.

%To maintain compatibility with the pre-trained VLM space, we keep the original image-text alignment loss $\originalloss$~\yiming{cite CLIP?}, preserving high-level semantic consistency.
The three auxiliary learning objectives which align structure-centric visual and textual contents at multiple levels are: i) the primary \emph{Structure-centric image-text alignment loss} $\structloss$, featuring the structural-centric image-text alignment to promote the learning of structurally-aligned representation across both modalities; ii) the \emph{Local structure-centric image-text alignment loss}  $\structlosslocal$, which captures compositional semantics between local parts in both modalities; %we also introduce  between the visual patches of the structure-centric image and the textual chunks of structure-centric text; 
iii) finally, the \emph{Consistency regularization loss} $\consistencyloss$ between the raw color image and the extracted structure-centric visual content, preventing modality drift. %we introduce as a regularization term, . 
%Together, these objectives progressively refine the model’s ability to ground structural semantics with increasing granularity.



\noindent\textbf{Structure-centric image-text alignment $\structloss$.}
Building upon the extracted structure-centric visual and textual content,
we introduce a structural contrastive objective 
to explicitly align the representation between $\imagestruct$ with $\textstruct$. 
We quantify the similarity $\structsimilarity$ between  $\visualencoder(\imagestruct)$ and $\textencoder(\textstruct)$ as:
\begin{equation}
\structsimilarity = \tempstruct<\visualencoder(\imagestruct),~\textencoder(\textstruct)>,
\end{equation}
where $\tempstruct$ is a separate learnable temperature dedicated to the structure-centric image-text alignment, and $<\cdot,~\cdot>$ is the operator computing the cosine similarity of two vectors.
We aim to minimize the structure-centric cross-modal similarity via the symmetric InfoNCE loss, expressed as:
\begin{equation}
% \resizebox{0.99\linewidth}{!}{$
\structloss 
= \frac{1}{2N} \sum_{i=1}^{N}
\left(
-\log \frac{\exp(\structsimilarity_{i,i})}{\sum_{j=1}^{N}\exp(\structsimilarity_{i,j})}
-\log \frac{\exp(\structsimilarity_{i,i})}{\sum_{j=1}^{N}\exp(\structsimilarity_{j,i})}
\right),
% $}
\label{eq:structloss}
\end{equation}
where $N$ is the batch size. $\structloss$ follows the same loss expression as the original image-text alignment loss $\originalloss$, but focuses on capturing  the semantic alignment on the structural semantics on both modalities.
%$\mathcal{L}_{\text{ET}}$ focuses on the structural correspondence between modalities, 
%thereby decoupling geometric reasoning from appearance modeling.

\noindent\textbf{Local structure-centric image-text alignment $\structlosslocal$.} 
In addition to $\structloss$, which features the global alignment between between $\imagestruct$ with $\textstruct$, we further introduce a local-level alignment to capture the fine-grained correspondences of atomic structural semantic. A scheme is reported in Fig.~\ref{fig:overview}. 
Inspire by Local Image–Sentence Matching (LISM)~\cite{goal2025}, we first segment both the structure-centric image $\imagestruct$ and the text $\textstruct$, where the segments from both modalities are then aligned during the learning. 
Specifically, we apply the Segment Anything Model (SAM)~\cite{kirillov2023segment} on the original color image $\image_i$ to generate a set of visually and semantically coherent masks $\maskset_i$. With these visual masks, we can then obtain the corresponding regions of the structure-centric image $\imagestruct$, obtaining the set of local structure-centric visual regions $\imageregionset_i$. On the textual side, we segment the textual counterpart $\textstruct$ into multiple phrases based on sentence delimiters (\eg, periods or semicolons), forming a set of text chunks $\textchunkset_i$ of size $M_i$ that varies based on each textual description. 

We employ a multi-positive contrastive learning strategy to jointly model the one-to-many correspondence between each local phrase $\textchunk_{m}\in \textchunkset_i$ and a total of $K$ structure-centric visual regions that are most semantically aligned $\imageregionset_m^K$~based on the pre-trained VLM encoders. %For each local phrase $\textchunk_{i,n}$, we compute cross-modal similarity between and all candidate regions using the basic CLIP model, and retain the top-$K$ most relevant structural embeddings as the local positive set:
% \begin{equation}
%     \mathcal{P}_i = \{\mathbf{v}_{i,k}\}_{k=1}^{K}.
% \end{equation}
%To achieve alignment within the structural modality, we crop the corresponding regions in the structural image $I^{\text{str}}$ based on the coordinates of the selected regions in the RGB image, thus obtaining matched structural-text local pairs. 
For each text chunk $\textchunk_{m}$ of structure-centric image $\imagestruct_i$, the local alignment loss $\ell_{m}$ is computed as:
\begin{equation}
    \ell_{m}
    = -\log
    \frac{
        \sum\limits_{\imageregion_k \in \imageregionset_n^K}
        \exp~\bigl(\gamma\, \textencoder(\textchunk_{m})\cdot \visualencoder(\imageregion_k)\bigr)
    }{
        \sum\limits_{\imageregion_j \in \imageregionset^{B}}
        \exp~\bigl(\gamma\, \textencoder(\textchunk_{m})\cdot \visualencoder(\imageregion_j)\bigr)
    },
    \label{eq:local_loss}
\end{equation}
where $\gamma$ is the temperature and $\imageregionset^{B}$ represents the set of visual local regions within a batch.

The final loss $\structlosslocal$ is computed by averaging $\ell$ over the visual regions of all samples in the batch of size $N$:
%Finally, to obtain the overall local alignment objective we average the loss across all valid samples in the batch to obtain the overall local alignment objective:
\begin{equation}
\structlosslocal =
\frac{1}{N}
\sum_{i=1}^{N}
\frac{1}{M_i}
\sum_{m=1}^{M_i}
\ell_{m}.
\label{eq:chunkloss}
\end{equation}
$\structlosslocal$ does not require additional annotations, and its multi-positive formulation allows each text phrase to align with multiple structure-centric visual regions simultaneously, enhancing the model’s capacity to capture compositional semantics
and multi-part descriptions.

\noindent\textbf{Consistency regularization $\consistencyloss$.}
While the structure-centric alignment provides additional supervision, its representation may gradually deviate from the original semantic manifold during the VLM finetuning. To mitigate this issue, we introduce the consistency regularization loss $\consistencyloss$, using the visual representation of the original image as an anchor to constrain the updated representation within the shared embedding space.
We compute $\consistencyloss$ within the N-batch as:
\begin{equation}
\consistencyloss =
\frac{1}{N} \sum_{i=1}^{N}
\left(
1 - <\visualencoder(\image_i),~\visualencoder(\imagestruct_i)>
% \frac{
% \visualencoder(\image_i) \cdot \visualencoder(\imagestruct_i)
% }{|\visualencoder(\image_i)|_2 , |\visualencoder(\imagestruct_i)|_2
% }
\right).
\end{equation}
This regularization anchors the representation learning within the pre-trained vision-language latent space, ensuring training stability and semantic consistency.


% \noindent\textbf{Global RGB-Text Alignment Loss.} \yiming{this can be left minimal since it is the original loss.} We retain the standard contrastive learning objective to maintain compatibility with the global vision-language embedding space.
% Given an RGB image $I^{\text{rgb}}$ and its caption $T^{\text{orig}}$, 
% we encode them as:
% \begin{equation}
% \mathbf{v}^{\text{rgb}} = f_\theta(I^{\text{rgb}}),
% \quad
% \mathbf{t}^{\text{orig}} = g_\theta(T^{\text{orig}}),
% \end{equation}
% and compute their cosine similarity after $\ell_2$ normalization:
% \begin{equation}
% S^{\text{rgb-txt}}_{ij} = \tau_{\text{rgb}} \, \hat{\mathbf{v}}^{\text{rgb}}_i (\hat{\mathbf{t}}^{\text{orig}}_j)^\top,
% \end{equation}
% where $\tau_{\text{rgb}}=\exp(\alpha_{\text{rgb}})$ is a learnable temperature. 
% The symmetric InfoNCE loss is defined as:
% \begin{equation}
% \mathcal{L}_{\text{RT}} 
% = \frac{1}{2N} \sum_{i=1}^{N}
% \Big[
% -\log \frac{\exp(S^{\text{rgb-txt}}_{ii})}{\sum_{j}\exp(S^{\text{rgb-txt}}_{ij})}
% -\log \frac{\exp(S^{\text{rgb-txt}}_{ii})}{\sum_{k}\exp(S^{\text{rgb-txt}}_{ki})}
% \Big].
% \end{equation}
% This loss ensures global semantic alignment between RGB images and captions in the joint embedding space.

\noindent\textbf{Full Learning Objective.}
%\ourmethod is designed as a structure-aware finetuning framework 
%built upon pretrained vision-language models, 
%targeting more stable and precise alignment under complex and long-text descriptions.
The full training objective combines the three proposed losses that encourages multimodal structural semantic alignment, with the original $\originalloss$ in a weighted manner:
\begin{equation}
\mathcal{L}_{\text{total}} 
%= \lambda_{1}\originalloss
= \originalloss
+ \lambda_{1}\structloss
+ \lambda_{2}\consistencyloss
+ \lambda_{3}\structlosslocal,
\end{equation}\label{eq:total.loss}
where $\lambda_{1\text{--}3}$ are weighting coefficients that are empirically set.
% $\lambda_{1}=1.0$, $\lambda_{2}=0.25$, $\lambda_{3}=0.1$, and $\lambda_{4}=0.1$.
Through this finetuning objective, 
\ourmethod can effectively enhance the shared multimodal representation with a better alignment in appearance and structural semantics, especially for long texts with rich semantic details.
%
%
%
\subsection{A theoretical view}
Here we provide an information-theoretic perspective on \ourmethod, supported by a numerical analysis conducted on a real fine-tuning experiment that produced the performance results reported for \ourmethod in Tab.~\ref{tab:main_results}.

We consider visual-language alignment under an information-theoretic lens~\cite{poole2019variational,wu2020mutualinformationcontrastivelearning}, following common practice in contrastive representation learning. 

The overall objective in Eq.~\ref{eq:total.loss} seeks to maximize 
the mutual information $\mutualinfo(\image,~\desc)$ between the image representation $\image$ and its corresponding text $\desc$. In this analysis, we focus on the three losses $\originalloss$, $\structloss$ and $\consistencyloss$, since the local loss $\structlosslocal$ can be seen as a specification of $\structloss$.
\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/loss_gradnorm_cosine_compact.pdf}
    \caption{Empirical analysis confirming the information-theoretic view of \ourmethod. a) Loss convergence; b) Gradient norms and ratio evolution; c) Inter-task cosine similarity.}
    \label{fig:theory.exp}
\end{figure}
Let $\structextractor(\cdot)$ and $\mathcal{F}(\cdot)$ be deterministic mappings that produce simplified counterparts
$\imagestruct=\structextractor(\image)$ and $\textstruct = \mathcal{F}(\desc)$, respectively.
In practice, $\imagestruct$ is an edge map encoding structural information, while $\textstruct$ is a caption filtered to remove tokens related to color and material.
Both can therefore be regarded as information-reduced versions of the original modalities, since (i) the edge map contains binary ${0,1}$ values instead of RGB triplets, and (ii) the textual vocabulary is stripped of color and material terms. %Still,  preserving structure while discarding appearance cues.

By the Data Processing Inequality (DPI)~\cite{tishby99information}, 
the compressed representations satisfy
\[
\mutualinfo(\imagestruct,~\textstruct) \le \mutualinfo(\image,~\desc).\footnote{We also verify numerically by MINE mutual information neural estimator~\cite{belghazi2018mine} that $\mutualinfo(\imagestruct,~\textstruct)\simeq0.01$; $ \mutualinfo(\image,~\desc)\simeq 0.1$  on the DOCCI dataset~\cite{docci2024} in the experiment of Tab.~\ref{tab:main_results}.}
\]
As commonly done in information-theoretic representation learning, we approximate the two mutual information quantities using their InfoNCE lower bounds~\cite{poole2019variational,wu2020mutualinformationcontrastivelearning}:
$\mutualinfo(\image,\desc) \ge \log N - \mathbb{E}[\originalloss]$ and
$\mutualinfo(\imagestruct,\textstruct) \ge \log N - \mathbb{E}[\structloss]$,
where $N$ is the batch size.

In Fig.~\ref{fig:theory.exp}~a) we show the two losses $\originalloss$ and $\structloss$. Empirically, we observe that the gradients of the two losses,
$\nabla_\theta \originalloss$ and $\nabla_\theta \structloss$,
are positively correlated in their direction (Fig.\ref{fig:theory.exp}~c)), considering cosine similarity ($\mu=0.6872, \sigma=0.1028$, min$=0.57$, max$=0.89$)
This indicates that the two optimization objectives
pursue compatible optima in the parameter space. Experimentally, we observed that the presence of the consistency loss $\consistencyloss$ strengthens this correlation, while disabling it does not significantly reduce the correlation, indicating that the two problems are inherently related.

However, since $\imagestruct$ and $\textstruct$ encode fewer degrees of freedom,
the auxiliary maximization $\mutualinfo(\imagestruct,\textstruct)$
is inherently more difficult, leading to a later convergence of $\structloss$, as we can see from Fig.\ref{fig:theory.exp}~a) where we showed the iteration after which we measured convergence of the two losses, and Fig.\ref{fig:theory.exp}~b) where we plot the magnitude of the gradients of $\nabla_\theta \originalloss$ and $\nabla_\theta \structloss$ and their ratio. Convergence has been evaluated by adopting the two-regime learning-curve method of Gaussian-process theory, which defines the onset of convergence as the point where model error becomes comparable to or lower than the estimated noise level~\cite{sollich2002learning,viering2022shape}.

As a result, $\structloss$ provides a persistent and informative gradient
even when $\originalloss$ flattens, effectively steering optimization toward
semantically coherent minima.

This mechanism can be interpreted considering multitask optimization
and gradient diversity.
Information-theoretic analyses of multitask learning~\cite{MTLasMOO.NIPS18}
and contrastive representation learning~\cite{wu2020mutualinformationcontrastivelearning}
show that auxiliary objectives with lower mutual information act as implicit
regularizers, introducing controlled gradient diversity that expands the
effective search space and improves convergence stability.
In our formulation, the structure-centric auxiliary alignment $\structloss$ plays exactly this role:
it introduces a correlated, information-reduced objective that contributes
complementary gradient directions, maintaining active updates when the main
contrastive gradients approach zero.
This interpretation is consistent with multi-objective optimization theory~\cite{gradientSGDvariantNIPS20},
where correlated auxiliary tasks help avoid premature convergence, thus promoting better generalization.






==> sec/old/notification13.11.25.tex <==

\newcommand{\Real}{\mathbb{R}}
\newcommand{\sharedspace}{\Real^d}%
\newcommand{\textspace}{\mathcal{L}}
\newcommand{\visualspace}{\mathcal{V}} 
\newcommand{\image}{I}
\newcommand{\desc}{T}
\newcommand{\prompfiltering}{P}
\newcommand{\imagestruct}{I'}
\newcommand{\textstruct}{T'}
\newcommand{\tempstruct}{\tau'}
\newcommand{\vocappearance}{\mathcal{V}^{a}}
\newcommand{\structextractor}{\mathcal{E}}
\newcommand{\originalloss}{\mathcal{L}_{I,T}}
\newcommand{\structloss}{\mathcal{L}_{I',T'}}
\newcommand{\structlosslocal}{\mathcal{L}_{I',T'}^{local}}
\newcommand{\consistencyloss}{\mathcal{L}_{I,I'}}
\newcommand{\ourloss}{\mathcal{L}^{*}}
\newcommand{\visualencoder}{f_{\mathtt{img}}} % Visual encoder
\newcommand{\textencoder}{f_{\mathtt{txt}}}   % Text encoder
\newcommand{\structsimilarity}{s'}
\newcommand{\imageregion}{r}
\newcommand{\textchunk}{c}
\newcommand{\imageregionset}{\mathcal{R}}
\newcommand{\textchunkset}{\mathcal{C}}
\newcommand{\maskset}{\mathcal{K}}

%\newcommand{\mutualinfo}{\mathcal{MI}}
\newcommand{\mutualinfo}{I_{\text{MI}}}

==> sec/old/relatedwork12.11.25.tex <==
\section{Related Works}
\label{sec:sota}



\noindent\textbf{Vision-language alignment.}
Contrastive pre-training on image-text pairs defines the dominant paradigm for joint vision--language embedding. Two loss formulations underpin nearly all current systems: CLIP \cite{radford2021learning}, which employs an InfoNCE softmax contrastive loss, and SigLIP \cite{zhai2023siglip}, later extended by SigLIP~2 \cite{zhai2023siglip2}, which replaces global normalization with pairwise sigmoid matching for improved scalability. Most subsequent dual-encoder variants remain within this family, refining the alignment through debiasing, adaptive weighting, or geometric and modular regularization, as in DeCLIP \cite{li2021declip}, ALIP \cite{dong2023alip}, GOAL \cite{goal2025}, SmartCLIP \cite{smartclip2025}, CoAPT \cite{wanglearning} and AVSE \cite{liu2025asymmetric}. Architectural extensions such as LongCLIP \cite{zhang2024longclip} expand CLIP’s text capacity via knowledge-preserving fine-tuning, while large-scale backbones such as EVA-CLIP \cite{fang2023eva} and Florence-2 \cite{yuan2024florence} push the limits of model and data size.
Fine-tuning strategies (Double-Filter, FATE, MLMP) range from full end-to-end adaptation to parameter-efficient updates \cite{he2025double, xu2025fate,noori2025test}. LiT \cite{zhai2022lit} tunes only the text branch; prompt-based methods (CoOp, CoCoOp, MaPLe, ProGrad) learn task-adaptive context tokens \cite{zhou2022coop,zhou2022cocoop,khattak2023maple,zhu2023prograd}; adapter and low-rank techniques (CLIP-Adapter, Tip-Adapter, LoRA, DoRA, Mma, Mmrl, UCDR-Adapter) provide lightweight adaptation \cite{zhang2022tipadapter,gao2023clipadapter,hu2022lora,liu2024dora,yang2024mma,guo2025mmrl,jiang2025ucdr}. 

\noindent\textbf{VLMs for long-text alignment.}
While advancement of VLMs in aligning visual and textual data, traditional models are limited to shot captions of roughly 77 tokens, which restricts their handling of complex text interactions.
Therefore, recent efforts have focused on long-text alignment. Long-CLIP \cite{zhang2024long}, TULIP \cite{najdenkoska2024tulip}, V2PE \cite{ge2025v2pe} and FineLIP \cite{asokan2025finelip} refine position encodings or introduce variable visual position encodings, achieving better alignment without affecting model semantics. DreamLIP \cite{zheng2024dreamlip} and longAlign \cite{liu2024improving} split long captions into subcaptions, aligning each with local image area to improve fine-grained correspondence. LoTLIP \cite{wu2024lotlip} generates a large-scale long text dataset and introduces learnable corner tokens in the text input to enhance the model's semantic aggregation ability for multi-clause texts. In \cite{urbanek2024picture}, images are described at the level of masked sub-regions, with each sub-region described by a caption, allowing for precise text-to-region alignment. Using a pre-trained LLM and a multi-stage projection module, MATE \cite{jang2024mate} enables efficient processing of long texts.
These methods operate on CLIP- or SigLIP-based foundations and differ mainly in how alignment is refined rather than redefined. Our approach follows this line: it augments standard contrastive training with structural edge-aware supervision, extracting visual geometry from appearance to yield sharper phrase--region correspondences and stronger optimization across all the considered backbones.









%\subsection{Vision--language alignment encoders}
%Contrastive pre-training on image--text pairs has become the default route to a joint embedding space. \textsc{CLIP} demonstrated that large-scale contrastive learning delivers strong zero-shot transfer \cite{radford2021learning}. Subsequent work stresses two axes of the recipe. First, \textsc{LongCLIP} relaxes the 77-token limit and re-aligns the space to handle lengthy or structured captions, improving retrieval under long descriptions \cite{zhang2024longclip}. Second, \textsc{SigLIP} replaces the softmax normalization in InfoNCE with a pairwise sigmoid objective, simplifying scaling while preserving alignment quality \cite{zhai2023siglip}. These encoders define the standard backbones our method builds upon.

%\subsection{ Fine-tuning strategies for VLMs}
%Fine-tuning has shifted from full end-to-end updates to parameter-efficient adaptation. \textsc{LiT} freezes the image tower and tunes only the text branch to preserve zero-shot generality while adapting to new domains \cite{zhai2022lit}. Prompt learning treats the context as learnable parameters: \textsc{CoOp} learns continuous prompts, \textsc{CoCoOp} conditions them on image features to recover out-of-distribution generalization, and \textsc{MaPLe} jointly prompts both modalities; \textsc{ProGrad} constrains prompt gradients to retain generic CLIP knowledge \cite{zhou2022coop,zhou2022cocoop,khattak2023maple,zhu2023prograd}. Adapter-based approaches insert light modules on frozen features: \textsc{Tip-Adapter} adds a non-parametric cache with optional refinement, while \textsc{CLIP-Adapter} learns residual adapters \cite{zhang2022tipadapter,gao2023clipadapter}. Low-rank updates provide strong parameter-efficiency trade-offs, from \textsc{LoRA} to weight-decomposed \textsc{DoRA} \cite{hu2022lora,liu2024dora}. Beyond classification, \textsc{DenseCLIP} formulates pixel--text alignment to transfer CLIP to dense prediction without altering the backbone \cite{rao2022denseclip}.
%``GOAL'' is a \emph{fine-tuning} recipe that augments a CLIP-like encoder with global--local geometric matching; it does not introduce a new backbone. Our approach differs in where and how supervision is applied: we disentangle \emph{structural} semantics from appearance by extracting edge-centric signals and inject them as auxiliary objectives on top of standard contrastive training. This yields sharper phrase--region correspondences and more stable optimization, and it complements rather than replaces full fine-tuning and PEFT (LoRA/DoRA). Empirically, the edge-aware objectives consistently improve cross-modal retrieval across CLIP-, LongCLIP-, and SigLIP-based backbones and also lift LoRA/DoRA variants under similar budgets, with especially clear gains on structure-sensitive datasets (sketches, fine-grained species, pathology).

%\subsection{Summary.}
%The literature suggests two high-leverage levers: change the encoder or change the supervision. We adopt the latter. By aligning edge-centric structure alongside global image--caption signals, our method keeps compatibility with common backbones and PEFT while strengthening local grounding and transfer.
%In this regard, our edge-aware auxiliary losses inject structural semantics during fine-tuning, which sharpens phrase–region grounding and remains compatible with full FT and PEFT; empirically this lifts retrieval across CLIP, LongCLIP, and SigLIP backbones, and also improves LoRA/DoRA variants with similar budgets, with the largest gains on structure-sensitive data.

\noindent\textbf{VLMs finetuning by disentanglement.} Our approach could be seen as disentangling structure oriented knowledge from the multimodal data. Recent research has explored how disentangling semantic factors can improve multimodal alignment. 
DEAL \cite{li2024deal} separates concept-level components within a category to enhance localization and interpretability in vision--language models, while PPE \cite{xu2021ppe} prevents attribute entanglement by explicitly decoupling textual and visual variations in image manipulation. 
UniDiff \cite{dong2023unidiff} integrates discriminative and generative objectives to maintain semantic consistency during fine-tuning, and VLMo \cite{bao2021vlmo} introduces a mixture-of-experts backbone that balances modality-specific and shared representations. 
\mc{from here on it is a little complicated, since there are many dangerous terms as structured supervision (that we do not have anything to do)... maybe it is better to talk about supervision by disentanglement?}
Disentangled retrieval formulations further highlight that structured supervision improves cross-modal generalization \cite{zhou2022vdr,jin2023dicosa,zhang2024homology}. 
These studies collectively suggest that injecting structural priors early in the pipeline can act as an inductive bias, guiding alignment toward more compositional and geometry-aware representations \cite{wang2025textural,li2024deal,wang2024learning,varma2024ravl}. 
Unlike these approaches, our method formalizes this intuition within an information-theoretic framework: the auxiliary alignment between edge maps and edge-oriented text introduces a correlated, information-reduced objective that maintains active gradients and stabilizes contrastive fine-tuning, ultimately leading to sharper phrase–region correspondences.

==> sec/old/somelogs.tex <==
\usepackage{booktabs}
\usepackage{siunitx}
\usepackage{xcolor}
\sisetup{detect-weight=true, detect-inline-weight=math}

\definecolor{origbg}{HTML}{FFF8DC} % light yellow
\definecolor{qwenbg}{HTML}{E9FFE9} % light green

\begin{table*}[ht!]
\centering
\small
\renewcommand{\arraystretch}{1.2}

% ---------- ORIGINAL TEST SET ----------
\rowcolors{2}{origbg}{white}
\begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
}
\toprule
\multicolumn{6}{c}{\textbf{Test Set: original\_test\_set (Text→Image)}}\\
\midrule
\textbf{Model} & {\textbf{R@1}} & {\textbf{R@5}} & {\textbf{R@10}} & {\textbf{R@25}} & {\textbf{R@50}} \\
\midrule
original\_clip & 1.31 & 4.73 & 8.40 & 16.20 & 25.66 \\
qwen3\_clip & 1.04 {\color{red}↓0.27} & 4.71 {\color{red}↓0.02} & 7.65 {\color{red}↓0.75} & 14.76 {\color{red}↓1.44} & 22.76 {\color{red}↓2.90} \\
original\_ours & \textbf{1.29} {\color{blue}↑0.02} & \textbf{5.23} {\color{blue}↑0.50} & \textbf{8.92} {\color{blue}↑0.52} & \textbf{17.81} {\color{blue}↑1.61} & \textbf{26.53} {\color{blue}↑0.87} \\
qwen3\_ours & 1.02 {\color{red}↓0.29} & 4.51 {\color{red}↓0.22} & 7.65 {\color{red}↓0.75} & 15.33 {\color{red}↓0.87} & 24.52 {\color{red}↓1.14} \\
qwen3+original\_ours (B) & 1.19 {\color{blue}↑0.12} & 4.78 {\color{blue}↑0.05} & 8.35 {\color{blue}↓0.05} & 17.36 {\color{blue}↑1.16} & 26.58 {\color{blue}↑0.92} \\
\bottomrule
\end{tabular}

\vspace{0.5em}

\rowcolors{2}{origbg}{white}
\begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
}
\toprule
\multicolumn{6}{c}{\textbf{Test Set: original\_test\_set (Image→Text)}}\\
\midrule
\textbf{Model} & {\textbf{R@1}} & {\textbf{R@5}} & {\textbf{R@10}} & {\textbf{R@25}} & {\textbf{R@50}} \\
\midrule
original\_clip & 1.02 & 4.29 & 7.13 & 15.90 & 24.47 \\
qwen3\_clip & 0.87 {\color{red}↓0.15} & 4.43 {\color{blue}↑0.14} & 7.33 {\color{blue}↑0.20} & 14.61 {\color{red}↓1.29} & 23.41 {\color{red}↓1.06} \\
original\_ours & \textbf{1.11} {\color{blue}↑0.09} & \textbf{5.20} {\color{blue}↑0.91} & \textbf{8.79} {\color{blue}↑1.66} & \textbf{16.52} {\color{blue}↑0.62} & \textbf{25.14} {\color{blue}↑0.67} \\
qwen3\_ours & 0.92 {\color{red}↓0.10} & 4.06 {\color{red}↓0.23} & 7.41 {\color{blue}↑0.28} & 15.61 {\color{red}↓0.29} & 23.66 {\color{red}↓0.81} \\
qwen3+original\_ours (B) & 1.29 {\color{blue}↑0.27} & 4.90 {\color{blue}↑0.61} & 8.35 {\color{blue}↑1.22} & 16.03 {\color{blue}↑0.13} & 24.89 {\color{blue}↑0.42} \\
\bottomrule
\end{tabular}

% ---------- QWEN3 TEST SET ----------
\vspace{1em}
\rowcolors{2}{qwenbg}{white}
\begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
}
\toprule
\multicolumn{6}{c}{\textbf{Test Set: qwen3\_test\_set (Text→Image)}}\\
\midrule
\textbf{Model} & {\textbf{R@1}} & {\textbf{R@5}} & {\textbf{R@10}} & {\textbf{R@25}} & {\textbf{R@50}} \\
\midrule
original\_clip & 1.14 & 4.41 & 7.41 & 14.44 & 22.79 \\
qwen3\_clip & 0.94 {\color{red}↓0.20} & 4.58 {\color{blue}↑0.17} & 7.63 {\color{blue}↑0.22} & 14.57 {\color{blue}↑0.13} & 23.48 {\color{blue}↑0.69} \\
original\_ours & 1.04 {\color{red}↓0.10} & 4.63 {\color{blue}↑0.22} & 8.25 {\color{blue}↑0.84} & 15.70 {\color{blue}↑1.26} & 23.68 {\color{blue}↑0.89} \\
qwen3\_ours & 1.16 {\color{blue}↑0.02} & 4.31 {\color{red}↓0.10} & 7.90 {\color{blue}↑0.49} & 15.48 {\color{blue}↑1.04} & 24.75 {\color{blue}↑1.96} \\
qwen3+original\_ours (B) & \textbf{1.31} {\color{blue}↑0.17} & \textbf{4.71} {\color{blue}↑0.30} & \textbf{8.05} {\color{blue}↑0.64} & \textbf{15.75} {\color{blue}↑1.31} & \textbf{24.62} {\color{blue}↑1.83} \\
\bottomrule
\end{tabular}

\vspace{0.5em}

\rowcolors{2}{qwenbg}{white}
\begin{tabular}{
    l
    S[table-format=1.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
    S[table-format=2.2]
}
\toprule
\multicolumn{6}{c}{\textbf{Test Set: qwen3\_test\_set (Image→Text)}}\\
\midrule
\textbf{Model} & {\textbf{R@1}} & {\textbf{R@5}} & {\textbf{R@10}} & {\textbf{R@25}} & {\textbf{R@50}} \\
\midrule
original\_clip & 1.24 & 3.59 & 6.69 & 14.12 & 22.05 \\
qwen3\_clip & 1.14 {\color{red}↓0.10} & 3.89 {\color{blue}↑0.30} & 7.08 {\color{blue}↑0.39} & 14.39 {\color{blue}↑0.27} & 22.54 {\color{blue}↑0.49} \\
original\_ours & 1.04 {\color{red}↓0.20} & 4.09 {\color{blue}↑0.50} & 7.23 {\color{blue}↑0.54} & 14.64 {\color{blue}↑0.52} & 23.31 {\color{blue}↑1.26} \\
qwen3\_ours & 1.14 {\color{red}↓0.10} & 3.91 {\color{blue}↑0.32} & 7.28 {\color{blue}↑0.59} & 14.34 {\color{blue}↑0.22} & 23.04 {\color{blue}↑0.99} \\
qwen3+original\_ours (B) & \textbf{1.07} {\color{red}↓0.17} & \textbf{4.24} {\color{blue}↑0.65} & \textbf{7.41} {\color{blue}↑0.72} & \textbf{14.79} {\color{blue}↑0.67} & \textbf{23.66} {\color{blue}↑1.61} \\
\bottomrule
\end{tabular}
\caption{\textbf{Retrieval results (R@K) comparison across models and test sets.} 
Yellow background: original\_test\_set; Green background: qwen3\_test\_set. 
Blue numbers indicate improvements, red indicate declines relative to baseline.}
\label{tab:pathgen_results}
\end{table*}


==> sec/why.tex <==
\section{Why does the structural alignment work?}
\subsection{A theoretical view}
Given the broad applicability and strong empirical performance of \ourmethod, 
it is natural to investigate its underlying theoretical properties. 
From an information-theoretic perspective, the overall objective is to maximize 
the mutual information $\mutualinfo(\image,~\desc)$ between the representation of the image $\image$ and its corresponding text $\desc$. 

Let $\structextractor(\cdot)$ and $\mathcal{F}(\cdot)$ be deterministic mappings 
that produce structural counterparts $\imagestruct=\structextractor(\image)$ and $\textstruct = \mathcal{F}(\desc)$, respectively. 
%
In terms of representational complexity, $\imagestruct$ and $\textstruct$ can be regarded as simplified versions of $\image$ and $\desc$, 
as they encode fewer degrees of freedom: 
$\imagestruct$ is a binary $\{0,1\}$ edge map, while $\textstruct$ removes tokens that are associated with 
chromatic or stylistic attributes.  

By the Data Processing Inequality (DPI)~\cite{tishby99information}, 
the compressed views satisfy
\[
\mutualinfo(\imagestruct,~\textstruct) \le \mutualinfo(\image,~\desc).
\]
The mutual information of both of them are estimated through InfoNCE lower bounds: 
$\mutualinfo(\image,\desc) \ge \log N - \mathbb{E}[\originalloss]$ and 
$\mutualinfo(\imagestruct,~\textstruct) \ge \log N - \mathbb{E}[\structloss]$, 
where $N$ denotes the batch size.

Empirically, the gradients of the two losses, 
$\nabla_\theta \originalloss$ and 
$\nabla_\theta \structloss$, 
exhibit similar orientation, suggesting that the two 
mutual information maximization problems are \textbf{\textit{correlated}} 
and \textbf{\textit{act toward compatible optima}}. 
However, since $I'$ and $T'$ contain less information, 
the auxiliary problem is inherently more difficult, 
and its InfoNCE bound saturates slower. 
Consequently, $\structloss$ provides a persistent gradient signal 
even when $\originalloss$ approaches saturation, 
effectively pulling the optimization toward more stable 
and semantically coherent configurations in parameter space.

\subsection{Empirical analysis on loss correlation}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{imgs/loss_gradnorm_two_legends.pdf}
    \caption{Caption}
    \label{fig:placeholder}
\end{figure}
\yiming{here we show the correlation of the two losses, I believe. the blow should be revised }

In this section, we provide empirical emphasis on 
the correlation of the two losses

Specifically, we investigates what kind of characteristics in the edge are most effective. Key factors to investigate: structural density, sharper (high-frequency) or smother (low-frequency), uniformly distributed or more clustered?
We can identify some samples that 1) base model fails, but our model succeed, 2) base model works but our model fails, 3) base model fails, and our model also fails, 4) base model works, and our model works. Then we extract the investigated factor and we check if there are any clear correlation.

% \section{Why the model works with few data}
% \yiming{I feel this part below can be integrated into the ablation part as part of the discussion why low-data regime works.}
% Our approach exhibits strong performance in the few-data fine-tuning regime because it focuses the optimization on the informative components of the signal. 
% In standard global fine-tuning, the model must adapt a large parameter space to account for every visual and textual variation, including nonsemantic noise, which requires extensive supervision. 
% In contrast, our disentangled extractions $X_E$ and $Y_E$ isolate structural cues such as edges and textual chunks that retain the core semantics while suppressing nuisance factors. 
% The accompanying objectives $\mathcal{L}_{\text{ST}}$, $\mathcal{L}_{\text{RS}}$, and $\mathcal{L}_{\text{CK}}$ further constrain the alignment toward consistent and interpretable relations across modalities. 
% This structural bias effectively reduces the hypothesis space and the variance of gradient updates, yielding faster convergence and improved generalization under limited data. 
% In simple terms, the model learns less but better, focusing its capacity on semantically stable features that global fine-tuning must otherwise relearn from larger datasets.





